Probing Across Time: What Does RoBERTa Know and When?

Models of language trained on very large corpora have been demonstrated useful for NLP. As fixed artifacts, they have become the object of intense study, with many researchers "probing" the extent to which linguistic abstractions, factual and commonsense knowledge, and reasoning abilities they acquire and readily demonstrate. Building on this line of work, we consider a new question: for types of knowledge a language model learns, when during (pre)training are they acquired? We plot probing performance across iterations, using RoBERTa as a case study. Among our findings: linguistic knowledge is acquired fast, stably, and robustly across domains. Facts and commonsense are slower and more domain-sensitive. Reasoning abilities are, in general, not stably acquired. As new datasets, pretraining protocols, and probes emerge, we believe that probing-across-time analyses can help researchers understand the complex, intermingled learning that these models undergo and guide us toward more efficient approaches that accomplish necessary learning faster.

==> archived/first_version/abstract.tex <==
\begin{abstract}
%\jungo{Overall, we need better organization and paragraph transitions. There are several places where I didn't know why you started talking about something only to find it out in the middle of the paragraph.}
Numerous probing papers have shown the abundance of a wide extent of \textit{knowledge} in pretrained language models (PTLMs), which explains their success on a wide range of downstream tasks. However, it remains unclear at which stage and with which pattern some tested knowledge is learned from unstructured text by mere self-supervision signals. 
% To push our understanding of PTLMs forward, we realize and utilize one fundamental premise of the probing literature --- probes should reflect the knowledge of PTLMs at any stage of training. \jungo{The preceding sentence seems a bit odd to me. Can we rephrase it to something like ``we propose dynamic probing''? Love to hear you guys' thought. } \zeyu{I agree its confusing, see next sentence} 
% \jungo{Cool. Delete the preceding sentence then?}
To advance our understanding of PTLMs, we propose \textit{dynamic probing}, a probing framework motivated by a hidden probe construction premise --- the correctness on probing examples reflects how closely model conforms to human understanding of the world regardless of model's state.  We leverage a large suite of probes developed recently to observe \textit{knowledge dynamics}, the trajectory of knowledge in the model during the course of pretraining. Our experiments on different domains reveal several very different patterns of knowledge dynamics for different types of knowledge. First, linguistics knowledge, often deemed as crucial for the success of PTLMs, is usually mastered very fast and early.
Second, factual and some commonsense knowledge is learned relatively slowly. Lastly, some reasoning knowledge is not stably stored in the model. Our results confirms that the self-supervision signal surprisingly may not suffice to create a train-once-use-everywhere PTLM; and the quality of some knowledge in PTLMs depends much on the choice of corpus domain and size.
Our findings provide insight into further development of PTLMs.
\end{abstract}


% Second version
% \begin{abstract}
% To attribute the universal success of Pre-Trained Language Models (e.g. \robertaAtEnd) on a wide range of downstream tasks (e.g. SQuAD \citet{squad1.1-dataset}), many interpretability work have used their performance --- usually the higher, the better --- on carefully designed probing tasks (e.g. Part-of-Speech tagging) to show those models ``contain more knowledge of some desired property" by comparing against the performances of reasonably chosen baselines (e.g. GloVe). But is this design paradigm complete? In this paper, we propose to add a global \textit{learning dynamics view} on designed probes, which associates probing performances with the pretraining procedure of any Language Models. This perspective allows us to i) discover that some way to probe models seems \textit{invalid} for attribution and compare any new probes with existing probe if what they measures overlaps, and ii) more interestingly, utilize the valid probes to have a closer look at the knowledge acquisition process of any language models.
% % \footnote{We called them \textit{probes} in this paper.}
% \end{abstract}
% % For example, ``stronger" representations from \roberta are able to make probe achieve higher performance on the Part-of-Speech tagging task than ``weaker" representations (e.g. GloVe). But does this design paradigm guarantee us with a completely trust worthy probes? 


% First version
% \begin{abstract}
% Pre-trained language models have dominated many NLP tasks, and recent research has revealed that the representations from these models can encode surprising extents of knowledge, including linguistic properties, factual knowledge, commonsense or even complex \zeyu{?} reasoning. However, it remains unclear how such knowledge is learned from the unstructured text by mere self-supervision. In this work, we investigate the pre-training dynamics of typical language models, by looking at not only the loss but also a series of probing tasks over training stages. We find that different types of knowledge are learned in very different patterns and have dependency on different factors, and the layers for encoding them also change during pre-training. We show that the speed of learning linguistic knowledge are negatively correlated with the superficiality of one linguistic aspect (e.g., POS tagging, CCG parsing). We further correlate the successfully learned knowledge with our training data, showing that models can learn new non-linguistic knowledge by both memorization and generalization. \yizhong{Some conclusions here are just hypotheses.}
% \end{abstract}



==> archived/first_version/conclusion.tex <==
\section{Conclusion and Future Implication}

In this work, we offer a framework to study the knowledge dynamics during pretraining. We were not the first to monitor PTLM dynamics over time \citep{dynamics-by-svcca}, but we were the first to do so from a \textit{knowledge probing} perspective with broad coverage. With \roberta as a case study, we found different knowledge has very distinct learning patterns and various lengths of learning phases. 

Given these observations, future PTLM researcher should think of how to help PTLM more efficiently incorporate senses in token representation and acquire non-linguistic knowledge comprehensively. Promising directions offered by us include: 1) clever data selection as part of preprocessing 2) more generalizable objective that is superior and more comprehensive than MLM by design 3) modification on transformer design that leads to wider knowledge acquisition --- stacking Multi-Head Attention is NOT` all you need! For future interpretability researchers, our finding encourages the discovery of more knowledge probes and, arguably more importantly, more fine-grained analysis to pin-point the success of PTLM (e.g. which groups of neurons help to learn $\mathcal{X}$ knowledge and, in the context of optimization/dynamics, why so).

==> archived/first_version/discusison.tex <==
\section{Discussion of knowledge}
In another word, the approximate measure of ``knowledge" by probes is the measure of how the model, by self-supervision, learns to conform human designed reference. 

==> archived/first_version/dynamic_probing.tex <==
\section{Probes across Time}
We present our method to probe the knowledge dynamics of self-supervised pretraining here. \textsection \ref{sec:method:core_idea} discusses the motivation of our methodology and high-level design choices. Then, we discuss the pretraining process (\textsection \ref{sec:method:pretraining}), knowledge probes (\textsection \ref{sec:method:probes}), and downstream tasks (\textsection \ref{sec:method:downstream}) chosen in our framework. 
\label{sec:method}

\subsection{Background and Motivation}
\label{sec:method:core_idea}
\textit{Why do pretrained language models work so well in so many tasks?}
Since the success of large-scale pretraining \cite{elmo, devlin_bert:_2018}, this fundamental question has inspired a flurry of recent papers that analyze and interpret pretrained language models (PTLMs) in various aspects of natural language, including syntax \cite{blevins-etal-2018-deep, hewitt-manning-2019-structural}, semantics \cite{nelson-probe}, and commonsense knowledge \cite{da-kasai-2019-cracking, lama-probe}.
These analysis papers measure the degree to which contextual representations from PTLMs encode different types of information by evaluating on targeted \textit{probing} tasks.
While a wide range of probing tasks have recently been proposed \cite{belinkov-etal-2020-interpretability-tutorial}, almost all the probes are assumed to be static up until now: probing is only applied to publicly available pretrained models that are obtained after an arbitrary number of updates.
But what is happening in the course of the parameter updates? Do we really need so many update steps that make it virtually impossible to pretrain competitive language models from scratch in a standard academic environment?
Can we make pretraining more efficient?

We fill this gap in the probing literature by developing a dynamic probing framework. In particular, we apply a rich suite of probes over the course of pretraining a masked language model, \roberta, and analyze how the probing performance progresses over time.
Our extensive observations contribute to the large body of work that investigates why PTLMs substantially improve downstream performance.

%accurate a pretrained language model can get on a set of examples constructed by using some knowledge repertoires.
%This is indicative of how closely the model conforms to human understanding of the world because those knowledge sources i) were constructed \textit{independently} of training the probed model and ii) intend to best reflect human knowledge --- linguistic (e.g., PennTree Bank) or non-linguistic (e.g., ConceptNet) \jungo{citation}. In other words, the test does not depend on the prior about any model but on the desired outcome from a learning process (i.e., training the model). In our case, this leads to a very simple yet crucial premise for probing PTLM: 

%\textit{The performances of designed probes reflect the ability of a PTLM at any stage of training}.


%To the best of our knowledge, this straightforward premise is surprisingly unspoken at time of previous probe designs \cite{kohn-2015-whats,  cooper-1996-early-behavioral-probe} \zeyu{both are from \citet{belinkov-etal-2020-interpretability-tutorial}; first is earliest structural probe, second is earliest behavioral; no permission to read the last, judge from abstract}. However, we believe this premise has to hold and already drives the probe designs for years. Our work utilizes this premise to advance our understanding of PTLMs.

\subsection{Pretraining Checkpoints}
In order to analyze a pretrained language model over the course of its training, we train a \roberta model from scatch and periodically save the checkpoints.
We save more frequently (every 1000 updates) in the first epoch. Later, if the dataset is smaller than 12GB, we save a checkpoint every epoch; otherwise, we save every time 12GB of text is fed to the model.
%to collect enough checkpoints.
\zeyu{Need to confirm with Yizhong}


Our \roberta training setting follows closely the one prescribed in \citet{liu_roberta:_2019}. 
We choose corpora of varies sizes from different domains to study the effect of the corpus size and domain (see Table \ref{tab:corpus-domain}).
We build on the tutorial from Google\footnote{\url{https://cloud.google.com/tpu/docs/tutorials/roberta-pytorch}} and run training on a v3-8 TPU.\footnote{Free usage for the public in the duration of this work.} 
More details are described in Appendix \ref{appendix:roberta-corpus}.


\subsection{Probe Suite Construction}
Here we describe how we constructed a rich set of probing tasks that we use to assess each checkpoint. We categorize probes into four classes based on the target task nature: linguistic, factual, commonsense, and basic reasoning probes. Each family contains many probes, but we provide example probes in Table \ref{tab:examples-main}.

\input{tables/tab_probe_examples_main}


%\jungo{left off here. The following needs edits.}
%We categorize the collected knowledge probes into four types --- \textbf{linguistic}, \textbf{factual}, \textbf{commonsense}, \textbf{basic reasoning} --- each containing many probes. We include probes that show both PTLM's success and its failure because we want to avoid 1) the possible catastrophic forgetting \citep{intermediate-fintuning} that may happen during pretraining \jungo{I don't know why this avoids forgetting} and 2) the arbitrary gradient updates to obtain our ``final model" (\textsection \ref{sec:intro}). Due to the space limit, we select one representative task from each probes and for each knowledge type (See Table \ref{tab}). The full descriptions are deferred to the original work, and we include the full list of probes in Appendix \ref{appendix:probe-examples}.
%

\subsubsection{Linguistic Probes} 
Due to the various linguistic theories proposed and levels of analysis (e.g., morphology, syntax, and semantics), there are many linguistic aspects from which we can analyze a sentence.
To maximize the coverage of our linguistic probes,we use non-overlapping probes from prior work \cite{nelson-probe, edge-probe, blimp-probe}.
%from \cwr\, and \edge.
\paragraph{Structural Analyses}
Structural analyses build a lightweight classifier that predicts some linguistic properties on top of contextual representations from a PTLM \cite{belinkov-etal-2020-interpretability-tutorial}.
\jungo{Need more details. Can you edit from here?}
For this we take X and Y tasks from \citet{nelson-probe} and \citet{edge-probe} respectively.
The former tasks build a classifier on each token. 
The latter trains a classifier on pairs of tokens (\textit{edge probing}).
Using insights from \citet{hewitt-probe-control}, we choose a linear model for our classifier for better selectivity.
\jungo{Explain what selectivity is. I just read the paper, but not everyone knows this.}
In structural probe designs \jungo{not sure how we should call Nelson's method as opposed to edge probing. Structural probes are probably coined by Hewitt Manning.}, the classifier receives one or optionally two representation(s) and train to predict a label such as a constituent or relation type; in \edge, the representation is from a span of tokens, while, in \cwr, the representation comes from a token. \textbf{Metric:} The accuracy is determined by whether the classifier predict the label correctly.
\jungo{Oh you're explaining CWR and edge probing here a bit. But be clearer and explain earlier.}
\paragraph{Behavioral Analyses}
%Our linguistic probes includes structural probes --- \cwr\,(Contextual Word Representation; \citet{nelson-probe}) and \edge\,(Edge Probing; \citet{edge-probe}) --- and behaviors probes --- \blimp\, (Benchmark of Linguistic Minimal Pairs; \citet{blimp-probe}).
Behavioral analyses, on the other hand, directly assess the performance of a language model on a challenge set.
\blimp\, consists of 67 individual datasets (12 tested phenomena), each containing 1,000 minimal pairs, i.e. pairs of minimally different sentences that contrast in grammatical acceptability and isolate specific phenomenon in syntax, morphology, or semantics. Each test contains minimal pair of sentences. \textbf{Metric:} we determined the correctness by whether PTLM assigns higher probability to the the grammatical token given the context.


% Our linguistic probing suite includes labeling tasks: Part-of-speech tagging (\PTBpos, \EWTpos; constructed from the PennTreeBank and the English Web Treebank); Named Entity Recognition (\ner); CCG supertagging (\ccg); Syntactic Chunking (\chunk); Grammatical Error Detection (\ged); Conjunct Identification (\conj); Event Factuality (\ef); Preposition Supersense Disambiguation for lexical semantic function (\psFxn) and the semantic role or relation it mediates (\psRole); similar to part-of-speech tagging, Syntactic Dependency Arc Prediction and Classification task on PTB and EWT --- \PTBsynPred, \PTBsynClass, \EWTsynPred, \EWTsynClass; Coreference Arc Prediction (\coref); Semantic Role Labeling (\srl); Semantic Proto-Role Labeling, constructed using PTB (\PTBspr) and EWT (\EWTspr); Relation Classification (\rel).

% two tokens --- $w_{head}$  as 
% $w_{mod}$ as 
\subsubsection{Commonsense Probes}
Currently, there are different ways people have tested commonsense knowledge based on the model's behavior rather than a trained classifier \cite{da-kasai-2019-cracking}. One way is \lama\,, which contains a widely used commonsense knowledge base --- ConceptNet (\lamaConcept). 
\jungo{LAMA appears again here. Mention something like similar to .... otherwise not clear why you have the same name appear in two categories.}

Similar to \lama\,, \citet{numersense-probe} develops a specialized probe --- only numbers in range $[0, 10]$ are included --- for \textit{numerical} commonsense knowledge, called ``\text{{\normalsize N}{\footnotesize UMER}{\normalsize S}{\footnotesize ENSE}}" (\numer). \textbf{Metric:} Since the output space is much smaller than that of \lama, we measure its accuracy by whether PTLM chooses the right number.
\jungo{What is numerical commonsense? Explain?}

Another way to probe is \cat (Commonsense Ability Test; \citet{cats-probe}), where they unify the form of all the chosen datasets and compares PTLMs' probability-based score on positive (sentence that fits commonsense) and negative samples (sentences that don't). \textbf{Metric:} The accuracy is determined by whether a PTLM can score positive sample the highest. 
% For this one, we include test suites constructed from: Conjunction Acceptability (\catCA), Sense Making (\catSM), Winograd Schema Challenge (\catWSC), SWAG (\catSwag), HellaSwag (\catHS), Sense Making with Reasoning (\catSMR) and the original Argument Reasoning Comprehension Task (\catArctOne); we also include the argumented ARCT (\catArctTwo) by adding negation to alleviate its statistical cues.

\subsubsection{Factual Probes}
Factual probes deal with knowledge that requires memorization and is usually explicitly stated, in contrast to the more intuitive and implicit commonsense knowledge. 

We use probes from \lama\, (LAnguage Model Analysis; \citet{lama-probe}). For more systematic coverage, \lama\, is constructed using large knowledge bases like the Google-RE corpus \footnote{\url{https://code.google.com/archive/p/relation-extraction-corpus/}}.  These probes test the model on simple\footnote{Subject-Verb-Object sentence, optionally passive} sentences with their object masked and asked the model to predict the masked words (e.g. ``Albert Einstein was born in [MASK]"). \textbf{Metric:} Since the output space is a subset of \roberta vocabulary that excludes sub-tokens, we measure its accuracy by how high the model ranks the correct word (i.e., Precision at $K$).
% Our factual probing suite includes use knowledge sources from: Google-RE corpus (\lamaGoogle), T-REx (\lamaTrex), and SQuAD (\lamaSquad).

\subsubsection{Basic Reasoning Probes}
% we use the DELPH-IN MRS-Derived Semantic Dependencies (DM) target representation from the SemEval 2015 shared task \citep{semeval-2015-task-dataset} and
% with the DELPH-IN MRS-Derived Semantic Dependencies (DM) target representation. The probe is trained
\olmpics (\textbf{o}n what \textbf{L}anguage \textbf{M}odel \textbf{p}re-tra\textbf{i}ning \textbf{c}apture\textbf{s}; \citet{olmpics-probe}) uses ConceptNet, WordNet and others to categorize and design eight focused tests for basic reasoning abilities (e.g. Age-Comparison). The framing is similar to \numer\,and \lama, except the output space is restricted to 2-5 words depending on the tests. They show PTLMs lack many tested reasoning abilities. 
%  To account for the difference in use of language between pretraining corpus and the probing dataset, we use the fine-tuning setup where we first fine-tune \robertaAtEnd's language head \jungo{What's language head?} on a training set, and then infer on the test set; for simplicity, we only consider the final fine-tuned model's performance.
% To make \olmpics more comparable to other non-linguistic probes, we only adopt task that test PTLM as an MLM (i.e. only MC-MLM setup in the paper). 
\textbf{Metric:} Similar to \numer, we measure its accuracy by whether PTLM chooses the right token.

% The tested ability includes: use of Always-Never (\olmpicsAlways); comparison between age (\olmpicsAge) and object (\olmpicsObj) sizes; properly applying negation in the context of \textit{synonyms v.s. antonyms} (\olmpicsAntonym); ability to find concepts for which a conjunction of properties holds (\olmpicsProperty; “What is located in a street and is related to octagon?”) and find the mutual hypernym of a pair of concepts (\olmpicsTaxonomy; e.g. “A germ and a human are both a type of [MASK].”); capability to do question answering of encyclopedic (\olmpicsEncyc; e.g. ``When did the band where John Lennon played first form?”) and multi-hop (\olmpicsMultiHop; e.g. “When comparing a 83 year old, a 63 year old and a 56 year old, the [MASK] is oldest”) nature.



\label{sec:method:probes}
\input{tables/tab_baselines}
\subsection{Baselines}
Establishing appropriate baselines is critical when conducting probes: 
Due to their slightly different design, each probe has its own empirical lower and upper bounds to set references for \textit{the worst performance} and \textit{the best performance}. Although baseline performances are not comparable, we use (mostly) same idea for setting the baselines. 
\jungo{what's the idea?}

For each probe, an upper bound is the probe performance from officially released \roberta --- \robertaOfficial. Lower bounds include randomly initialized \roberta, averaged across 3 trials. In addition, each behavioral probe includes the expected accuracy by using random guess $\left(=\frac{1}{\text{\# choices}}\right)$. For each structural probe, we also replace the contextual representation with GloVe and random vectors of $[-2,2]^d$, where $d$ is the dimension of GloVe \zeyu{basically copy Table \ref{tab:baselines} caption}.
Table \ref{tab:baselines} is the full list of probes and baselines. 


%\subsection{Pretraining}
%\label{sec:method:pretraining}
%
%\paragraph{Usage} During pretraining, we periodically save the pretraining trajectory of \roberta. Overall, we save more frequently (e.g. every 1000 updates) around the first epoch; later, if the dataset is ``small" ($\leq 12$GB), we save checkpoints by epoch; otherwise, we save every 12GB text to collect enough checkpoints for later usage. 
%\zeyu{Need to confirm with Yizhong}
%
%\input{tables/tab_probe_examples_main}
%
%Our \robertaAtEnd\, and training setting follows closely the settings prescribed in \citet{liu_roberta:_2019}. 
%We choose corpora of varies sizes from different domains to study the effect of corpus size and domain (see Table \ref{tab:corpus-domain} \zeyu{Not sure why it doesn't compile here}). 
%We build on tutorial from Google\footnote{\url{https://cloud.google.com/tpu/docs/tutorials/roberta-pytorch}} and run training on a v3-8 TPU\footnote{Free usage for the public in the duration of this work} with setting specified in \ref{appendix:roberta-corpus}.
%
%

% For our experiments, we only include probes that shows, in each original paper, \roberta is superior to baseline by a noticeable margin (i.e. $>$10\% accuracy).
\paragraph{Usage} We run each probe specified below on the saved checkpoints (usually) with \roberta frozen.
\jungo{usually? Specify more here.} 
We will get a score per probe from its test set, which serves as a proxy of the tested knowledge.
Each set of probes has its own baselines due to distinct designs across probes.


% \label{sec:method:probes:linguistic}
\subsection{Downstream tasks}
\jungo{Why do we care about downstream tasks in this probing paper? Explain?}
\label{sec:method:downstream}
\paragraph{Usage} We finetune \robertaAtEnd\, checkpoints per downstream task with a linear top layer to avoid introducing too many parameters irrelevant to \robertaAtEnd's weights. Settings are detailed in \textsection \ref{appendix:downstream-setting} 

\jungo{I see. The following paragraph should be the starting statement because this is why we're talking about downstream. See my previous comment.}
By using downstream tasks, we connect diagnostic measures with some more practical contexts, which offer hints like which knowledge help the practical tasks we care more about. Another radical view is that these tasks can be seen as ``consequence-based" analyses \citep{kodner-gupta-2020-overestimation} where the model has to utilize knowledge recognized by the current probes and those to be recognized in the future. 
% Note that \roberta is trained when fine-tuning for downstream tasks while diagnostic probes keep \roberta freezed. 


Our task suite uses three representative well-known and -established tasks: \sstTwo\, --- single-sentence classification --- with accuracy of predicting the right class; \mnli\, --- sentence-pair classification --- with accuracy on matched (\mnlim) and mismatched (\mnliMm) genres; \squad\,--- extractive reading comprehension --- with predicted span measured by exact match (\squadEM) and F1 score (\squadFOne).
\jungo{Again, this is a laundry list. Describe it better?}

\subsection{$\epsilon$-Learning phases}
After we follow the instruction above, for each probing or downstream task, we will have a series of scores $S$ over the pretraining trajectory. For examples, for each \roberta checkpoint, we will have a CCG supertagging score. To quantify the notion of ``fast-to-learn" and ``slow-to-learn" for a specific task, we introduce an interval $I_{\epsilon}(S)$ called $\epsilon$-Learning phase, where $\epsilon \in [0, 0.5)$. It is calculated by $$ I_{\epsilon}(S) = \texttt{end}_\epsilon(S) - \texttt{start}_\epsilon(S)$$

$\texttt{start}_\epsilon(S)$: the first time the model achieve equal or higher than $\epsilon$ of the best probing performance in $S$

$\texttt{end}_\epsilon(S)$: the first time the model achieve equal or higher than $1-\epsilon$ of the best probing performance in $S$

With such a simple concept introduced, ``fast-to-learn" simply means the model reaches a high enough performance within a shorter interval and vice versa.\footnote{we set $\epsilon = 0.05$ in our paper. \jungo{More justification/discussion on this?}} Note this learning phase doesn't allow comparing knowledge dynamics across different trains of PTLM, e.g. CCG supertagging may achieve different max performance by using PTLMs trained on \wiki and \realnews.

\subsection{Limitation and Discussion}
\jungo{We need much more work on this.}
\label{sec:limitation}

One obvious limitation of this work is the designed probes. Although the cited probes make convincing argument for trustworthy design and are well received by the community, there are possibility for potential flaws in the probes. However, our framework is compatible with any future probes and provide insights into pretraining nonetheless.

Another limitation is using probes adds an extra layer of ``modeling" or still monitors PTLM's behavior indirectly. We suspect there can be a more direct framework that bridge neurons and ``knowledge" in the context of optimization, which might offer a more concrete way of answering what ``knowledge" means to models. We left that for future work.

no consensus in modeling (linear models MLPs etc)

\jungo{Cite the info theory Cambridge paper here?}
\jungo{Add comments on multilingual pretraining}

\zeyu{maybe yizhong has more opinion}

\jungo{Be careful here. Categorization could happen in various dimensions: task nature (linguistic, commonsense etc; methodwise (edge probing, structural probe, behavioral) I don't think the latter dimension is very useful for our purpose. So I'd suggest we delete the following paragraph.}
%Many probing tasks and methods have been developed so far. 
\textit{Behavioral} probes test the model's behavior as a language model  (e.g. whether predict word correctly; \citet{blimp-probe, lama-probe, numersense-probe, cats-probe, olmpics-probe}). Their repertoires are usually knowledge bases (e.g. ConceptNet) or carefully crafted sentence-generating templates.  The examples from those behavioral probes are then validated by crowdsource workers. The correctness is measured by whether the model chooses the sensible sentence from distractor(s). 
Contextual representation is a byproduct of current PTLM.
\jungo{It's actually the main product now.}
\textit{Structural} probes (classified in \citet{belinkov-etal-2020-interpretability-tutorial}) implemented as diagnostic classifiers test the abundance (or easeness of extraction) of linguistic knowledge in those representations \citep{nelson-probe, edge-probe}. In this case, the repertoire is chosen to be expert-annotated dataset (e.g. PenTree Bank, OntoNotes) and the abundance is measured by the accuracy of classifier.
\jungo{It's great to have some categorization of probing tasks. So this preceding section does that. But I'm not sure if crowsource vs.\ expert is a good contrast. You can ask experts to make behavioral probes as well? I need to check Belinkov's paper, but you should probably not make too many assumptions.}

==> archived/first_version/introduction.tex <==

\section{Introduction}
\label{sec:intro}

In the past few years, pretrained language models (PTLMs) such as BERT \cite{devlin_bert:_2018}, \robertaAtEnd \cite{liu_roberta:_2019}, and XLNet \cite{yang_xlnet:_2019} have become a key component of state-of-the-art neural NLP models.
Contextual representations from these PTLMs give consistent performance boosts over  uncontextualized embeddings (e.g., GloVe \citealp{pennington-etal-2014-glove}, fastText \citealp{bojanowski-etal-2017-enriching}) across various downstream tasks (e.g., SST-2 \citealp{sst2-dataset}, MNLI \citealp{mnli-dataset}, SQuAD \citealp{squad1.1-dataset}).
PTLMs are already deployed in real-world systems, such as search engines\footnote{\url{https://blog.google/products/search/search-language-understanding-bert/}} and hate speech detection.\footnote{\url{https://ai.facebook.com/blog/ai-advances-to-better-detect-hate-speech/}}
Thus, developing methods to interpret the fundamental building block of PTLMs is crucial for the accountability, trust, fairness, safety, and reliability of machine learning applications \cite{DoshiVelez2017TowardsAR, Lipton2018TheMO}.
To this end, recent papers investigated ways to explain this success and developed a surge of \textit{probing} methods in a wide range of aspects, including linguistic and factual knowledge tasks \citep{edge-probe, nelson-probe, lama-probe}.
Those works demonstrate that PTLMs achieve higher scores on their probing tasks than randomly initialized baselines and claim that PTLMs have a certain degree of the tested knowledge.
% Intuitively, the \textit{abundance} of those knowledge might \textit{account for} PTLMs' success over baselines on downstream tasks (e.g. SST-2, MNLI, SQuAD; \citet{sst2-dataset, mnli-dataset, squad1.1-dataset}). 

In this paper, we take our understanding of pretrained language models (PTLMs) one step further.
Probes are only applied to pretrained models that are obtained after an arbitrary number of parameter updates.
But what is happening during the course of pretraining?
We study the entire pretraining trajectory through our \textit{dynamic probing} framework.
This analysis offers insight into training efficiency and benefits future designing of pretraining methods.
%\jungo{Maybe discuss Tal's work on sample efficiency?}
%In advocate of \citet{PAID-position-paper},
Recent work \cite{PAID-position-paper} argued that PTLMs lack human-like generalization, and we need to reconsider their sample inefficiency compared to humans. 
Our work sheds new light on the current PTLMs' sample efficiency from the perspective of training knowledge dynamics. 
%in terms of how quickly the self-supervised model
%can conform to human knowledge.


In our dynamic probing framework, we first collect and categorize a wide and diverse set of existing probes into two major aspect of knowledge: linguistic and non-linguistic knowledge.
%Due to its long-tailed nature \zeyu{need some reasoning here or later part of paper}
We further subdivide non-linguistic knowledge into factual, commonsense, and basic reasoning knowledge (\textsection \ref{sec:method:probes}).
We introduce \textit{$\epsilon$-learning phases} (\textsection \ref{sec:3}) to quantify the notion of \textit{fast-to-learn} (\textsection \ref{sec:1}) and \textit{slow-to-learn} (\textsection \ref{sec:2}) in the pretraining trajectory.
\input{tables/tab_corpus-domain}

Our analysis reveals several interesting insights:
\begin{enumerate}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item \roberta, \footnote{\roberta denotes \roberta-BASE, if not specified otherwise.} a masked language model widely used in NLP tasks, learns linguistic knowledge within a short and early time interval during pretraining. 
    %Training on different corpus domains shows
    This linguistic knowledge dynamics can be observed regardless of the pretraining corpus domain.
    \item In contrast, factual and most commonsense knowledge is acquired incrementally as the model iterates over the dataset epoch by epoch. This slowness hints at the inefficiency of using just the masked language modeling objective in learning those types of knowledge and confirms the rationale behind recent PTLMs augumented with external knowledge sources \cite{KnowBERT, zhang-etal-2019-ernie}.
    Our controlled experiments show the training dynamics of these types of knowledge depend very much on the selection of the domain.
    \item Some basic reasoning and commonsense knowledge is not stable in \roberta. Such instability provides more concrete confirmation that \roberta does not learn the the abilities \citep{cats-probe, olmpics-probe}.
    \item When we compare our observation from probes with downstream tasks, we find that once linguistic knowledge is mastered at an early stage, the gain from pretraining (i.e., acquisition of the other knowledge) is marginal. This suggests possible early stopping to make pretraining more efficient, since we are making parameter updates for only marginal gains. This also provides evidence for the long-tailed nature of non-linguistic tasks.
\end{enumerate}



==> archived/first_version/limitation.tex <==
\section{Limitation}
\jungo{We need much more work on this.}
\label{sec:limitation}

One obvious limitation of this work is the designed probes. Although the cited probes make convincing argument for trustworthy design and are well received by the community, there are possibility for potential flaws in the probes. However, our framework is compatible with any future probes and provide insights into pretraining nonetheless.

Another limitation is using probes adds an extra layer of ``modeling" or still monitors PTLM's behavior indirectly. We suspect there can be a more direct framework that bridge neurons and ``knowledge" in the context of optimization, which might offer a more concrete way of answering what ``knowledge" means to models. We left that for future work.

\jungo{Cite the info theory Cambridge paper here?}

\zeyu{maybe yizhong has more opinion}

==> archived/first_version/question1.tex <==
\section{Fast Linguistic Learning}
\label{sec:1}
% Could we offer some hypothesis with supporting evidence that linguistic task learns fast while the other two knowledge learns slow
% Following the original probing setting, we use GloVe embedding \citep{pennington-etal-2014-glove} as our baseline. \jungo{What is the ``original probing setting"?} To quantify the ``best" \roberta can learns in the pretraining process, we use the public release of \roberta and BERT-base-cased as empirical upper bounds.

Since no explicit labeling of the data is required, self-supervised learning is a type of unsupervised learning \citep{manning-emergent-linguistic-structure}. The structural linguistic probes test the how closely information in \robertaAtEnd representations conforms to annotations developed from different linguistics theories, with probing performances as proxies.  

Our experiments show the corpus size affects the knowledge obtained --- higher probing performance from training on larger datasets. By observing that the time to reach saturation on different training data are approximately the same, the acquisition of linguistic knowledge seems like a function of gradient updates rather than the corpus size.

In most linguistic probes, regardless of corpus domains, there is a ``booming" period, where \roberta suddenly learns. In different linguistic tasks, our \roberta exceeds the empirical upperbounds to different extents (Fig \ref{fig:ling:typical}). We suspect this is due to random seed, since in original \roberta more data is included and supposedly learn better.
\jungo{Maybe cite Jesse's work on the impact of random seed.}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.23\textwidth]{figures/ling/nelson/ccg.png}
% \includegraphics[width=0.23\textwidth]{figures/ling/nelson/sem_arc_class.png}
% \caption{Knowledge dynamics observed from \ccg\, and \semClass \jungo{bigger font and plots for all figures you have in this paper.}}
% \label{fig:ling:typical}
% \end{figure}


Being ``quick and early" is not the only pattern for linguistic knowledge. A smaller portion of probing tasks differ by that the saturation time is ``slower and later" (Fig \ref{fig:ling:untypical}). We realize syntactic tasks and structured semantic task follows ``quick and early" pattern, while the sense identification task follows ``slower and later" pattern. This suggests that MLM is good at discovering syntactic labels (like POS) and hidden token-wise structure (like semantic arc) but has room for improvement in effectively learning to identify senses for tokens. 
% We suspect \robertaAtEnd's strengths come from the multi-head attention design in transformer. \zeyu{A new hypothesis}
% \jungo{How are you planning to test this hypothesis?}
\zeyu{How to add (a,b,c,d) to the figure}
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.23\textwidth]{figures/ling/nelson/conj.png}
% \includegraphics[width=0.23\textwidth]{figures/ling/nelson/ef.png}
% \caption{Knowledge dynamics observed from \ef\, and \conj}
% \label{fig:ling:untypical}
% \end{figure}

Regardless of being quick or slow and the impact from corpus size, the linguistics knowledge is less affected by domains, shown by results in \wiki v.s.\ \realnews. Also, there is no sign of catastrophic forgetting overall for linguistics despite the fluctuation. We experiment with some overlapped probing tasks between the two cited papers \citep{nelson-probe, edge-probe} and they demonstrate similar \zeyu{ knowledge dynamics}. \jungo{Hmmn, I don't get this. You are saying we see similar patterns to the ones observed by the previous works?} There are differences in saturated performance, but we suspect this stems from different probe framing. From edge probing, for more syntactic tasks, probing performance of our training usually reach those of public \roberta when saturated, while for more semantic tasks, there is a noticeable gap.
See the full (non-overlapping) results in Appendix \ref{appendix:results:probe:ling}.

==> archived/first_version/question2.tex <==
\section{Slow Non-Linguistic Learning}
% \jungo{Maybe combine this and the preceding section? Also we need to explain the $\epsilon$ method earlier.}
% \label{sec:2}
% Since non-linguistic probes test PTLMs' behavior on different inputs as a language model, we can't use off-the-shelf embeddings to set the baseline. Instead, for the best and a simple illustration, we simply set the baseline performance as the expected accuracy by random guesses. We also closely follow the original settings. 
% \jungo{So this section is for describing a random baseline?}

\subsection{Still Learnable Knowledge}

\paragraph{Factual} We observe \roberta learns factual knowledge slowly (if it ever learns) --- much longer time taken to saturate --- and the stronger impact of domain than on linguistic knowledge --- \roberta trained on \bookcorpus barely learns any factual knowledge tested. And the (relatively) superior \lamaGoogle\, performance of \roberta trained on \wiki (Fig.\ \ref{fig:factual:all}) further supports the importance of the domain choice, because \wiki contains lots of bibliography information explicitly (e.g., the date of birth) \jungo{bibliography? biography?} while \realnews doesn't \zeyu{Just my impression}. \jungo{This is definitely true, isn't it?} Despite occasional large fluctuation, the performance increases.
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.47\textwidth]{figures/factual/lama/linear_xscale.png}
% \caption{Knowledge dynamics observed from \lama.}
% \label{fig:factual:all}
% \end{figure}

\paragraph{Commonsense} Commonsense knowledge is similar to factual in speed to saturation, while the impact from domain is little (see Fig \ref{fig:comm:all}, \cat, \wiki v.s. \realnews). Thus, it seems reasonable to conclude the commonsense knowledge is domain-agnostic but affected by the corpus size. By observation from \numer, corpus size hinders the learning and stable storage of numerical commonsense knowledge. For the task that public \roberta barely surpasses random guess --- \catArctOne\, and \catArctTwo, the dynamics is very unstable, which confirms the original conclusion that PTLM is weak in those tests by our premise 2 (stability of probing performance).
% lower performance on \bookcorpus is due to the data size. 


% \begin{figure}[h]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/commonsense/cats/all.png}
% \includegraphics[width=0.47\textwidth]{figures/commonsense/numer/acc@1.png}
% \caption{Knowledge dynamics observed from \cat\, and \numer.}
% \label{fig:comm:all}
% \end{figure}

\subsection{(Nearly) Unlearnable Knowledge}

\paragraph{Basic reasoning} Our dynamics on basic reasoning knowledge fails in most of the tasks either by low performance or instability, and only shows seeming success in \olmpicsTaxonomy, \olmpicsAntonym, \olmpicsAlways. However, if we look at the three probes more carefully, we realize a suspicious phenomenon that  \olmpicsAntonym\, and \olmpicsAlways\, yield high performance in the very beginning. We suspect such early success potentially comes from the fine-tuning the top language model head. 
\jungo{As far as I know, `language model head' isn't a widely used term in the community. Rephrase?}
To confirm our hypothesis, we test without finetuning and found \roberta barely exceeds random guess over time. \zeyu{experiments TBDone}. This is a clear sign that the masked language modeling objective or transformer's design capture little ability for basic reasoning. We suspect this will be the case for all MLM language models, if they were probed from a dynamics perspective.
\jungo{A better claim can be: since the primary objective of many pretrained models are all masked language modeling \cite{devlin_bert:_2018}, albert etc, we suspect this will be the case for those models.}
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/reasoning/olmpics/linear.png}
% \caption{Knowledge dynamics observed from \cat\, and \numer.}
% \label{fig:comm:all}
% \end{figure}
% \include{tables/tab_learning_patterns}
% Question when studying tension between memorization and generalization, what's the dynamic of this tension?:
% \begin{itemize}
%     \item \textbf{Objective measure:} Similarity (by model-agnostic measure e.g. td-idf) between probe examples and training examples?
%     \item \textbf{Subjective measures:} Is there any easy examples and hard examples memorized by \textbf{the model}? The evidence for generalization is: if there is a set of easy examples (measures by ppl), does the model has small ppl (in validation set) for the nearest neighbours (by various metric) of this set of easy examples?
%     \item parallel with the child language acquisition
% \end{itemize}

==> archived/first_version/question3.tex <==
\section{Practical implication}
\label{sec:3}

We calculate the learning phases of all learnable knowledge (i.e. \olmpics\, excluded). 
\jungo{learnable knowledge is not well defined.}
For discussion, we also do it for the dynamics of downstream tasks performance and MLM loss on validation set (Fig.\ \ref{fig:learningphase:all}).


The learning phases show that there is a clear boundary between where more than a half of linguistic knowledge learns well, and where more than half of commonsense knowledge learns well. However, the boundary for factual is blurry. Another observation is that the MLM loss tells nothing about how the models learns knowledge, since we observe it drops rapidly within first epoch and slowly decrease (basically flatten) from then on. 

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/learning_phases/eps0.03_learning_phases_mix_sortByEnd.png}
% \caption{$\epsilon$-learning phases of all tested knowledge, downstream tasks, and MLM loss on validation set}
% \label{fig:learningphase:all}
% \end{figure}

\jungo{I'm not sure about this. Can we claim it's causation rather than correlation?}
Another critical implication is that linguistic knowledge mainly contribute to the downstream tasks (their dynamics are similar in shape as well); this rationalize the previous focus on interpreting linguistic knowledge in models. The impact from non-linguistic knowledge seems marginal. However, when we try to observe the dynamics on commonsenseQA \zeyu{TBDone}, the usefulness of non-linguistic knowledge is emphasized.

% \zeyu{How does our results shows there are still knowledge undiscovered?}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/finetune/all.png}
% \caption{Dynamics of performance on downstream tasks}
% \label{fig:finetun:all}
% \end{figure}

==> archived/first_version/related.tex <==
\section{Related Work}
\paragraph{Training dynamics of language models}
\jungo{self-note: cite Rumelhart's past tense work}
Early work \cite{} observed the dynamics in a feedforward neural network to assess the cognitive plausibility of a connectionist model. They focused on the case of past tense acquisition and observed similar staged learning in the distributed representations from a neural network.
To the best of our knowledge, \citet{dynamics-by-svcca} is the closest to our work. \jungo{what makes it closets?} However, they studied the recurrent-based Long Short-Term Memory (LSTM) LM, while we studied the feedforward-based \jungo{attention-based, rather?} transformer LM. 
\jungo{I don't think this should be most critical difference. LSTM vs.\ transformer isn't really our main focus, and it's possible the same methods or even arguments hold for both. The difference is our rich probing suite and focus on many different aspects of pretrained models.}
Our work allows the use of probe classifier since the encoded feature by a transformer may be more easily interpreted by a linear classifier than the ones by LSTMs \citep{dynamics-by-svcca}. Also, their work make use of separate tag-specific LSTM networks to correlate LSTM LM, while ours study solely the trained LM. Moreover, the wide range of probing literature based on BERT-like LMs offer us the special advantage to study LM from a broad knowledge acquisition perspective, while \citet{dynamics-by-svcca} can only focus on linguistic perspective and study the correlation between .
\jungo{Right. You wrote the most importance different in the final sentence...}


\paragraph{Dynamics over layers} Given the state of the model at a time step (e.g. final state), \citet{dynamics-by-layers} study the view the evolution of a token representation between layers from the compression/prediction trade-off perspective with different training objectives. Therefore, compared with our work, this view of PTLMs is static. However, interestingly, their conclusion further supports our choice of MLM over LM due to the superior performance \jungo{performance on what? downstream tasks like QA? Probe results?} of the MLM objective over the standard left-to-right LM pretraining objective, and studying the superior one may provide more insights into a more efficient pretraining algorithm.




==> archived/old_files/2_background.tex <==
% \section{Background: Probes as Proxies for Encoded Knowledge}
% \label{sec:background}
% \hanna{The overall story is a bit unclear at this point; I recommend re-structuring this section as an overview and background; It includes the overall description of probes; the construction of your probe; the big picture of knowledge that you are probing and listing the three questions. Here, you should kind of prepare an outline of the work. Especially right now sections 5 and 6 come out of place; it is important to position them in this overview section. }


% \hanna{I would give a title to each paragraph here; for example this paragraph would be "Control Baselines"}  
% \zeyu{We break this section and blend it to section \ref{sec:probing_across_time}}





% \textit{Why do pretrained language models work so well in so many tasks?}
Since the success of large-scale pretraining \cite{elmo, devlin_bert:_2018}, this fundamental question has inspired a flurry of recent papers that analyze and interpret pretrained language models (PTLMs) in various aspects of natural language, including syntax \cite{blevins-etal-2018-deep, hewitt-manning-2019-structural}, semantics \cite{nelson-probe}, and commonsense knowledge \cite{da-kasai-2019-cracking, lama-probe}.
These analysis papers measure the degree to which contextual representations from PTLMs encode different types of information by evaluating on targeted \textit{probing} tasks.
While a wide range of probing tasks have recently been proposed \cite{belinkov-etal-2020-interpretability-tutorial}, almost all the probes are assumed to be static up until now: probing is only applied to publicly available pretrained models that are obtained after an arbitrary number of updates.
But what is happening in the course of the parameter updates? Do we really need so many update steps that make it virtually impossible to pretrain competitive language models from scratch in a standard academic environment?
% Can we make pretraining more efficient?

We fill this gap in the probing literature by developing a dynamic probing framework. In particular, we apply a rich suite of probes over the course of pretraining a masked language model, \roberta, and analyze how the probing performance progresses over time.
% Our extensive observations contribute to the large body of work that investigates why PTLMs substantially improve downstream performance.

% \subsection{Two types of probes}
% \paragraph{Classifier Probes}  % Classifier probes 
% (also coined ``structural probes" in \citet{belinkov-etal-2020-interpretability-tutorial}) build a classifier that predicts some annotations on top of contextual representations from a PTLM. This type of probes was widely used to test linguistic knowledge.

% For examples, in Part-of-Speech tagging, each word $w$ will be represented as a vector $\bm{x}_w$, either using precomputed embedding like GloVe \citep{pennington-etal-2014-glove} or PTLM. A classifier $f(\bm{x}_w)$ will be trained on annotated dataset (e.g. PennTree Bank) to predict its correct PoS tag $y_w$.

% Using insights from \citet{hewitt-probe-control}, we choose a linear model for our classifier for lower model complexity and selectivity --- lower difference in accuracies between training on gold annotations and training on ``shuffled" annotations.

% In our work, to account for intermediate representations, we use contextual representations from all the layers $$[\bm{x}_w^{(0)}, \cdots, \bm{x}_w^{(\ell)}, \cdots, \bm{x}_w^{(L)}]$$ to train the classifier. To reduce the amount of experiments, we follow \citet{nelson-probe} and use learnable parameters $\bm{\alpha}$ to perform a weighted sum to get our input for classifier, i.e. 
% $$\bm{x}_w = \sum_{i=0}^L \bm{x}_w^{(\ell)} \cdot \bm{\alpha}^{(l)}.$$
% In structural probe designs \jungo{not sure how we should call Nelson's method as opposed to edge probing. Structural probes are probably coined by Hewitt Manning.}, the classifier receives one or optionally two representation(s) and train to predict a label such as a constituent or relation type; in \edge, the representation is from a span of tokens, while, in \cwr, the representation comes from a token. \textbf{Metric:} The accuracy is determined by whether the classifier predict the label correctly.

% \paragraph{Behavioral Probes} % Behavioral probse,
% %Our linguistic probes includes structural probes --- \cwr\,(Contextual Word Representation; \citet{nelson-probe}) and \edge\,(Edge Probing; \citet{edge-probe}) --- and behaviors probes --- \blimp\, (Benchmark of Linguistic Minimal Pairs; \citet{blimp-probe}).
% , on the other hand, ignore the representation from PTLM and assess the \textit{behavior} of PTLM as a language model on a challenge set. The behavior of the PTLM includes but not limited to: \textbf{i) Fill-in [MASK]:} whether PTLM correctly predicts or ranks, based on probability, a masked word in its context (e.g. ``Albert Einstein was born in [MASK]"); \textbf{ii) Comparing sentence scores:} given some scoring method based on probability (e.g. \citet{salazar-etal-2020-masked}), whether PTLM can score the more or most ``sensible" sentence from the distractor(s). See more detailed illustrations in Table \ref{tab:examples-main}.
% \blimp\, consists of 67 individual datasets (12 tested phenomena), each containing 1,000 minimal pairs, i.e. pairs of minimally different sentences that contrast in grammatical acceptability and isolate specific phenomenon in syntax, morphology, or semantics. Each test contains minimal pair of sentences. \textbf{Metric:} we determined the correctness by whether PTLM assigns higher probability to the the grammatical token given the context.


%accurate a pretrained language model can get on a set of examples constructed by using some knowledge repertoires.
%This is indicative of how closely the model conforms to human understanding of the world because those knowledge sources i) were constructed \textit{independently} of training the probed model and ii) intend to best reflect human knowledge --- linguistic (e.g., PennTree Bank) or non-linguistic (e.g., ConceptNet) \jungo{citation}. In other words, the test does not depend on the prior about any model but on the desired outcome from a learning process (i.e., training the model). In our case, this leads to a very simple yet crucial premise for probing PTLM: 

%\textit{The performances of designed probes reflect the ability of a PTLM at any stage of training}.


%To the best of our knowledge, this straightforward premise is surprisingly unspoken at time of previous probe designs \cite{kohn-2015-whats,  cooper-1996-early-behavioral-probe} \zeyu{both are from \citet{belinkov-etal-2020-interpretability-tutorial}; first is earliest structural probe, second is earliest behavioral; no permission to read the last, judge from abstract}. However, we believe this premise has to hold and already drives the probe designs for years. Our work utilizes this premise to advance our understanding of PTLMs.











==> archived/old_files/background-first.tex <==
\section{Background}

\subsection{Pretraining}

Since ELMo \citep{elmo} was proposed, there is a trend in the learning of most NLP systems that consists of three stages: (1) pretraining of a word prediction model on a corpus of arbitrary size; (2) fine-tuning (transfer learning) on a training set representing a classification task; (3) evaluation on a test set drawn from the same distribution as that training set \citep{PAID-position-paper}. \zeyu{I just copy abstract of PAID}

One well-known PTLM is \roberta \citep{liu_roberta:_2019} --- an improvement of transformer-based Masked Language Model over its predecessor, BERT \citep{devlin_bert:_2018}. During learning, it is self-supervised with a masked language modeling objective (i.e., cross-entropy loss on predicting randomly masked tokens). The unlabeled pretraining corpus for \roberta contains over 160 GB of uncompressed raw text from different English-language corpora (see Appendix \textsection \ref{appendix:roberta-corpus}) \citep{gururangan-etal-2020-dont}. Different from BERT, it does not have the Next Sentence Prediction objective which \citet{liu_roberta:_2019} empirically shows to be harmful for learning. \zeyu{I basically copy Don't Stop Pretraining}

 We use \roberta as the starting point for investigating the knowledge acquisition because: (i) it was trained with a pure language model objective, and (ii) compared with pretraining procedures like XLNet and SpanBERT \citep{yang_xlnet:_2019, SpanBERT}, it has closer connection to how conventional neural language models are trained, and (iii) most of knowledge probes were developed based-on it, and (iv) compared with GPT-$n$ ($n$ $=$ $1,2,3$) \citep{gpt2, gpt3} \zeyu{Does gpt3 follow the same training procedure as gpt2?}, it is only directly trained on a small portion of its vocabulary set (e.g. 15\% of the tokens in the corpus are masked), so it leaves more room for the interesting debate on ``generalization v.s. memorization". \zeyu{I think point (iv) is clever lol, never realized I can make that connection}
 
\zeyu{I basically follows the structure of Don't Stop Pretraining}

% In various interpretability papers \cite{olmpics-probe, numersense-probe}, it is widely observed that \roberta contains more knowledge than BERT. Also, \roberta offers more performance boost in downstream tasks than BERT \cite{liu_roberta:_2019}.
\subsection{Probes}
Due to the black-box nature of recent end-to-end learning systems, different analysis tools were proposed for a better understanding, accountability, and interpretability of those models  \citep{belinkov-etal-2020-interpretability}. Arguably, the most famous ones are ``probes". In this paper, ``probes" includes ``structural analysis" and ``behavioral analysis" as categorized in  \citet{belinkov-etal-2020-interpretability}, which we call structural probes and behavioral probes respectively. \zeyu{Better to ground the meaning of the terms} 

In formula, the studied model is a function $f: x \rightarrow y$ that maps an input $x$ to an output $y$. $f$ might be a complicated neural network with many layers or other components. In this paper, we use $f = \robertaAtEnd$. The used \roberta includes $L=$ 12 transformer layers, tokenizer, and optionally requires the language model head for behavioral probes. $x$ is the sub-word token in string for both probes, while $y$ varies for different probes. 

%  (\textsection \ref{sec:structural-probes}) 
%   (\textsection \ref{sec:behavioral-probes}) 

\zeyu{Below, I basically rephrase the slide of \href{https://sebastiangehrmann.com/assets/files/acl_2020_interpretability_tutorial.pdf}{ACL 2020 interpretability tutorials}}

% \label{sec:structural-probes}
\textbf{Structural Probes} have $y$ to be the final contextual embedding from \robertaAtEnd. They are usually implemented by a classifier for linguistic knowledge where theoretically supported human annotations $z$ can be made (e.g. Part-of-Speech tagging). To investigate part of the model, we use $f^{\ell}(x)$, the contextual embedding of the network at the $\ell$-th layer. Then, we train a classifier $g: f^{\ell}(x) \rightarrow z$ that maps the representations to the annotations $z$, and get the optimized classifier $g^*$. For selectivity, the probe should be as simple as possible \citep{hewitt-probe-control}. The accuracy of $g^*$ serves as a proxy to the quality of representations $f^{\ell}(x)$ w.r.t. $z$, human knowledge about language. In information theoretic terms, $g^*$ maximize the mutual information between $f^{\ell}(x)$ and $z$.

Given a linguistic annotation $z$, we train a classifier $g\left(\sum_{\ell=0}^L \alpha^{(\ell)} f^{\ell}(x)\right) = z$. To save computations and still compare the importance of different layers, our design choices are (i) $\alpha^{(\ell)} $ is a parameter that was jointly learned with the parameter of classifier $g$, and (ii) $\ell \in \{0,1,2 \cdots 12\}$, where $f^{0}$ is the embedding lookup table, and $f^{12}$ is the final contextual representation of \robertaAtEnd.

\zeyu{Below, the slide is not working very well for our cases, so I need to thinking of some way to talk about our probes in some general terms and detail in \ref{sec:methods}}

% \label{sec:behavioral-probes}
\textbf{Behavioral Probes} have $y$ to be a set $S$. In general, the probes measure the average-case performance of the studied model on $S$. $S$ can be a set of words or a set of sentences in different probes. The probes measures whether the model ranks the correct element among the top $K$ choices (Precision at $K$) by using probability for words or probability-based scores for sentences. We will specify details in \textsection \ref{sec:diagnostic-probes}. This kind of probes rewards models for performing well on common phenomena, and could hide the fact that they perform poorly on “the tail”. However, challenge sets can be proposed to cover specific, diverse phenomena so that this kinds of probes facilitate fine-grained analysis of model performance. This diagnostic probes have a long history \cite{TSNLP, using-the-framework}.


==> archived/old_files/background.tex <==
\section{Background}
\label{sec:background}
\subsection{Pretraining and Perplexity}

Since ELMo \citep{elmo} was proposed, there is a trend in the learning of most NLP systems that consists of three stages: (1) pretraining of a word prediction model on a corpus of arbitrary size; (2) fine-tuning (transfer learning) on a training set representing a classification task; (3) evaluation on a test set drawn from the same distribution as that training set \citep{PAID-position-paper}. \zeyu{I just copy abstract of PAID}

One well-known PTLM is \roberta \citep{liu_roberta:_2019} --- an improvement of transformer-based Masked Language Model over its predecessor, BERT \citep{devlin_bert:_2018}. During learning, it is self-supervised with a masked language modeling objective (i.e., cross-entropy loss on predicting randomly masked tokens). The unlabeled pretraining corpus for \roberta contains over 160 GB of uncompressed raw text from different English-language corpora (see Appendix \textsection \ref{appendix:roberta-corpus}) \citep{gururangan-etal-2020-dont}. Different from BERT, it does not have the Next Sentence Prediction objective which \citet{liu_roberta:_2019} empirically shows to be harmful for learning. \zeyu{I basically copy Don't Stop Pretraining}

 We use \roberta as the starting point for investigating the knowledge acquisition because: (i) it was trained with a pure language model objective, and (ii) compared with pretraining procedures like XLNet and SpanBERT \citep{yang_xlnet:_2019, SpanBERT}, it has closer connection to how conventional neural language models are trained, and (iii) most of knowledge probes were developed based-on it, and (iv) compared with GPT-$n$ ($n$ $=$ $1,2,3$) \citep{gpt2, gpt3} \zeyu{Does gpt3 follow the same training procedure as gpt2?}, it is only directly trained on a small portion of its vocabulary set (e.g. 15\% of the tokens in the corpus are masked), so it leaves more room for the interesting debate on ``generalization v.s. memorization". \zeyu{I think point (iv) is clever lol, never realized I can make that connection}
 
\zeyu{I basically follows the structure of Don't Stop Pretraining}

% In various interpretability papers \cite{olmpics-probe, numersense-probe}, it is widely observed that \roberta contains more knowledge than BERT. Also, \roberta offers more performance boost in downstream tasks than BERT \cite{liu_roberta:_2019}.
\subsection{Probes}
Due to the black-box nature of recent end-to-end learning systems, different analysis tools were proposed for a better understanding, accountability, and interpretability of those models  \citep{belinkov-etal-2020-interpretability-tutorial}. Arguably, the most famous ones are ``probes". In this paper, ``probes" includes ``structural analysis" and ``behavioral analysis" as categorized in  \citet{belinkov-etal-2020-interpretability-tutorial}, which we call structural probes and behavioral probes respectively. \zeyu{Better to ground the meaning of the terms} 

In formula, the studied model is a function $f: x \rightarrow y$ that maps an input $x$ to an output $y$. $f$ might be a complicated neural network with many layers or other components. In this paper, we use $f = \robertaAtEnd$. The used \roberta includes $L=$ 12 transformer layers, tokenizer, and optionally requires the language model head for behavioral probes. $x$ is the sub-word token in string for both probes, while $y$ varies for different probes. 

%  (\textsection \ref{sec:structural-probes}) 
%   (\textsection \ref{sec:behavioral-probes}) 

% \zeyu{Below, I basically rephrase the slide of \href{https://sebastiangehrmann.com/assets/files/acl_2020_interpretability_tutorial.pdf}{ACL 2020 interpretability tutorials}}

% \label{sec:structural-probes}
\textbf{Structural Probes} have $y$ to be the final contextual embedding from \robertaAtEnd. They are usually implemented by a classifier for linguistic knowledge where theoretically supported human annotations $z$ can be made (e.g. Part-of-Speech tagging). To investigate part of the model, we use $f^{\ell}(x)$, the contextual embedding of the network at the $\ell$-th layer. Then, we train a classifier $g: f^{\ell}(x) \rightarrow z$ that maps the representations to the annotations $z$, and get the optimized classifier $g^*$. For selectivity, the probe should be as simple as possible \citep{hewitt-probe-control}. The accuracy of $g^*$ serves as a proxy to the quality of representations $f^{\ell}(x)$ w.r.t. $z$, human knowledge about language. In information theoretic terms, $g^*$ maximize the mutual information between $f^{\ell}(x)$ and $z$.

Given a linguistic annotation $z$, we train a classifier $g\left(\sum_{\ell=0}^L \alpha^{(\ell)} f^{\ell}(x)\right) = z$. To save computations and still compare the importance of different layers, our design choices are (i) $\alpha^{(\ell)} $ is a parameter that was jointly learned with the parameter of classifier $g$, and (ii) $\ell \in \{0,1,2 \cdots 12\}$, where $f^{0}$ is the embedding lookup table, and $f^{12}$ is the final contextual representation of \robertaAtEnd.

% \zeyu{Below, the slide is not working very well for our cases, so I need to thinking of some way to talk about our probes in some general terms and detail in \ref{sec:methods}}

% \label{sec:behavioral-probes}
\textbf{Behavioral Probes} have $y$ to be a set $S$. In general, the probes measure the average-case performance of the studied model on $S$. $S$ can be a set of words or a set of sentences in different probes. The probes measures whether the model ranks the correct element among the top $K$ choices (Precision at $K$) by using probability for words or probability-based scores for sentences. We will specify details in \textsection \ref{sec:diagnostic-probes}. This kind of probes rewards models for performing well on common phenomena, and could hide the fact that they perform poorly on “the tail”. However, challenge sets can be proposed to cover specific, diverse phenomena so that this kinds of probes facilitate fine-grained analysis of model performance. This diagnostic probes have a long history \cite{TSNLP, using-the-framework}.
\input{tables/tab_corpus-domain}

==> archived/old_files/experiments-first.tex <==
\section{Experiments}
\zeyu{Yizhong may want to help here}
\subsection{Pretrained Language Model}
% \subsection{Knowledge Probes}
% \input{tables/tab_corpus-domain}
Our LM pretraining follows the settings prescribed for training \roberta as much as possible and we build on tutorial from Google\footnote{\url{https://cloud.google.com/tpu/docs/tutorials/roberta-pytorch}}. To study the effect of domain, each training is run on a v3-8 TPU with the same settings which are specified in \ref{appendix:roberta-corpus}.

% \subsection{Learning dynamics of different types of knowledge}

% \subsection{Which layers learn the knowledge best?}

% \subsection{Does the model forget?}
% We can compare the correct subsets of the probing examples at different checkpoints, and show the number / proportion of flips. \citep{toneva_empirical_2018}

% \subsection{Learning $=$ memorizing ?} 

% \textbf{Reasoning? }

% \textbf{Seemingly more interesting }

% ``apple" appears near ``fruit" in the training ?

% pair-wise coref      

% If one word/phrase is seen in training, is it more likely to be linked in conference (I think Nikos referes to some Coref downstream task)?

% don't stop pretraining -- only do one epoch --- memorizing?





% If the model learns some factual knowledge at some point, we want to investigate the training data it sees, and see if it's correlated or not. What kind of generalization happens?

% How about linguistic knowledge? Maybe we can show the model learns consistent linguistic knowledge even though the pretraining data is different? See the next subsection.

% \subsection{Comparing Domains of Pretraining Data}
% Wikipedia corpus v.s. bookcorpus

==> archived/old_files/experiments.tex <==
\section{Method}
\label{sec:exp}
\subsection{Pretraining}
\label{sec:exp:pretraining}
Our PTLM follows the settings prescribed for training \roberta as much as possible and we build on tutorial from Google\footnote{\url{https://cloud.google.com/tpu/docs/tutorials/roberta-pytorch}}. To study the effect of domain, each training is run on a v3-8 TPU with the same settings specified in \ref{appendix:roberta-corpus}. 
\input{tables/tab_corpus-domain}
\subsection{Probing tasks}
\label{sec:exp:probes}
Due to the space limit, we left all the examples for each probing tasks in \textsection \ref{appendix:probe-examples}.
\label{sec:linguistic-probes}
\paragraph{Linguistic probes} To maximize the coverage of linguistic ability, we use non-overlapping probes from \citet{nelson-probe} (\cwr\textbf{-}) and \citet{edge-probe}(\edge\textbf{-}). Linguistics probes are all chosen to be structural probes, implemented by a diagnostic classifier \citep{belinkov-etal-2020-interpretability-tutorial}. Using insights from \citet{hewitt-probe-control}, we choose linear model for our classifier for better selectivity. In both probe designs, the classifier receives one or optionally two representation(s) and train to predict a label such as a constituent or relation type; in \citet{edge-probe}, the representation is from a span of tokens, while, in \citet{nelson-probe}, the representation comes from a token. 

Our linguistic probing suite includes use labeling tasks: Part-of-speech tagging (\PTBpos, \EWTpos; constructed from the PennTreeBank and the English Web Treebank); Named Entity Recognition (\ner); CCG supertagging (\ccg); Syntactic Chunking (\chunk); Grammatical Error Detection (\ged); Conjunct Identification (\conj); Event Factuality (\ef); Preposition Supersense Disambiguation for lexical semantic function (\psFxn) and the semantic role or relation it mediates (\psRole); similar to part-of-speech tagging, Syntactic Dependency Arc Prediction and Classification task on PTB and EWT (\PTBsynPred, \PTBsynClass, \EWTsynPred, \EWTsynClass); Coreference Arc Prediction (\coref); Semantic Role Labeling (\srl); Semantic Proto-Role Labeling, constructed using PTB (\PTBspr) and EWT (\EWTspr); Relation Classification (\rel)
% two tokens --- $w_{head}$  as 
% $w_{mod}$ as 

% we use the DELPH-IN MRS-Derived Semantic Dependencies (DM) target representation from the SemEval 2015 shared task \citep{semeval-2015-task-dataset} and
% with the DELPH-IN MRS-Derived Semantic Dependencies (DM) target representation. The probe is trained


\subsection{Downstream tasks}
\label{sec:exp:downstream}



==> archived/old_files/future.tex <==
\section{Future work}

==> archived/old_files/introduction-first.tex <==
\section{Introduction}

% Recently, researchers have found that pretraining Language Model (LM) on a large corpus helps the language model to learn ``good'' representations for tokens (word, sub-word, etc.). The most famous of all includes ELMo, BERT, RoBERTa, and GPT-$n$ ($n=1,2,3$). They work as powerful off-the-shelf contextual embedders in place of the non-contextual word type embeddings such as GloVe \jungo{TODO: cite papers}. However, those embedders are utilized as a black-box and it is hard to understand why using them will give performance boost on downstream tasks. 

% This source of confusion gave rise to a line of work to probe those pretrained language models for attributing the models' success or simply understanding the model. However, the subjects been investigated in those paper are all officially released models. Although those important investigations lead to the conclusion that the final Pre-Trained Language Models (PTLMs) \textit{acquired} those three types of knowledge, there are still many interesting and important questions left unanswered. For example,
% \begin{enumerate}
%     \item What is the \textit{acquisition process} of knowledge during pretraining?
%     \item What is the \textit{knowledge distribution} within PTLMs during pretraining?
%     \item Is there any \textit{learning curriculum} that PTLMs follow ? If so, \textit{what} is it?
%     \item Is there any \textit{catastrophic forgetting} during pretraining? If so, \textit{what} is forgotten?
%     \item Is the knowledge acquisition affected by the \textit{corpus domain} on which PTLMs are trained?
% \end{enumerate}

% In this paper, we present the first work to scrutinize the learning dynamics of PTLMs during pretraining and investigate the learning procedure with finer granularity. We believe answering those questions would shed light on the learning dynamics of PTLM and help researchers design better algorithms and models to increase data efficiency \cite{linzen_how_2020}.

% Due to the philosophical difficulties to define knowledge, we utilize a wide range of probes as proxies to classify and quantify the knowledge learned. Specifically, we classify three types of knowledge the final PTLMs possess: linguistic (LING), factual (FA), commonsense (COM). To assist deeper investigation into PTLM and future research, we also publish our pretraining checkpoints\footnote{\url{tbd}} and code-base\footnote{\url{tbd}}

% current stage of PTLM and interpretability work
In the past few years, \textbf{P}re-\textbf{T}rained \textbf{L}anguage \textbf{M}odels (PTLMs) have became a key component of state-of-the-art neural NLP models \citep{liu_roberta:_2019, devlin_bert:_2018, yang_xlnet:_2019}. Contextual word representations produced by those PTLMs are extraordinarily effective—using them in place of traditional static word vectors within the latest models leads to large gains across a variety of NLP tasks\citep{nelson-probe}.  When designing large-scale pretraining, people have the intuition that the model will \textit{acquire} ``knowledge" when the model iterate over the corpus \zeyu{can we find support from any paper?}. However, the success of those trained models remains a mystery. 

To attribute the success of PTLMs, recent work has developed a series of ``probes" and showed that PTLMs exhibit surprising extent of knowledge, e.g. \citep{nelson-probe, edge-probe}, factual \citep{lama-probe}, and commonsense \cite{cats-probe, numersense-probe}, reasoning \citep{olmpics-probe}. Intuitively, the containment of those knowledge might explain PTLMs' success and be useful for downstream tasks (e.g. closed-book question answering). 

% given the current status, what's more to be done. 

Those probes prove the \textit{existence} of knowledge. However, the knowledge acquisition during pretraining --- how the knowledge turns from \textit{non-existence} to \textit{existence} --- still remains a black-box procedure.

\todo{We might need a schematic graph on first page to give intuitive explanation}

Meanwhile, even more pretraining models and procedures are proposed for different purpose --- Question Answering \citep{SpanBERT} or Relationship Extraction \citep{KnowBERT} \zeyu{not sure about this}. Therefore, we believe understanding this knowledge acquisition process will offer a more general guidance to design more useful and efficient pretraining algorithms in the future. In the long run, understanding this will help drive our NLP system towards human-like generalization partially described in \citet{PAID-position-paper}. Towards that end goal, we investigate the learning dynamic of knowledge acquisition during pretraining and the textual effect on knowledge acquisition. To the best of our knowledge, we are the first paper to do so for PTLMs from a knowledge perspectives.
In this work, we ask and answer:
\begin{enumerate}
    \item Do different types of knowledge in PTLM follow the same \textit{learning curriculum}? (\textsection \ref{sec:q1})
    \item During learning, is the model generalizing or memorizing knowledge? (\textsection \ref{sec:q2})
    \item Given PTLM learns ``good enough" diagnostically, how much practical meaning does it have ? (\textsection \ref{sec:q3})
\end{enumerate}
\zeyu{Even though, we break down the question into sub-parts, we might not use all knowledge probes to answer each question due to the nature of probes}

% Brief summary of our methodology
In this work, we address those questions for one such high-performance model, \roberta\footnote{In this paper, \roberta refers to \robertaAtEnd-BASE in \citet{liu_roberta:_2019}} under various training configuration. For each train, we first save checkpoints with different granularity and then run massive analysis tools on all checkpoints. Our analysis tools include (i) diagnostic probes and (ii) downstream tasks. The diagnostic suite includes probes for three knowledge types: (a) linguistic, (b) factual, and (c) commonsense. We use structural probes for linguistic knowledge and behavioral probes for factual and commonsense knowledge \citep{belinkov-etal-2020-interpretability}. Such design choice is due to the current status of interpretability research. Our downstream suite includes tasks that are deemed to require different kinds of knowledge \zeyu{any support from paper? I know those tasks are used in Roberta} such as SST-2 \citep{sst2-dataset}, MNLI \citep{mnli-dataset}, SQuaD \citep{squad1.1-dataset}. 

% Brief summary of our conclusion
Our analysis reveals interesting insights such as: \zeyu{some of those still wait to be confirmed}
\begin{itemize}
    \item There is a ``tipping point" moment when learning linguistic knowledge, while factual and commonsense knowledge learns epoch by epoch. Most of linguistic knowledge and all commonsense knowledge are domain-agnostic, while part of linguistic knowledge and factual knowledge are very domain-dependent. 
    \item Over all states we checked, PTLM learns all knowledge both by generalization and memorization. Memorization dominates the learning process of commonsense and factual knowledge, while generalization dominates that of linguistic knowledge. \zeyu{I think our in-depth analysis in linguistic knowledge can support this. Hopefully, we can find PTLM's embedding learns linguistic notations (e.g. CCG, Dep) hierarchically since the model figure out the unobserved notation unsupervisedly}. 
    \item Our investigation shows that there is a long-tail effect of factual and commonsense knowledge on downstream tasks. Since our linguistic diagnostics shows that the learned linguistic knowledge quickly saturate the model, seemingly, effect of linguistic knowledge on downstream tasks is one-time.
\end{itemize}

We make our code and checkpoints for pretrained model publicly available for future investigation in knowledge acquisition.

\zeyu{We might  need some hypothesis in some previous work that our experiments can demystify. Those can be the takeaway from our paper. see \ref{sec:wrong-hypothesis}}

==> archived/old_files/introduction-fourth.tex <==
\zeyu{correlate the obseravtion and previous papers, and why our finding is exciting. Most of ling probes, emphasize on easy learning.}

\section{Introduction}
\label{sec:intro}
In the past few years, pretrained language models (PTLMs) such as BERT \cite{devlin_bert:_2018}, \robertaAtEnd \cite{liu_roberta:_2019}, and XLNet \cite{yang_xlnet:_2019} have become a key component of state-of-the-art neural NLP models.
Using these contextualized representations from PTLMs instead of uncontextualized embeddings (e.g., GloVe \cite{pennington-etal-2014-glove}, fastText \cite{bojanowski-etal-2017-enriching}) gives consistent performance boost across various downstream tasks (e.g., SST-2 \cite{sst2-dataset}, MNLI \cite{mnli-dataset}, SQuAD \cite{squad1.1-dataset}).
However, the reason for such success is unknown, which inspired a surge of probes.
\jungo{``The" reason seems too strong. There's probably many reasons. So say something like ``for this reason, recent papers investigated reasons for the success and developed a surge of \textit{probing} methods?"}
In those works, by demonstrating that PTLMs achieve higher scores on their defined linguistic probing tasks, they show that PTLMs ``contain more knowledge" about $\mathcal{X}$ than their chosen baselines, where $\mathcal{X} \in \{\text{Part-of-Speech, Syntactic Dependency,} \cdots \}$ \citep{nelson-probe, edge-probe}. 
% Intuitively, the \textit{abundance} of those knowledge might \textit{account for} PTLMs' success over baselines on downstream tasks (e.g. SST-2, MNLI, SQuAD; \citet{sst2-dataset, mnli-dataset, squad1.1-dataset}). 

For all probes, we realize \jungo{Hmmn no one has really done dynamic probing right? So maybe our proposal?} one fundamental but not explicitly stated conjecture\zeyu{premise? theorem?} is

\textbf{Conjecture: } \textit{The designed probe should reflect the ability of PTLM at any stage of training}.
\zeyu{Another premise of the paper is: if the knowledge is learned well by the model, then the knowledge probe performance should be stably increase overall during pretraining}
The reasoning is very simple: probes are designed in a \textit{model-agnostic} way by utilizing independently developed resources that conform human's understanding of the world --- e.g. linguistic theory \citep{nelson-probe}, knowledge base \citep{lama-probe}, carefully designed corpora (wino scheme challange\zeyu{cite}). In another word, the tested ability does not depend on the prior knowledge about PTLM; otherwise, we are faking to attribute PTLM's success. We believe this premise has to hold and already drives the research in probes for years. 
\jungo{I don't think linguistic theory is human understanding. Humans show linguistic phenomena and linguistic theories try to explain them by theory.}
\jungo{This paragraph will probably be most important; this is where we say something about recent trends in probing. \zeyu{Agree to discuss that in intro, I add two following paragraphs}} 

\citet{belinkov-etal-2020-interpretability-tutorial} survey the state of interpretability literature whose focus is on probes. One interesting characteristic is that the previous literature mainly focuses on whether the model or representation from the model well captures grammaticality of natural language.
\jungo{Not anymore? There's commonsense probing etc now right?}
This is an obvious and tempting direction and starting point to account for PTLM's success because linguistics is arguably the most systematic theory human have developed on language, and heavily drives NLP system design even in current data-driven era \zeyu{not sure what to cite}. However, recent works show other types of knowledge are also captured by PTLMs to a good extent \citep{cats-probe, numersense-probe}. This makes us introduce the notion of \textit{knowledge dynamics}, the behavior of knowledge in the model during pretraining, proxied by the probing performance. This work is mainly inspired by the hypothesis that \textit{different types of knowledge have different dynamics that together construct learning phases of PTLMs}. By showing what is missed and mastered, we believe making this analysis will offer insights in future redesigning and rethinking of current PTLM methods. 
\jungo{Nice!}

Another characteristic is that, partly for the sake of convenience, designed probes are tested on public release of PTLMs and compare with probing performance on baseline. Although we know something about these ``final models", the pretraining process remains black-box and anything could happen between the initialization and training stop (e.g. the possibility of catastrophic forgetting \citet{intermediate-fintuning}). From a radical view, although some early stopping metric (e.g. validation loss) can be used, those ``final models" are trained ``arbitrarily" for $K$ gradient updates (e.g. affected by random seed).  This work fill in the gap left by current probe design papers by studying the entire pretraining trajectory. Although prior work \citep{dynamics-by-svcca} investigated into similar problem with three linguistic tasks by focusing on the dynamics of representations from Long Short-Term Memory Networks, our work takes the advantage of recent massive probes to systematically attack the problem from a knowledge perspective and study a much stronger transformer-based PTLM --- \robertaAtEnd\footnote{We use \robertaAtEnd-BASE in this work}.   

With those in mind, we ask and answer two core questions overall:
\begin{enumerate}
    \item What do different knowledge dynamics look like?
    \item What are the implications?
\end{enumerate}

We propose a probe-based framework to observe knowledge dynamics and learning phases of different kinds of knowledge proxied by probes. First, we collect and categorize a wide and diverse set of existing probes into two major aspect of knowledge: Linguistic and Non-Linguistic knowledge. Due to its long-tailed nature \zeyu{need some reasoning here or later part of paper}, we also further break Non-Linguistic knowledge into Factual, Commonsense, and Basic Reasoning knowledge (\textsection \ref{sec:method:probes}). Then, we replicate pretraining with controlled corpus domain (\textsection \ref{sec:method:pretraining})) monitor the knowledge in \roberta with those \textit{knowledge probes} \citep{nelson-probe, edge-probe, lama-probe, cats-probe, numersense-probe, olmpics-probe} during the course of pretraining. Meanwhile, we also introduce some representative downstream tasks (\textsection \ref{sec:method:downstream}) to draw connections between diagnosis and more practical use of PTLM. We introduce \textit{$\epsilon$-learning phases} (\textsection \ref{sec:3}), an data analysis method to quantify the notion of \textit{fast-to-learn} (\textsection \ref{sec:1}) and \textit{slow-to-learn} (\textsection \ref{sec:2}). The intuition is: if a set of probes (e.g. Part-of-Speech, Syntactic Dependency, etc.) testing one kind of knowledge (e.g. linguistics) shows both consistent performance trends and $\epsilon$-learning phases compared with other knowledge probes, we can make some reasonable conclusions about learning patterns of the knowledge and its contribution to the downstream tasks. 

Our analysis reveals interesting insights such as:
\begin{enumerate}
    \item Surprisingly, \roberta  learns linguistic knowledge within a short and early time interval during pretraining. Training on different corpora domains shows the linguistic knowledge dynamics is independent of domain. \roberta is consistently showing improvement on the ling probing tasks.
    \item In contrast, factual and most commonsense knowledge is acquired incrementally as model iterate over the dataset by epoch. This slowness may hints at the inefficiency of using just Masked Language Model (MLM) objective in learning those knowledge and confirm the rationale behind recent specialized PTLM (e.g. KnowBERT, SpanBERT; \citet{KnowBERT, SpanBERT}). Controlled experiments show those knowledge depends very much on the selection of domain.
    \item Some basic reasoning and commonsense knowledge are not stable in \roberta. Such instability provides more concrete confirmation that \roberta doesn't learn the the abilities \citep{cats-probe, olmpics-probe}.
    \item When we compare our observation from probes with well-known finetuning tasks --- SST-2, MNLI, SQuAD, we realize that once linguistic knowledge is mastered at early stage, the gain from pretraining (i.e. acquisition of the other knowledge) is marginal. This suggests possible early stopping for pretraining, since we might be spending long time on pretraining for only marginal gain and provides evidence the long-tailed nature of non-linguistic task.
\end{enumerate}

% To answer Q(uestion)\ref{question:1}, we ground the validity of each probe by simply doing a \textit{pattern matching} between its trend and the trends of all downstream tasks. The intuition behind is that the underlying drive of probes is to \textit{account for} PTLM's superior performances on downstream tasks which by themselves are a \textit{consequential analysis} to better test a model's ``ability" \citep{kodner-gupta-2020-overestimation}. This should supposedly hold regardless of the \textit{time steps} (i.e. how many gradient updates the model has made), because we can pretrain for any number of steps and call it our ``final model". 

% Therefore, the probing performance should be reflective of the model's ``ability" at \textit{any time step} and it would be weird to see that some probing performance is really high, while the model trips on downstream tasks, or vice versa. Through visual and quantitative selection, we can not only determine what trends of some probe (or maybe just different probing setup made in the original papers) are problematic but also compare the trends among probes if the same type of knowledge is supposedly measured (e.g. syntactic dependency arc).

 
% The idea is very simple. We 1) train a PTLM with controlled domains; and due to the saving budget, we first save checkpoints more frequently in the beginning of training and less so when the PTLM is more trained. 2) select a wide range of probes with different design mechanism and different aimed knowledge or capability. In this work, we select \cwr\, \citep{nelson-probe} and \edge \, \citep{edge-probe} for linguistic knowledge, \lama\, \citep{lama-probe} for factual knowledge, \cat\, and \numer\, \citep{cats-probe, numersense-probe} for commonsense knowledge, and \olmpics\, \citep{olmpics-probe} for knowledge about basic reasoning. 3) select 

%  Through those work, we conclude that PTLM trained with a self-supervision signal is highly effective to learn internal structure of linguistic knowledge to understand human language, although being a different learning process from human's. And more recently, probing PTLMs from other perspectives also shows PTLMs are aware of other knowledge \citep{lama-probe, cats-probe, olmpics-probe}.
\zeyu{Notes:}
\begin{enumerate}
    \item show our observation contradict with common believes
    \item We need to find some surprising points
    \item in some probing papers, they claim the final percen makes people believe; we show the model can achive this 
    \item message: you will not learn such knowldge with current pertraining. Instead of just increasing dataset, we should think of ways to make
\end{enumerate}

==> archived/old_files/introduction-second.tex <==



\section{Introduction}

In the past few years, \textbf{P}re-\textbf{T}rained \textbf{L}anguage \textbf{M}odels (PTLMs) have become a key component of state-of-the-art neural NLP models \citep{liu_roberta:_2019, devlin_bert:_2018, yang_xlnet:_2019}, because using the PTLMs instead of previous off-the-shelf embeddings (e.g. GloVe, fastText) gives consistent performance boost across various downstream tasks \citep{elmo}. However, the reason for such success is unknown, which inspired a surge of probes. In those work, by demonstrating that PTLMs achieve higher scores on their defined probing tasks, they show that PTLMs contain more of some knowledge than their chosen baselines \citep{nelson-probe, edge-probe, lama-probe, cats-probe, olmpics-probe}. Intuitively, the \textit{abundance} of those knowledge might \textit{account for} PTLMs' success and assist downstream tasks (e.g. closed-book question answering). 

% , where $\mathcal{X} \in \left\{ \text{linguistic, factual, commonsense}, \cdots \right\}$ 
\zeyu{We are not trying to answer whether the containment of one knowledge account for the success, we are validating probes and then use validated probes to do further investigation}

However, from our perspective, it is very hard to \textit{validate} the claims from those probing papers mainly because: a) there are simply many different ways to frame a probing task. e.g. for one conceptual task (like syntactic dependency arc prediction), there are at least two ways to frame probes \citep{nelson-probe, edge-probe}. b) even for one chosen probe, we still can not fully believe its validity because the paper that develop them doesn't contain ways to falsify their proposal (sadly as always), while a scientific method should ideally be falsifiable. \zeyu{Not sure if this will cause wars from those authors. IMO, our paper is a proposal for validating probes which seems neutral.} 

Although \citet{hewitt-probe-control} provides us with the valuable insight that structural probe \citep{belinkov-etal-2020-interpretability-tutorial} should be as simple as possible to be selective, we believe the community still need a more concrete way to validate whether a probe is at least seemingly sensible (i.e. without solid theoretical proof). And more interestingly, given a set of \textit{valid} probes which arguably show the \textit{existence} of knowledge in a PTLM, can we utilize them to investigate a PTLM's knowledge acquisition process --- how the knowledge turns from \textit{paucity} to \textit{abundance}.

Towards this end, we propose an empirical approach. i) we select a wide range of probes and classify them into three types: linguistic, factual, commonsense. Then, we train \roberta on controlled domains of corpus and save checkpoints with different granularity. On those checkpoints, we ran our probes and make observations.


In this work, we ask and answer:
\begin{enumerate}
    \item How \textit{valid} are the examined probes? and what observations make the conclusion from a probe \textit{invalid}?  (\textsection \ref{sec:q1})
    \item Using creditable probes, what can we conclude about the learning dynamics of PTLM? (\textsection \ref{sec:q2})
    \item Can we suggest a plausible explanation to the observed learning dynamics? (\textsection \ref{sec:q3})
\end{enumerate}


==> archived/old_files/introduction-third.tex <==
\section{Introduction}

In the past few years, \textbf{P}re-\textbf{T}rained \textbf{L}anguage \textbf{M}odels (PTLMs) have become a key component of state-of-the-art neural NLP models \citep{liu_roberta:_2019, devlin_bert:_2018, yang_xlnet:_2019}, because using the contextualized representations from PTLMs instead of uncontextualized representation (e.g. GloVe, fastText) gives consistent performance boost across various downstream tasks (e.g. SST-2, MNLI, SQuAD; \citet{elmo, sst2-dataset, mnli-dataset, squad1.1-dataset}). However, the reason for such success is unknown, which inspired a surge of probes. In those work, by demonstrating that PTLMs achieve higher scores on their defined linguistic probing tasks, they show that PTLMs ``contain more knowledge" about $\mathcal{X}$ than their chosen baselines, where $\mathcal{X} \in \{\text{Part-of-Speech, Syntactic Dependency,} \cdots \}$ \citep{nelson-probe, edge-probe}. 
% Intuitively, the \textit{abundance} of those knowledge might \textit{account for} PTLMs' success over baselines on downstream tasks (e.g. SST-2, MNLI, SQuAD; \citet{sst2-dataset, mnli-dataset, squad1.1-dataset}). 

However, despite the convincing design and arguments from probing papers, it is still very hard to \textit{validate} their claims because the papers that develop them doesn't contain ways to falsify their methodology (sadly as always), while a scientific method should ideally be falsifiable.

One reason for structural probe is: there are simply many hyper-parameters one can set or design choices one can make for the classifier model. e.g. using Multi-Layer Perceptrons or linear transformation, size of hidden layer if using the former, etc. \citet{hewitt-probe-control} realized the differences among structural probes  \citep{belinkov-etal-2020-interpretability-tutorial} could originate from model complexity. Using control tasks, they demonstrate that structural probes should be validated to be as simple as possible for selectivity.

Some other difficulties includes: \circled{1} there are different ways to frame one probing task. e.g. for syntactic dependency arc prediction task, there are at least two ways to frame it \citep{nelson-probe, edge-probe}. \circled{2} even for one chosen probe (for one probing task), researchers only used the final model at the end of training (publicly released or trained by ourselves) to make comparison with baselines, and we know nothing about what happens during pretraining.

To make things more complicated, recently, even more probes on PTLMs for different knowledge (e.g. commonsense) and with different methodology (e.g. behavioral probes; \citet{belinkov-etal-2020-interpretability-tutorial}) has been proposed \citep{lama-probe, cats-probe, olmpics-probe}.

At early stage of the research field, \circled{1} is unavoidable because we lack a standardized way and enough probes to compare against. Like-wise, at early stage of developing one methodology, \circled{2} is also unavoidable for the sake of designing. However, the two difficulties leave two very important questions untouched respectively, regardless of how many probes will be proposed for PTLMs.
\begin{enumerate}
    \item \textit{How can we validate and compare probes?} \label{question:1}
    \item \textit{What can probes reflect about the knowledge acquisition process of PTLM?} \label{question:2}
\end{enumerate}
We believe these two questions need to be investigated for the community to move forward. From a data analysis standpoint, we believe adding a global \textit{learning dynamics view} on probes will kill the two birds with one stone. As an overview of our experiment setup, a) we chose to (almost) replicate training of \roberta for reasons detailed in (\textsection \ref{sec:exp:pretraining}). b) we choose a wide range of probing tasks (\textsection  \ref{sec:exp:probes}), and c) a set of well-established downstream tasks (\textsection \ref{sec:exp:downstream}). Then, our method assumes checkpoints of \roberta over the course of pretraining and probing performances of all probing and downstream tasks on each PTLM checkpoints. \textsection  \ref{sec:methods} details more about the underlying rationale of our method. With all the materials prepared, we are able to start our dynamics analysis and further discussions on the two important questions (\textsection \ref{sec:1}, \ref{sec:2}, \ref{sec:3}). 

The contribution of this work includes:
\begin{itemize}
  \item Our proposed analysis perspective provides a ground to validate and compare probes. We use \roberta as a case study but the method is generalizable to any PTLM and probes.
  \item With the validated probes, we discover some surprising insight into takeaway from the knowledge acquisition patterns and phases of \roberta. 
  \item To inspire future research, we provides more in-depth analysis on our observations and try to offer some possible explanation by referring to the trade-off between generalization and memorization. 
\end{itemize}

Due to the page limit, we try to be succinct about our findings and left more supplementary materials in the Appendix.

% To answer Q(uestion)\ref{question:1}, we ground the validity of each probe by simply doing a \textit{pattern matching} between its trend and the trends of all downstream tasks. The intuition behind is that the underlying drive of probes is to \textit{account for} PTLM's superior performances on downstream tasks which by themselves are a \textit{consequential analysis} to better test a model's ``ability" \citep{kodner-gupta-2020-overestimation}. This should supposedly hold regardless of the \textit{time steps} (i.e. how many gradient updates the model has made), because we can pretrain for any number of steps and call it our ``final model". 

% Therefore, the probing performance should be reflective of the model's ``ability" at \textit{any time step} and it would be weird to see that some probing performance is really high, while the model trips on downstream tasks, or vice versa. Through visual and quantitative selection, we can not only determine what trends of some probe (or maybe just different probing setup made in the original papers) are problematic but also compare the trends among probes if the same type of knowledge is supposedly measured (e.g. syntactic dependency arc).

 
% The idea is very simple. We 1) train a PTLM with controlled domains; and due to the saving budget, we first save checkpoints more frequently in the beginning of training and less so when the PTLM is more trained. 2) select a wide range of probes with different design mechanism and different aimed knowledge or capability. In this work, we select \cwr\, \citep{nelson-probe} and \edge \, \citep{edge-probe} for linguistic knowledge, \lama\, \citep{lama-probe} for factual knowledge, \cat\, and \numer\, \citep{cats-probe, numersense-probe} for commonsense knowledge, and \olmpics\, \citep{olmpics-probe} for knowledge about basic reasoning. 3) select 

%  Through those work, we conclude that PTLM trained with a self-supervision signal is highly effective to learn internal structure of linguistic knowledge to understand human language, although being a different learning process from human's. And more recently, probing PTLMs from other perspectives also shows PTLMs are aware of other knowledge \citep{lama-probe, cats-probe, olmpics-probe}.

==> archived/old_files/methods-first.tex <==
\section{Methods}
\label{sec:methods}
\subsection{Pretraining}
\label{sec:pretraining}
\label{sec:diagnostic-probes}
% \textbf{Motivation for each type of probes}
% \textbf{short description of each task}
% \textbf{at least one example from each probe}
Due to the large number of probes we included in this studies, we briefly explain what each probes measures and defer the details to the original work.

\subsection{Linguistic probes} Due to the nature of tasks, linguistic probes are all structural probes. We prefix diagnostic tasks selected from \citep{nelson-probe} with \cwr\textbf{-}  and tasks from \citet{edge-probe} with \edge\textbf{-}.  We also give examples of each tasks in \textsection \ref{appendix:probe-examples}.
\label{sec:linguistic-probes}

% (e.g. \ccg) 
% (e.g. \textbf{\edge-POS})
\label{sec:nelson-probes}
\subsubsection{\cwr\textbf{-} Probes}
\textbf{Part-of-speech tagging} (\pos) is the syntactic task of assigning tags such as noun, verb, etc. to individual tokens. We test on the PennTreeBank (\PTBpos; \citet{ptb-dataset}) and the English Web Treebank (\EWTpos; \citet{ewt-parse-dataset}).

\textbf{Named entity recognition} (\ner) examines whether contextual representations encode information about entity types. % on the CoNLL 2003 shared task dataset \citep{conll-2003-shared-task-ner}.

\textbf{CCG supertagging} (\ccg) assesses the fine-grained information about the syntactic roles of contextual representations. %  on CCGBank dataset \citep{ccg-ptb-dataset}.
 
\textbf{Syntactic chunking} (\chunk) tests whether the word representations contain shallow notions of spans and boundaries. % on the CoNLL 2000 shared task dataset \citep{conll-2000-shared-task-chunking}.
% ; the task is to segment text into shallow constituent chunks. 

\textbf{Grammatical error detection} (\ged) is the task of identifying tokens which need to be edited to produce a grammatically correct sentence. %  on converted First Certificate in English dataset \citep{first-certificate-in-english-dataset}.

\textbf{Conjunct identification} (\conj) challenges the model to identify the tokens that comprise the conjuncts in a coordination construction. % on coordination-annotated PTB of \citet{coordination-annotated-PTB-dataset}.

\textbf{Event factuality} (\ef) task involves labeling phrases with the factuality of the events they describe. % on Universal Decompositional Semantics It Happened v2 dataset \citep{event-factuality-dataset}.

\textbf{Preposition supersense disambiguation} is the task of classifying a preposition’s lexical semantic function (\psFxn) and the semantic role or relation it mediates (\psRole). % on the STREUSLE 4.0 corpus \citep{streusle-4.0-corpus-dataset}.

In \textbf{syntactic dependency arc} task, the model is given the representations of a head token and a modifier token, and the trained probe predicts, in the sentence’s syntactic dependency parse, the \textit{existence} (\textbf{SynArc-Pred}) and the \textit{type} (\textbf{SynArc-Class}) of a dependency arc between them. Like \pos, we test on PTB (\PTBsyn\textbf{-[Pred/Class]}\,) and EWT (\EWTsyn\textbf{-[Pred/Class]}).
% two tokens --- $w_{head}$  as 
% $w_{mod}$ as 

Similarly, for \textbf{semantic dependency arc}, the trained probe predict the existence (\semPred) and type (\semClass) of a semantic dependency arc.
% we use the DELPH-IN MRS-Derived Semantic Dependencies (DM) target representation from the SemEval 2015 shared task \citep{semeval-2015-task-dataset} and
% with the DELPH-IN MRS-Derived Semantic Dependencies (DM) target representation. The probe is trained

\textbf{Coreference arc prediction} (\coref) task has the probe trained to predict whether two entities corefer from their contextual representation.

\subsubsection{\edge\textbf{-} Probes}
\label{sec:jiant-probes}
\textbf{
Semantic role labeling} (\srl) is the task of imposing predicate-argument structure onto a natural language sentence.

\textbf{Semantic proto-role} (\spr) labeling is the task of annotating fine-grained, non-exclusive semantic attributes, such as change of state or awareness, over predicate-argument pairs. We also test on PTB (\PTBspr) and EWT (\EWTspr).

\textbf{Relation Classification} (\rel) is the task of predicting the real-world relation that holds between two entities, typically given an inventory of symbolic relation types (often from an ontology or database schema). make distinction from LAMA


% Part-of-speech tagging (POS)

\subsection{Factual (\lama\textbf{-}) Probes}
\label{sec:factual-probes}
In our factual probes, $S$ is a subset of the \roberta vocabulary set. In commonsense probes, $S$ is a set of sentences which contains one positive sentence and at least one negative sentences. Our factual probe is from \citet{lama-probe}. The test dataset is constructed from Google-RE (\lamaGoogle), SQuaD (\lamaSquad), TREx (\lamaTrex), and ConceptNet (\lamaConcept).









\subsection{Commonsense Probes}
\label{sec:commonsense-probes}
pick the positive sentence along side with one or more negative sentences

\subsubsection{\cat\textbf{-} Probes}
\label{sec:cat-probes}

\subsubsection{\olmpics\textbf{-} Probes}
\label{sec:olmpics-probes}

\subsubsection{\numer\textbf{-} Probes}
\label{sec:numersense-probes}

\subsection{Models to Investigate}

\paragraph{Baselines}
glove, random initialization

\subsection{Downstream Tasks}
\label{sec:downstream}


probing task look for whether info contained in or accessible ?
comparison with random model? 




==> archived/old_files/methods.tex <==
\section{Method}
We present our method to probe the knowledge dynamics of self-supervised pretraining here. \textsection \ref{sec:method:core_idea} discusses the motivation of our methodology and high-level design choices. Then, we discuss the pretraining process (\textsection \ref{sec:method:pretraining}), knowledge probes (\textsection \ref{sec:method:probes}), and downstream tasks (\textsection \ref{sec:method:downstream}) chosen in our framework. 
\label{sec:method}

\subsection{Motivation and baselines}
\label{sec:method:core_idea}

\jungo{The following paragraph seems to need some more work to make it clear. This is arguably the most important paragraphs in this section. We can cite early probing papers (what's even the earliest?, I don't know.) and claim no one really applied it to dynamics.} \zeyu{Agree, made some changes, still think we can improve}
\paragraph{Motivation} \textit{Does a model learn knowledge?} This is a hard philosophical question. Current probe literature addresses this issue by measuring how accurate a pretrained language model can get on a set of examples constructed by using some knowledge repertoires.
This is indicative of how closely the model conforms to human understanding of the world because those knowledge sources i) were constructed \textit{independently} of training the probed model and ii) intend to best reflect human knowledge --- linguistic (e.g., PennTree Bank) or non-linguistic (e.g., ConceptNet) \jungo{citation}. In other words, the test does not depend on the prior about any model but on the desired outcome from a learning process (i.e., training the model). In our case, this leads to a very simple yet crucial premise for probing PTLM:

\textit{The performances of designed probes reflect the ability of a PTLM at any stage of training}.

To the best of our knowledge, this straightforward premise is surprisingly unspoken at time of previous probe designs \cite{kohn-2015-whats,  cooper-1996-early-behavioral-probe} \zeyu{both are from \citet{belinkov-etal-2020-interpretability-tutorial}; first is earliest structural probe, second is earliest behavioral; no permission to read the last, judge from abstract}. However, we believe this premise has to hold and already drives the probe designs for years. Our work utilizes this premise to advance our understanding of PTLMs.

\paragraph{Probe construction} \textit{Behavioral} probes test the model's behavior as a language model  (e.g. whether predict word correctly; \citet{blimp-probe, lama-probe, numersense-probe, cats-probe, olmpics-probe}). Their repertoires are usually knowledge bases (e.g. ConceptNet) or carefully crafted sentence-generating templates.  The examples from those behavioral probes are then validated by crowdsource workers. The correctness is measured by whether the model chooses the sensible sentence from distractor(s). 

Contextual representation is a byproduct of current PTLM.
\jungo{It's actually the main product now.}
\textit{Structural} probes (classified in \citet{belinkov-etal-2020-interpretability-tutorial}) implemented as diagnostic classifiers test the abundance (or easeness of extraction) of linguistic knowledge in those representations \citep{nelson-probe, edge-probe}. In this case, the repertoire is chosen to be expert-annotated dataset (e.g. PenTree Bank, OntoNotes) and the abundance is measured by the accuracy of classifier.
\jungo{It's great to have some categorization of probing tasks. So this preceding section does that. But I'm not sure if crowsource vs.\ expert is a good contrast. You can ask experts to make behavioral probes as well? I need to check Belinkov's paper, but you should probably not make too many assumptions.}


\input{tables/tab_baselines}
\paragraph{Baseline setup} Due to their slightly different design, each probe has its own empirical lower and upper bounds to set references for \textit{the worst performance} and \textit{the best performance}. Although baseline performances are not comparable, we use (mostly) same idea for setting the baselines. 
\jungo{what's the idea?}

For each probe, an upper bound is the probe performance from officially released \roberta --- \robertaOfficial. Lower bounds include randomly initialized \roberta, averaged across 3 trials. In addition, each behavioral probe includes the expected accuracy by using random guess $\left(=\frac{1}{\text{\# choices}}\right)$. For each structural probe, we also replace the contextual representation with GloVe and random vectors of $[-2,2]^d$, where $d$ is the dimension of GloVe \zeyu{basically copy Table \ref{tab:baselines} caption}.
Table \ref{tab:baselines} is the full list of probes and baselines. 


\subsection{Pretraining}
\label{sec:method:pretraining}

\paragraph{Usage} During pretraining, we periodically save the pretraining trajectory of \roberta. Overall, we save more frequently (e.g. every 1000 updates) around the first epoch; later, if the dataset is ``small" ($\leq 12$GB), we save checkpoints by epoch; otherwise, we save every 12GB text to collect enough checkpoints for later usage. 
\zeyu{Need to confirm with Yizhong}

Our \robertaAtEnd\, and training setting follows closely the settings prescribed in \citet{liu_roberta:_2019}. 
We choose corpora of varies sizes from different domains to study the effect of corpus size and domain (see Table \ref{tab:corpus-domain} \zeyu{Not sure why it doesn't compile here}). 
We build on tutorial from Google\footnote{\url{https://cloud.google.com/tpu/docs/tutorials/roberta-pytorch}} and run training on a v3-8 TPU\footnote{Free usage for the public in the duration of this work} with setting specified in \ref{appendix:roberta-corpus}.


\subsection{Knowledge Probes}
\label{sec:method:probes}

% For our experiments, we only include probes that shows, in each original paper, \roberta is superior to baseline by a noticeable margin (i.e. $>$10\% accuracy).
We categorize the collected knowledge probes into four types --- \textbf{linguistic}, \textbf{factual}, \textbf{commonsense}, \textbf{basic reasoning} --- each containing many probes. We include probes that show both PTLM's success and its failure because we want to avoid 1) the possible catastrophic forgetting \citep{intermediate-fintuning} that may happen during pretraining \jungo{I don't know why this avoids forgetting} and 2) the arbitrary gradient updates to obtain our ``final model" (\textsection \ref{sec:intro}). Due to the space limit, we select one representative task from each probes and for each knowledge type (See Table \ref{tab}). The full descriptions are deferred to the original work, and we include the full list of probes in Appendix \ref{appendix:probe-examples}.

\paragraph{Usage} We run each probe specified below on the saved checkpoints (usually) with \roberta frozen.
\jungo{usually? Specify more here.} 
We will get a score per probe from its test set, which serves as a proxy of the tested knowledge.
Each set of probes has its own baselines due to distinct designs across probes.
\input{tables/tab_probe_examples_main}


% \label{sec:method:probes:linguistic}
\subsubsection{Linguistic probes} 

Our linguistic probes includes structural probes --- \cwr\,(Contextual Word Representation; \citet{nelson-probe}) and \edge\,(Edge Probing; \citet{edge-probe}) --- and behaviors probes --- \blimp\, (Benchmark of Linguistic Minimal Pairs; \citet{blimp-probe}).
\jungo{Need more explanation what edge probing, bilmp mean etc.}

Due to the various linguistic theories proposed and the hierarchy of linguistic theory (e.g. morphology, syntax, semantics, etc.), there are many aspects from which linguistics researchers can analyze a sentence. To maximize the coverage of linguistic information encoded in representation, we use non-overlapping probes from \cwr\, and \edge.

Using insights from \citet{hewitt-probe-control}, we choose a linear model for our classifier for better selectivity.
\jungo{Explain what insight you are getting from it.}
In structural probe designs, the classifier receives one or optionally two representation(s) and train to predict a label such as a constituent or relation type; in \edge, the representation is from a span of tokens, while, in \cwr, the representation comes from a token. \textbf{Metric:} The accuracy is determined by whether the classifier predict the label correctly.
\jungo{Oh you're explaining CWR and edge probing here a bit. But be clearer and explain earlier.}

\blimp\, consists of 67 individual datasets (12 tested phenomena), each containing 1,000 minimal pairs, i.e. pairs of minimally different sentences that contrast in grammatical acceptability and isolate specific phenomenon in syntax, morphology, or semantics. Each test contains minimal pair of sentences. \textbf{Metric:} we determined the correctness by whether PTLM assigns higher probability to the the grammatical token given the context.

\zeyu{Maybe we can include some presented probes here}
% Our linguistic probing suite includes labeling tasks: Part-of-speech tagging (\PTBpos, \EWTpos; constructed from the PennTreeBank and the English Web Treebank); Named Entity Recognition (\ner); CCG supertagging (\ccg); Syntactic Chunking (\chunk); Grammatical Error Detection (\ged); Conjunct Identification (\conj); Event Factuality (\ef); Preposition Supersense Disambiguation for lexical semantic function (\psFxn) and the semantic role or relation it mediates (\psRole); similar to part-of-speech tagging, Syntactic Dependency Arc Prediction and Classification task on PTB and EWT --- \PTBsynPred, \PTBsynClass, \EWTsynPred, \EWTsynClass; Coreference Arc Prediction (\coref); Semantic Role Labeling (\srl); Semantic Proto-Role Labeling, constructed using PTB (\PTBspr) and EWT (\EWTspr); Relation Classification (\rel).

% two tokens --- $w_{head}$  as 
% $w_{mod}$ as 
\subsubsection{Factual probes} The name ``factual" emphasizes this tested knowledge requires memorization and are usually explicitly stated, in contrast to the more intuitive and implicit commonsense knowledge. 

We use probes from \lama\, (LAnguage Model Analysis; \citet{lama-probe}). For more systematic coverage, \lama\, is constructed using large knowledge bases like the Google-RE corpus \footnote{\url{https://code.google.com/archive/p/relation-extraction-corpus/}}.  These probes test the model on simple\footnote{Subject-Verb-Object sentence, optionally passive} sentences with their object masked and asked the model to predict the masked words (e.g. ``Albert Einstein was born in [MASK]"). \textbf{Metric:} Since the output space is a subset of \roberta vocabulary that excludes sub-tokens, we measure its accuracy by how high the model ranks the correct word (i.e., Precision at $K$).
% Our factual probing suite includes use knowledge sources from: Google-RE corpus (\lamaGoogle), T-REx (\lamaTrex), and SQuAD (\lamaSquad).

\subsubsection{Commonsense probes}
Currently, there are different ways people have tested commonsense knowledge based on the model's behavior rather than a trained classifier \cite{da-kasai-2019-cracking}. One way is \lama\,, which contains a widely used commonsense knowledge base --- ConceptNet (\lamaConcept). 
\jungo{LAMA appears again here. Mention something like similar to .... otherwise not clear why you have the same name appear in two categories.}

Similar to \lama\,, \citet{numersense-probe} develops a specialized probe --- only numbers in range $[0, 10]$ are included --- for \textit{numerical} commonsense knowledge, called ``\text{{\normalsize N}{\footnotesize UMER}{\normalsize S}{\footnotesize ENSE}}" (\numer). \textbf{Metric:} Since the output space is much smaller than that of \lama, we measure its accuracy by whether PTLM chooses the right number.
\jungo{What is numerical commonsense? Explain?}

Another way to probe is \cat (Commonsense Ability Test; \citet{cats-probe}), where they unify the form of all the chosen datasets and compares PTLMs' probability-based score on positive (sentence that fits commonsense) and negative samples (sentences that don't). \textbf{Metric:} The accuracy is determined by whether a PTLM can score positive sample the highest. 
% For this one, we include test suites constructed from: Conjunction Acceptability (\catCA), Sense Making (\catSM), Winograd Schema Challenge (\catWSC), SWAG (\catSwag), HellaSwag (\catHS), Sense Making with Reasoning (\catSMR) and the original Argument Reasoning Comprehension Task (\catArctOne); we also include the argumented ARCT (\catArctTwo) by adding negation to alleviate its statistical cues.

\subsubsection{Basic Reasoning probes}
% we use the DELPH-IN MRS-Derived Semantic Dependencies (DM) target representation from the SemEval 2015 shared task \citep{semeval-2015-task-dataset} and
% with the DELPH-IN MRS-Derived Semantic Dependencies (DM) target representation. The probe is trained
\olmpics (\textbf{o}n what \textbf{L}anguage \textbf{M}odel \textbf{p}re-tra\textbf{i}ning \textbf{c}apture\textbf{s}; \citet{olmpics-probe}) uses ConceptNet, WordNet and others to categorize and design eight focused tests for basic reasoning abilities (e.g. Age-Comparison). The framing is similar to \numer\,and \lama, except the output space is restricted to 2-5 words depending on the tests. They show PTLMs lack many tested reasoning abilities. 
%  To account for the difference in use of language between pretraining corpus and the probing dataset, we use the fine-tuning setup where we first fine-tune \robertaAtEnd's language head \jungo{What's language head?} on a training set, and then infer on the test set; for simplicity, we only consider the final fine-tuned model's performance.
% To make \olmpics more comparable to other non-linguistic probes, we only adopt task that test PTLM as an MLM (i.e. only MC-MLM setup in the paper). 
\textbf{Metric:} Similar to \numer, we measure its accuracy by whether PTLM chooses the right token.

% The tested ability includes: use of Always-Never (\olmpicsAlways); comparison between age (\olmpicsAge) and object (\olmpicsObj) sizes; properly applying negation in the context of \textit{synonyms v.s. antonyms} (\olmpicsAntonym); ability to find concepts for which a conjunction of properties holds (\olmpicsProperty; “What is located in a street and is related to octagon?”) and find the mutual hypernym of a pair of concepts (\olmpicsTaxonomy; e.g. “A germ and a human are both a type of [MASK].”); capability to do question answering of encyclopedic (\olmpicsEncyc; e.g. ``When did the band where John Lennon played first form?”) and multi-hop (\olmpicsMultiHop; e.g. “When comparing a 83 year old, a 63 year old and a 56 year old, the [MASK] is oldest”) nature.

\subsection{Downstream tasks}
\jungo{Why do we care about downstream tasks in this probing paper? Explain?}
\label{sec:method:downstream}
\paragraph{Usage} We fine-tune \robertaAtEnd\, checkpoints per downstream task with a linear top layer to avoid introducing too many parameters irrelevant to \robertaAtEnd's weights. Settings are detailed in \textsection \ref{appendix:downstream-setting} 

\jungo{I see. The following paragraph should be the starting statement because this is why we're talking about downstream. See my previous comment.}
By using downstream tasks, we connect diagnostic measures with some more practical contexts, which offer hints like which knowledge help the practical tasks we care more about. Another radical view is that these tasks can be seen as ``consequence-based" analyses \citep{kodner-gupta-2020-overestimation} where the model has to utilize knowledge recognized by the current probes and those to be recognized in the future. 
% Note that \roberta is trained when fine-tuning for downstream tasks while diagnostic probes keep \roberta freezed. 


Our task suite uses three representative well-known and -established tasks: \sstTwo\, --- single-sentence classification --- with accuracy of predicting the right class; \mnli\, --- sentence-pair classification --- with accuracy on matched (\mnlim) and mismatched (\mnliMm) genres; \squad\,--- extractive reading comprehension --- with predicted span measured by exact match (\squadEM) and F1 score (\squadFOne).
\jungo{Again, this is a laundry list. Describe it better?}

\subsection{$\epsilon$-Learning phases}
After we follow the instruction above, for each probing or downstream task, we will have a series of scores $S$ over the pretraining trajectory. For examples, for each \roberta checkpoint, we will have a CCG supertagging score. To quantify the notion of ``fast-to-learn" and ``slow-to-learn" for a specific task, we introduce an interval $I_{\epsilon}(S)$ called $\epsilon$-Learning phase, where $\epsilon \in [0, 0.5)$. It is calculated by $$ I_{\epsilon}(S) = \texttt{end}_\epsilon(S) - \texttt{start}_\epsilon(S)$$

$\texttt{start}_\epsilon(S)$: the first time the model achieve equal or higher than $\epsilon$ of the best probing performance in $S$

$\texttt{end}_\epsilon(S)$: the first time the model achieve equal or higher than $1-\epsilon$ of the best probing performance in $S$

With such a simple concept introduced, ``fast-to-learn" simply means the model reaches a high enough performance within a shorter interval and vice versa.\footnote{we set $\epsilon = 0.05$ in our paper. \jungo{More justification/discussion on this?}} Note this learning phase doesn't allow comparing knowledge dynamics across different trains of PTLM, e.g. CCG supertagging may achieve different max performance by using PTLMs trained on \wiki and \realnews.

==> archived/old_files/new-ideas.tex <==
\section{New Ideas}
% \subsection{}
Proposal of another analysis dimension — \textbf{dynamics} for interpretability to understand pretraining or just training in NLP. What’s the benefit of adding this layer of complication?

\begin{enumerate}
    \item understanding the learning of PTLM, why PTLM acquires knowledge in more fine-grained monitoring rather than just looking at the results because just looking at a one-time stamp, the picture is in-complete. From our observation, much more in-depth analysis can be made towards a better understanding of PTLM
    \item are probes similar to one or another, how can we quickly identify differences? Our approach is a very straightforward test-bed for this.  From this time perspective, "abnormality"/difference among probes can be easily/directly observed; it would signal to investigate what’s causing the abnormality. [How do people usually argue for differences in probes? They seldom do so, iirc.]. 
    \item Probes are usually run very fast (they should be as simple as possible), so new proposed probes can also run on PLTM checkpoints, which would contribute to the general understanding of PTLM training at a very relatively small GPU cost.
    \item We found there are still lots of things that remain un-covered for how PTLM learns. 
    \begin{enumerate}
        \item Why some knowledge is unstable? Is this a matter of probes or a matter of language models. Call for re-calibration of probes or standardized/systematic way to compare probes.
        \item Also, some weird pattern makes us suspecting the conclusion we get from probing papers. Even though the probing paper gives convincing reasons and intuitive conclusion that larger models learn more knowledge (despite the existence of weakness), when we pose probes in this dynamics settings, a lot of interesting discussions and more diverse investigation can be inspired. 
    \end{enumerate}
    \item Behavioral probes has proven its success in practical tasks like Entity Set Expansion
    
    \item \citet{kodner-gupta-2020-overestimation}: Criticism of Tal Linzen’s work —  one must take successes in template-based probing studies with a grain of salt, \textbf{support for Consequence-based analysis (e.g. finetuning results)}:
    
    Shortcoming of template methods: there may still be sufficient superficial word order information to achieve the effect despite the addition of optional modifiers e.g.  verbs that are more likely to appear in object Relative Clauses are likely to pattern similarly in other constructions too
        \begin{enumerate}
            \item An n-gram LM can only learn surface collocations and so cannot capture (hierarchical) syntax, so if it produces a significant differential adaptation effect, then the experiment is not able to discriminate between models which capture syntax from those which do not.
            \item Scrambled-input LSTM
        \end{enumerate}
    \item Research start to hope that PTLM would be a place for all sorts of knowledge. We see advances in different directions: 1. incooporate awareness of some knowledge during pretaining  2. given BERT, use already existing PTLM and then fuse knowledge into it. 3. But GPT-3 exists, which is a pure data-driven method? Therefore, it seems crucial to understand the learning dynamics with pretraining.
    \item encourage researchers who propose new PTLM to release their checkpoints for better understanding of PTLM in the community,  which likely leads to a better design
    \item Probing paper design probes and with their results speculate the learning process of PTLM. However, there is still rooms for explanation, but I think they sometimes admit this in their paper...
    \item How to connect this with data-leakage? Any Leakage from training set? Vocabulary coverage? fastText embedding comparison? Some inspiration from \citep{gonen-etal-2020-simple}
    \item we currently lack a toolkit for investigating the deep connection from this behavioral/representational trends to consequential trends. At this stage, only a more in-depth data analysis and its resulting speculation are provided for future research. Call for attentions on this.
    \item admit that our work is still very preliminary
    \item different "important neurons" for different probing tasks?
    \item dissociation between perplexity and syntactic generalization performance                                                           \cite{hu-etal-2020-systematic}
    \item Methods to measure generalization and memorization on synthetic/unnatural dataset: \url{https://jair.org/index.php/jair/article/view/11674/26576}
\end{enumerate}

\subsection{Potential To-do}
\begin{enumerate}
    \item include finetune task on DROP dataset
    \item when calculating correlation, also consider significance level
    \item include behavioral ling probes?
\end{enumerate}

==> archived/old_files/wrong_hypothesis.tex <==
\section{Wrong hypothesis}
\label{sec:wrong-hypothesis}
\begin{enumerate}
    \item no catastrophic forgetting during pretraining \cite{intermediate-fintuning} \zeyu{I think our experiments shows that MLM is an \textbf{knowledge-absorbing objective}}
    \item
\end{enumerate}


==> tables/old_tab_probe_examples_main.tex <==
\begin{table*}[thb]
    \tiny
    % \small
    \centering\renewcommand\cellalign{lc}
    \setlength\tabcolsep{2.5pt}
    \setcellgapes{4pt}\makegapedcells
    \def\arraystretch{1.2}
    \begin{tabular}{c|c|c|c|c} 
    \toprule
    \textbf{Probe Package} & \textbf{Knowledge} & \textbf{Task } & \textbf{Task Format} & \textbf{Example} \\ 
    \hline
    % $[\text{The}]_{\textbf{\text{NP/N}}}\; [\text{market}]_{\textbf{\text{N}}}\; [\text{crumbled}]_{\text{S\textbackslash NP}} [\text{.}]_\text{.}$   \zeyu{a placeholder}
    \multirow{13}{*}{\cwr} & \multirow{13}{*}{Linguistic} 
        & \multirow{3}{*}{POS Tagging} & \multirow{3}{*}{Token Labeling} & 
        \multirow{1}{*}{\begin{dependency}[style=above]
          \begin{deptext}[column sep=0.2em]
              PRON \& AUX \& VERB \& ADV \& ADP \& DET \& NOUN \& PUNCT \\
              I \& 'm \& staying \& away \& from \& the  \& stock  \& . \\
          \end{deptext}
        \end{dependency}} \\
        & & & & \\  % use this as an empty line to make multirow works
        % \taginline{Is}{VERB} \taginline{that}{DET} \taginline{a}{DET} \taginline{money}{NOUN} \taginline{marker}{NOUN} \taginline{?}{PUNCT}
        % $[\text{Is}]_{\textbf{\text{VERB}}}\; [\text{that}]_{\textbf{\text{DET}}}\; [\text{a}]_{\textbf{DET}}\; [\text{money}]_\textbf{NOUN} [\text{marker}]_\textbf{NOUN} [\text{?}]_\textbf{PUNCT}$
        % \text{\taginline{V}{Is} \taginline{Is}{that} \taginline{Is}{a} \taginline{Is}{money} \taginline{Is}{marker}}
        \cline{3-5}
        & & \multirow{3}{*}{Syntactic Chunking} & \multirow{3}{*}{Token Labeling} & 
        \multirow{1}{*}{
        \begin{dependency}[style=above]
            \begin{deptext}[column sep=0.1em]
              \graytextbf{B-NP} \& \graytextbf{B-VP} \& \graytextbf{B-PP} \& \textcolor{cyan}{\textbf{B-NP}} \& \textcolor{cyan}{\textbf{I-NP}} \& \textcolor{cyan}{\textbf{I-NP}} \& \graytextbf{O} \\
              \graytext{Shearson} \& \graytext{works} \& \graytext{at} \& \textcolor{cyan}{American} \& \textcolor{cyan}{Express} \& \textcolor{cyan}{Co} \& \graytext{.} \\
          \end{deptext}
        \end{dependency}} \\
        & & & & \\  % use this as an empty line to make multirow works
        \cline{3-5}
        % \taginline{Shearson}{B-NP} \taginline{is}{B-VP} \taginline{about}{B-ADJP} \taginline{60}{I-ADJP} \taginline{by}{B-PP} \taginline{American}{B-NP}  \taginline{Express}{I-NP} \taginline{Co}{I-NP}  \taginline{.}{O} \\
        & & \multirow{3}{*}{Named Entity Recognition} & \multirow{3}{*}{Token Labeling} &  % \taginline{By}{O} \taginline{stumps}{O} \taginline{Kent}{I-ORG} \taginline{had}{O} \taginline{reached}{O} \taginline{158}{O}  \taginline{for}{O} \taginline{three}{O}  \taginline{.}{O} \\
        \multirow{1}{*}{\begin{dependency}[style=above]
            \begin{deptext}[column sep=0.2em]
              \graytextbf{O} \& \graytextbf{O} \& \textcolor{magenta}{\textbf{I-ORG}} \& \textcolor{magenta}{\textbf{I-ORG}} \& \textcolor{magenta}{\textbf{I-ORG}} \& \graytextbf{O} \& \graytextbf{O} \& \graytextbf{O} \& \graytextbf{O} \\
              \graytextbf{By} \& \graytextbf{stumps} \& \textcolor{magenta}{Kent} \& \textcolor{magenta}{County} \& \textcolor{magenta}{Club} \& \graytextbf{had} \& \graytextbf{reached} \& \graytextbf{108} \& \graytextbf{.} \\
          \end{deptext}
        \end{dependency}} \\
        & & & & \\  % use this as an empty line to make multirow works
        \cline{3-5}
        & & \multirow{3}{*}{Syntactic Arc Classification}  & \multirow{3}{*}{Pairwise Relations} & \multirow{1}{*}{
        \begin{dependency}[edge vertical padding=-0.4ex]
          \begin{deptext}[column sep=2em]
              Peter \& and \& May \& bought \&  a \&[1em]  car \&[.1em] . \\
          \end{deptext}
          \deproot[edge unit distance=1.05ex, hide label]{4}{ROOT}
          \depedge[edge unit distance=1.1ex]{4}{2}{\tiny Subj}
          \depedge[edge unit distance=0.8ex]{2}{1}{\tiny Conj}
          \depedge[edge unit distance=0.8ex]{2}{3}{\tiny Conj}
          \depedge[edge unit distance=0.8ex,]{4}{6}{\tiny Obj}
          \depedge[edge unit distance=0.3ex,]{6}{5}{\tiny Det}
          \depedge[edge unit distance=0.95ex]{4}{7}{\tiny Punct}
        \end{dependency}} \\
        & & & & \\  % use this as an empty line to make multirow works
        % & & & & \\  % use this as an empty line to make multirow works
        \cline{3-5}
        & & \multirow{3}{*}{Syntactic Arc Prediction} & \multirow{3}{*}{Pairwise Relations}  & 
         \multirow{1}{*}{
         \begin{dependency}[edge vertical padding=-0.4ex]
          \begin{deptext}[column sep=2em,]
              Peter \& and \& May \& bought \&  a \&[1em]  car \&[.1em] . \\
          \end{deptext}
          \deproot[edge unit distance=1.05ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}, hide label]{4}{ROOT}
          \depedge[edge unit distance=1.1ex, label style={text=lightgray,draw=lightgray},  edge style={lightgray,densely dotted}]{4}{2}{\tiny Subj}
          \depedge[edge unit distance=0.8ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted},]{2}{1}{\tiny Conj}
          \depedge[edge unit distance=0.8ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted},]{2}{3}{\tiny Conj}
          \depedge[edge unit distance=0.3ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted},]{6}{5}{\tiny Det}
          \depedge[edge unit distance=0.95ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted},]{4}{7}{\tiny Punct}
          \depedge[edge unit distance=0.8ex, label style={text=red}, edge style={red!60!black,thick,>=triangle}]{3}{4}{\tiny \xmark}
          \depedge[edge unit distance=1ex, label style={text=red}, edge style={red!60!black,thick,>=triangle}]{1}{3}{\tiny \xmark}
          \depedge[edge unit distance=0.8ex, label style={text=green,}, edge style={green!60!black,thick,>=triangle},]{4}{6}{\tiny \boldsymbol{\cmark}} 
        \end{dependency}} \\
        & & & & \\  % use this as an empty line to make multirow works
        % & & & & \\  % use this as an empty line to make multirow works
    \cline{1-5}
    % \cline{3-5}
    \multirow{6}{*}{ \blimp} &  &  \multirow{2}{*}{Island Effect} & \multirow{2}{*}{Filler Gap} & \multirow{1}{*}{Which bikes is John fixing? Which is John fixing bikes?} \\
     &  &   &  &  \\
     \cline{3-5}
    &    &  \multirow{2}{*}{Filler Gap} &  \multirow{2}{*}{Comparing probabilty} & \multirow{1}{*}{Which bikes is John fixing? Which is John fixing bikes?} \\
    &    &    &    & \multirow{1}{*}{Which bikes is John fixing? Which is John fixing bikes?} \\
    &    &  \multirow{2}{*}{Irregular Forms} &   \multirow{2}{*}{Comparing probabilty} & \multirow{2}{*}{Which bikes is John fixing? Which is John fixing bikes?} \\
    &    &  \multirow{2}{*}{Determiner} &  \multirow{2}{*}{Comparing probabilty}  & \multirow{2}{*}{Which bikes is John fixing? Which is John fixing bikes?} \\
    &    &  \multirow{2}{*}{NPI Licensing} &  \multirow{2}{*}{Filler Gap}  & \multirow{2}{*}{Which bikes is John fixing? Which is John fixing bikes?} \\
    \hline
    \multirow{5}{*}{\lama} & \multirow{5}{*}{Factual} &  \multirow{2}{*}{Google RE} & \multirow{2}{*}{Filler Gap} & 
      \multirow{2}{*}{Which bikes is John fixing? Which is John fixing bikes?} \\
        & &  \multirow{2}{*}{T-REx} & \multirow{2}{*}{Filler Gap} & 
      \multirow{2}{*}{Which bikes is John fixing? Which is John fixing bikes?} \\
        & &  \multirow{2}{*}{SQuAD} & \multirow{2}{*}{Filler Gap} & 
      \multirow{2}{*}{Which bikes is John fixing? Which is John fixing bikes?} \\
      \cline{2-5}
      & &  \multirow{2}{*}{ConceptNet} & \multirow{2}{*}{Filler Gap} & 
      \multirow{2}{*}{Which bikes is John fixing? Which is John fixing bikes?} \\
    \cline{1-1}
    \multirow{3}{*}{ \cat} 
        & Commonsense & Argument Reasoning Comprehension &     \\
        &   &     Sense Making & \\
         &   &    Conjunction Acceptability  & & \\
         & &  Situations With Adversarial Generations & &  \\
         & &  Winograd Schema Challenge & & The trophy doesn’t fit into the brown suitcase because the trophy is too large.  \\
    \hline
    \multirow{3}{*}{ \olmpics} 
        & Reasoning &   &   \\
        &  &   &   \\
    \bottomrule
    \end{tabular}
    \caption{A table demonstrating the expected behavior of the chosen probes. 
    In the table, $\mathcal{C}$ denotes the context (e.g., unmasked tokens) of the masked token; $\mathbb{P}$ denotes a probe-specific scoring function (parameterized by PTLM) of the input (e.g., a token or a sentence); $V_{\text{PTLM}}$ denotes a subset of \roberta vocabulary that excludes sub-tokens.}
    \label{tab:examples-main}
\end{table*}

==> tables/older_tab_probe_examples_main.tex <==
\begin{table*}[thb]
    \tiny
    \centering\renewcommand\cellalign{lc}
    \setlength\tabcolsep{2.5pt}
    \setcellgapes{4pt}\makegapedcells
    % \def\arraystretch{0.5}
    \begin{tabular}{c|c|c|c} 
    \toprule
    \textbf{Knowledge} & \textbf{Task} & \textbf{Input} & \textbf{Output} \\ 
    \hline
    % $[\text{The}]_{\textbf{\text{NP/N}}}\; [\text{market}]_{\textbf{\text{N}}}\; [\text{crumbled}]_{\text{S\textbackslash NP}} [\text{.}]_\text{.}$
    \multirow{20}{*}{Linguistic} 
        & \begin{tabular}{@{}c@{}} Token Labeling in \cwr \\ (e.g. CCG supertagging) \end{tabular} & \textcolor{blue}{The} \textcolor{red}{market} crumbled \textcolor{green}{.} & \textbf{\textcolor{blue}{NP/N}} \textbf{\textcolor{red}{N}} \textbf{S\textbackslash NP} \textbf{\textcolor{green}{.}} \\
        \cline{2-4}
        & \begin{tabular}{@{}c@{}} Segmentation in \cwr \\ (e.g. Conjunct \\ Identification) \end{tabular} & They were 103 or 206 . &  \begin{tabular}{@{}c@{}} O O I O I O  \\ (using IO tags) \end{tabular} \\
        % \cline{2-4}
        % & Conjunct Identification & $[\text{They were}]_{\text{O}} [\text{103}]_{\text{I}} [\text{or}]_{\text{O}} [\text{206}]_{\text{I}} $\\
        \cline{2-4}
        & \begin{tabular}{@{}c@{}} Pairwise Relation in \cwr \\ (e.g. Semantic Arc \\ Classification) \end{tabular} & \multirow{2}{*}{\zeyu{need some drawing} } & \multirow{2}{*}{\zeyu{need some drawing}} \\
        \cline{2-4}
        & \begin{tabular}{@{}c@{}} \edge \\ (e.g. Relation \\ Classification) \end{tabular} & \begin{tabular}{@{}c@{}} The $[\text{burst}]_1$ has been caused \\by water hammer $[\text{pressure}]_2$ . \end{tabular} &  \begin{tabular}{@{}c@{}} Cause-Effect($e_2$, $e_1$) \\
        (i.e. $e_2$ cause $e_1$) \\ $e_1$ = burst, $e_2$ = pressure \end{tabular} \\ % \jungo{Explain casue-effect?} \\
        % & Semantic Arc Classification & \zeyu{need some drawing} \\
        % \cline{2-4}
        % & Event Factuality & I $[\text{love}]_{3.0}$ it.\\
        \cline{2-4}
        & \multirow{2}{*}{\begin{tabular}{@{}c@{}} \blimp \\ (e.g. Anaphor Agreement) \end{tabular}} 
            & \textbf{A.} Many girls insulted \underline{themselves}. &  \textbf{A} \\
        &   & \textbf{B.} Many girls insulted \underline{herself}. & $\because \mathbb{P}(\textbf{A}) >  \mathbb{P}(\textbf{B})$\\
    \hline
    \multirow{3}{*}{Factual} 
        & \lama & Nathan Alterman was a [MASK]. &  [MASK] = \textbf{poet}\\
        & (e.g. SQuAD)  & [MASK] $\in V_{\text{PTLM}}$ &  $\because \mathbb{P}(\textbf{poet}|\mathcal{C}) \geq \max_{v \in V_{\text{PTLM}}}\mathbb{P}(v|\mathcal{C})$ \\
    \hline
    \multirow{6}{*}{Commonsense} 
        & \lama/\numer & A nightmare is a [MASK] dream. &  [MASK] = \textbf{frightening}\\
        & (e.g. ConceptNet)  & [MASK] $\in V_{\text{PTLM}}$ &  %$\because \mathbb{P}(\textbf{frigh}...|\mathcal{C}) \geq  \max_{v \in V_{\text{PTLM}}}\mathbb{P}(v|\mathcal{C})$
        $\because \textbf{frightening} =  \argmax_{v \in \mathbb{V}} \mathbb{P}(v|\mathcal{C})$ \\
        % & \begin{tabular}{@{}c@{}} \lama \\ (e.g. ConceptNet) \end{tabular} & A nightmare is a [MASK] dream.\\
        \cline{2-4}
        & \cat & \textbf{A.} I walk to the \underline{school}. & \textbf{A} \\
        & (e.g. Sense Making) & \textbf{B.} I walk to the \underline{Moon}. & $\because \mathbb{P}(\textbf{A}) >  \mathbb{P}(\textbf{B})$ \\
    \hline
    \multirow{2}{*}{Basic Reasoning} 
        & \olmpics   & It was [MASK] hot,it was really cold. & \textbf{A} \\
        &      (e.g. Antonym Negation)      & \textbf{A. }not \;\;\; \textbf{B.} really & $\because \mathbb{P}(\textbf{A}|\mathcal{C}) >  \mathbb{P}(\textbf{B}|\mathcal{C})$\\
    \bottomrule
    \end{tabular}
    \caption{A table demonstrating the expected behavior of the chosen probes. 
    In the table, $\mathcal{C}$ denotes the context (e.g., unmasked tokens) of the masked token; $\mathbb{P}$ denotes a probe-specific scoring function (parameterized by PTLM) of the input (e.g., a token or a sentence); $V_{\text{PTLM}}$ denotes a subset of \roberta vocabulary that excludes sub-tokens.}
    \label{tab:examples-main}
\end{table*}

==> tables/tab_baselines.tex <==

\begin{table*}[thb]
    \centering\renewcommand\cellalign{lc}
    \setcellgapes{3pt}\makegapedcells
    \begin{tabular}{c|c|c|c|c} 
    \toprule
    \textbf{Knowledge} & \textbf{Probe package} & \textbf{Type} & \textbf{Lowerbound} & \textbf{Upperbound} \\ 
    \hline
    \multirow{2}{*}{Linguistic} & \cwr, \edge & Structural &  \makecell[c]{\robertaRand, Random Vectors, \\ GloVe} & \robertaOfficial \\
                                \cline{2-5}
                                & \blimp &  Behavioral & \robertaRand, Random Guess & \robertaOfficial \\
    \hline
    Factual & \lama & Behavioral &  \robertaRand, Random Guess &  \robertaOfficial\\
    \hline
    Commonsense & \makecell[c]{\lama, \cat, \\ \numer }& Behavioral &  \robertaRand, Random Guess &  \robertaOfficial\\
    \hline
    \makecell{Basic Reasoning} & \olmpics & Behavioral &  \robertaRand, Random Guess &  \robertaOfficial\\
    \bottomrule
    \end{tabular}
    \label{tab:baselines}
    \caption{\jungo{This table doesn't seem very useful to me. The rightmost two columns are almost identical.} A summary of probe package used in our framework and their \textit{empirical} lowerbound and upperbound. \robertaOfficial means probing with official \robertaAtEnd-B{\footnotesize ASE}; \robertaRand means probing with randomly initialized \robertaAtEnd-B{\footnotesize ASE}, averaged across 3 seeds. In behavioral probes, ``Random Guess" means expected accuracy by using random guess $\left(=\frac{1}{\text{No. choices}}\right)$.  ``Random Vectors" is points in space of $[-2,2]^d$\zeyu{Not remembering the range I used}, where $d$ is the dimension of GloVe.}
\end{table*}

==> tables/tab_corpus-domain.tex <==
\begin{table*} % [ht!]
\centering
\begin{tabular}{llll}
\toprule
\textbf{Domain} & \textbf{Pretraining Corpus} & \textbf{\# Token} & \textbf{Size} \\
\hline
\wiki & \wiki English used for BERT & 2.50B & 12GB \\
% \book & \bookcorpus \citep{bookcorpus-dataset} & 0.8B  & 4GB \\
\book & \stories \citep{stories-dataset} & N/A & 31GB \\
\news & 11.90M articles from \realnews \citep{realnews-dataset} & 6.66B & 120GB \\
\hline
\roberta & Datasets used for \citet{liu_roberta:_2019} (see Appendix \textsection \ref{appendix:roberta-corpus}) &  N/A & 160GB\\
\bottomrule
\end{tabular}
\caption{List of the domain-specific unlabeled datasets utilized in this paper. \jungo{}}
\label{tab:corpus-domain}
\end{table*}

==> tables/tab_finetuning_carbon_cost.tex <==

\begin{table*}[thb]
\small
\setlength\tabcolsep{8pt}   % Column separation
\def\arraystretch{1.8}      % row separation

\begin{tabular}{c|c|c}
\toprule
\textbf{Finetuning Task} & \textbf{Carbon Footprint (g CO2e)} & \textbf{Energy Needed (kWh)} \\
\cline{1-3}
CoLA                     & 16.15  & 0.04   \\
SST-2                          & 141.25  & 0.32   \\
MNLI                          & 726.4  & 1.6   \\
WNLI     & 4.03  & 0.0089   \\
MRPC & 8.07  & 0.0178   \\
SQuAD                        & 364.68  & 0.81    \\
ReCoRD              & 2659.41  & 5.88   \\
WSC                  & 7.24   & 0.012  \\
\bottomrule
Total                      & 54981.22  & 121.6418 \\
\bottomrule
\end{tabular}

\caption{For every finetuning tasks, we report their Carbon Footprint (g CO2e) and Energy Needed (kWh) for one single run. We ran those finetuning tasks with 14 checkpoints and include the estimated total cost in the bottom line.}
\label{tab:finetuning-carbon-cost}
\end{table*}


==> tables/tab_learning_patterns.tex <==

\begin{table}[thb]
    \centering\renewcommand\cellalign{lc}
    \setcellgapes{3pt}\makegapedcells
    \begin{tabular}{|c|c|c|} 
    \hline
    \textbf{Type} & \textbf{Speed} & \textbf{Domain} \\ 
    \hline
    Ling. & \makecell{i) Early in training \\ ii) within a short interval} & Independent \\
    \hline
    Factual & Epoch by epoch & Dependent\\
    \hline
    Comm. & Epoch by epoch & Independent\\
    \hline
    \end{tabular}
    \label{tab:learning-pattern}
    \caption{A summary of learning pattern of different kinds of knowledge}
\end{table}

==> tables/tab_probe_examples_main.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[thb]
\tiny
\setlength\tabcolsep{1.4pt}   % Column separation
\def\arraystretch{1.3}      % row separation

\begin{tabular}{c|c|c|c|ll}
\toprule
\textbf{Probe Package}            & \textbf{Knowledge}         & \textbf{Task}                                          & \textbf{Task Format  }                        & \multicolumn{2}{c}{\textbf{Examples}}                                                                                          \\
\cline{1-6}
\multirow{10}{*}{\begin{tabular}{@{}c@{}} \textbf{\texttt{Classifier}} \\ \textbf{\texttt{probing}} \end{tabular}}                        & \multirow{10}{*}{Linguistic}                   & \multirow{2}{*}{POS Tagging}                  & \multirow{2}{*}{Token Labeling}      & \multicolumn{2}{c}{\multirow{1}{*}{\begin{dependency}[style=above]
          \begin{deptext}[column sep=0.2em]
              PRON \& AUX \& VERB \& ADV \& ADP \& DET \& NOUN \& PUNCT \\
              I \& 'm \& staying \& away \& from \& the  \& stock  \& . \\
          \end{deptext}
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                            %  \cdashline{3-6}
                                             \cline{3-6}
                                             &                                                & \multirow{2}{*}{Syntactic Chunking}           & \multirow{4}{*}{\begin{tabular}{@{}c@{}} Segmentation \\  \\ \end{tabular}}      & \multicolumn{2}{c}{\multirow{1}{*}{
        \begin{dependency}[style=above]
            \begin{deptext}[column sep=0.1em]
              \graytextbf{B-NP} \& \graytextbf{B-VP} \& \graytextbf{B-PP} \& \textcolor{cyan}{\textbf{B-NP}} \& \textcolor{cyan}{\textbf{I-NP}} \& \textcolor{cyan}{\textbf{I-NP}} \& \graytextbf{O} \\
              \graytext{Shearson} \& \graytext{works} \& \graytext{at} \& \textcolor{cyan}{\textbf{American}} \& \textcolor{cyan}{\textbf{Express}} \& \textcolor{cyan}{\textbf{Co}} \& \graytext{.} \\
          \end{deptext}
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cline{3-3}
                                             \cline{5-6}
                                             &                                                & \multirow{2}{*}{Name Entity Recognition}     &       & \multicolumn{2}{c}{\multirow{1}{*}{\begin{dependency}[style=above]
            \begin{deptext}[column sep=0.2em]
              \graytextbf{O} \& \graytextbf{O} \& \textcolor{magenta}{\textbf{I-ORG}} \& \textcolor{magenta}{\textbf{I-ORG}} \& \textcolor{magenta}{\textbf{I-ORG}} \& \graytextbf{O} \& \graytextbf{O} \& \graytextbf{O} \& \graytextbf{O} \\
              \graytextbf{By} \& \graytextbf{stumps} \& \textcolor{magenta}{\textbf{Kent}} \& \textcolor{magenta}{\textbf{County}} \& \textcolor{magenta}{\textbf{Club}} \& \graytextbf{had} \& \graytextbf{reached} \& \graytextbf{108} \& \graytextbf{.} \\
          \end{deptext}
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cline{3-6}
                                             &                                                & \multirow{2}{*}{Syntactic Arc Predication} & \multirow{4}{*}{Pairwise Relations} & \multicolumn{2}{c}{\multirow{1}{*}{\begin{dependency}[edge vertical padding=-0.4ex]
          \begin{deptext} % [column sep=2em,]
              Peter \&[2em] and \& May \&[2em] bought \&[2em]  a \&[2em]  car \&[.0em] . \\
          \end{deptext}
          \deproot[edge unit distance=1.05ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted,>=}, hide label]{4}{ROOT}
          \depedge[edge unit distance=1.1ex, label style={text=lightgray,draw=lightgray},  edge style={lightgray,densely dotted,>=}, hide label]{4}{2}{\tiny Subj}
          \depedge[edge unit distance=0.8ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted,>=}, hide label]{2}{1}{\tiny Conj}
          \depedge[edge unit distance=0.8ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted,>=}, hide label]{2}{3}{\tiny Conj}
          \depedge[edge unit distance=0.3ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted,>=}, hide label]{6}{5}{\tiny Det}
        %   \depedge[edge unit distance=0.95ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted},]{4}{7}{\tiny Punct}
          \depedge[edge unit distance=0.8ex, label style={text=red}, edge style={red!60!black,thick,>=}]{3}{4}{\tiny \xmark}
          \depedge[edge unit distance=1ex, label style={text=red}, edge style={red!60!black,thick,>=}]{1}{3}{\tiny \xmark}
          \depedge[edge unit distance=0.8ex, label style={text=green,}, edge style={green!60!black,thick,>=},]{4}{6}{\tiny \boldsymbol{\cmark}} 
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cline{3-3}
                                             \cline{5-6}
                                             &                                                & \multirow{2}{*}{Syntactic Arc Classification}     &  & 
                                             \multicolumn{2}{c}{
                                             \multirow{1}{*}{\begin{dependency}[edge vertical padding=-0.4ex]
          \begin{deptext} % [column sep=2em]
            %   Peter \& and \& May \& bought \&  a \&[1em]  car \&[.1em] . \\
            Peter \&[2em] and \& May \&[2em] bought \&[2em]  a \&[2em]  car \&[.0em] . \\
          \end{deptext}
          \deproot[edge unit distance=1.05ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}, hide label]{4}{ROOT}
          \depedge[edge unit distance=1.1ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}]{4}{2}{\tiny Subj}
          \depedge[edge unit distance=0.8ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}]{2}{1}{\tiny Conj}
          \depedge[edge unit distance=0.8ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}]{2}{3}{\tiny Conj}
          \depedge[edge unit distance=0.8ex,]{4}{6}{\tiny Obj}
          \depedge[edge unit distance=0.3ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}]{6}{5}{\tiny Det}
        %   \depedge[edge unit distance=0.95ex]{4}{7}{\tiny Punct}
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cline{1-6}
\multirow{5}{*}{\blimp}                       & \multirow{5}{*}{Linguistic}                    & Island Effect                                 & \multirow{5}{*}{\begin{tabular}{@{}c@{}} Comparing \\ sentence scores \\ \textbf{Expected:} \\
$\mathbb{S}(\text{\boldsymbol{\textcolor{green}{\cmark}}}) >  \mathbb{S}(\text{\boldsymbol{\textcolor{red}{\xmark}}})$ \end{tabular}}                     & \boldsymbol{\textcolor{green}{\cmark}} Which \textit{\textbf{bikes}} is John fixing?                   & \boldsymbol{\textcolor{red}{\xmark}} Which is John fixing \textit{\textbf{bikes}}?                             \\
                                            %  \cdashline{3-3}
                                            %  \cdashline{5-6}
                                             &                                                & Filler Gap                                    &                      & \boldsymbol{\textcolor{green}{\cmark}} Brett knew \textit{\textbf{what}} many waiters find.                          & \boldsymbol{\textcolor{red}{\xmark}} Brett knew \textit{\textbf{that}} many waiters find.                      \\
                                            %  \cdashline{3-3}
                                            %  \cdashline{5-6}
                                             &                                                & Irregular Forms                               &                 &  \boldsymbol{\textcolor{green}{\cmark}} Aaron \textit{\textbf{broke}} the unicycle.                                   & \boldsymbol{\textcolor{red}{\xmark}} Aaron \textit{\textbf{broken}} the unicycle.                              \\
                                            %  \cdashline{3-3}
                                            %  \cdashline{5-6}
                                             &                                                & Determiner                                    &                     & \boldsymbol{\textcolor{green}{\cmark}} Rachelle had bought that \textit{\textbf{chair}}                             & \boldsymbol{\textcolor{red}{\xmark}} Rachelle had bought that \textit{\textbf{chairs}}.                        \\
                                            %  \cdashline{3-3}
                                            %  \cdashline{5-6}
                                             &                                                & NPI Licensing                                 &                      & \boldsymbol{\textcolor{green}{\cmark}} The truck has \textit{\textbf{clearly}}  tipped over                          & \boldsymbol{\textcolor{red}{\xmark}} The truck has \textit{\textbf{ever}} tipped over                          \\
                                             \cline{1-6}
\multirow{4}{*}{\lama}                        & \multirow{3}{*}{Factual}        & Google RE                                     & \multirow{4}{*}{\begin{tabular}{@{}c@{}}Fill-in [MASK] \\ \textbf{Expected:} \\ $\forall w \in V_{\text{PTLM}} / \{\text{\boldsymbol{\textcolor{green}{\cmark}}}\},$ \\ $\mathbb{P}(\text{\boldsymbol{\textcolor{green}{\cmark}}}\mid \mathcal{C}) >  \mathbb{P}(w\mid \mathcal{C})$ \\ \end{tabular}}                 & \multicolumn{2}{l}{Albert Einstein was born in \textit{\textbf{{[}MASK{]}}}       \hfill \boldsymbol{\textcolor{green}{\cmark}}: \textit{\textbf{{[}MASK{]}}} $= 1879$ }                            \\
                                            %  \cdashline{3-3}
                                            %  \cdashline{5-6}
                                             &                                                & T-REx                                         &                   & \multicolumn{2}{l}{Humphrey Cobb was a \textit{\textbf{{[}MASK{]}}} and novelist     \hfill \boldsymbol{\textcolor{green}{\cmark}}: \textit{\textbf{{[}MASK{]}}} $= \text{screenwriter}$ }                            \\
                                            %  \cdashline{3-3}
                                            %  \cdashline{5-6}
                                             &                                                & SQuAD                                         &                   & \multicolumn{2}{l}{A significant minority of in Warsaw were \textit{\textbf{{[}MASK{]}}}  \hfill \boldsymbol{\textcolor{green}{\cmark}}: \textit{\textbf{{[}MASK{]}}} $ = \text{Jewish}$ }                       \\
                                             \cdashline{2-3}
                                             \cdashline{5-6}
                                             &   \multirow{1}{*}{Commonsense}       & ConceptNet                                    &                   & \multicolumn{2}{l}{You can use \textit{\textbf{{[}MASK{]}}} to bathe your dog.    \hfill \boldsymbol{\textcolor{green}{\cmark}}: \textit{\textbf{{\textbf{[}MASK{]}}}} $= \text{shampoo}$ }                                \\
                                             \cline{1-6}
\multirow{11}{*}{\cat}                         & 
\multirow{11}{*}{Commonsense}                   & Conjunction Acceptability                     & \multirow{11}{*}{
\begin{tabular}{@{}c@{}} Comparing \\ sentence scores \\ \textbf{Expected:} \\
$\forall \text{\boldsymbol{\textcolor{red}{\xmark}}}, \mathbb{S}(\text{\boldsymbol{\textcolor{green}{\cmark}}}) >  \mathbb{S}(\text{\boldsymbol{\textcolor{red}{\xmark}}})$ \end{tabular}}                      & \boldsymbol{\textcolor{green}{\cmark}} Jim yelled at Kevin  \textit{\textbf{because}} Jim was so upset. & \boldsymbol{\textcolor{red}{\xmark}} Jim yelled at Kevin \textit{\textbf{and}}  Jim was so upset.                                                                                                  \\
                                            \cdashline{3-3}
                                            \cdashline{5-6}
                                             &                                                & Winograd                     &                     & \boldsymbol{\textcolor{green}{\cmark}} The fish ate the worm. The \textit{\textbf{fish}} was hungry.  & \boldsymbol{\textcolor{red}{\xmark}} The fish ate the worm. The \textit{\textbf{worm}} was hungry.                                                                                                  \\
                                             \cdashline{3-3}
                                             \cdashline{5-6}
                                             &                                                & Sense Making                                  &                      & \boldsymbol{\textcolor{green}{\cmark}} Money can be used for buying \textit{\textbf{cars}}. & \boldsymbol{\textcolor{red}{\xmark}} Money can be used for buying \textit{\textbf{stars}}.                                                                                      \\
                                             \cdashline{3-3}
                                             \cdashline{5-6}
                                             &                                                & \multirow{4}{*}{SWAG}      &                      & \multicolumn{2}{l}{\boldsymbol{\textcolor{green}{\cmark}} Someone unlocks the door and they go in. \textit{\textbf{Someone leads the way in}}.}\\
                                             &                                                &                &                       &    \multicolumn{2}{l}{\boldsymbol{\textcolor{red}{\xmark}} Someone unlocks the door and they go in. \textit{\textbf{Someone opens the door and walks out}}.}\\
                                             &                                                &                &                       &    \multicolumn{2}{l}{\boldsymbol{\textcolor{red}{\xmark}} Someone unlocks the door and they go in. \textit{\textbf{Someone walks out of the driveway}}. }\\
                                             &                                                &                &                       &    \multicolumn{2}{l}{\boldsymbol{\textcolor{red}{\xmark}} Someone unlocks the door and they go in. \textit{\textbf{Someone walks next to someone and sits on a pew.}}}\\
                                             \cdashline{3-3}
                                             \cdashline{5-6}
                                             &                                                &  \multirow{4}{*}{Argument Reasoning}              &                     &   \multicolumn{2}{l}{
                                             \boldsymbol{\textcolor{green}{\cmark}} People can choose not to use Google, \textit{\textbf{and since all other search engines re-direct to Google}}, }    \\
                                             &                                                &                 &                     &  \multicolumn{2}{l}{\;\;\;  Google is not a harmful monopoly.}      \\
                                             &                                                &                 &                     &   \multicolumn{2}{l}{
                                             \boldsymbol{\textcolor{red}{\xmark}} People can choose not to use Google, \textit{\textbf{but since other search engines do not re-direct to Google}}, }    \\
                                             &                                                &                 &                     &  \multicolumn{2}{l}{\;\; Google is not a harmful monopoly.}      \\
                                             \cline{1-6}
\multirow{5}{*}{\olmpics} & \multirow{5}{*}{Reasoning} & Taxonomy Conjunction                          & \multirow{5}{*}{\begin{tabular}{@{}c@{}}Fill-in [MASK] \\ \textbf{Expected:} $\forall \text{\boldsymbol{\textcolor{red}{\xmark}}},$ \\ $\mathbb{P}(\text{\boldsymbol{\textcolor{green}{\cmark}}}\mid \mathcal{C}) >  \mathbb{P}(\text{\boldsymbol{\textcolor{red}{\xmark}}}\mid \mathcal{C})$ \end{tabular}}                 & \multicolumn{2}{l}{A ferry and a floatplane are both a type of \textit{\textbf{{[}MASK{]}}}.  \hfill \boldsymbol{\textcolor{green}{\cmark}} vehicle \boldsymbol{\textcolor{red}{\xmark}} airplane \boldsymbol{\textcolor{red}{\xmark}} boat}            \\
                        % \cdashline{3-3}
                        % \cdashline{5-6}
                         &                            & Age Comparison                                &                  & \multicolumn{2}{l}{A 21 year old person age is \textit{\textbf{{[}MASK{]}}} than a 35 year old person.  \hfill  \boldsymbol{\textcolor{green}{\cmark}} younger \boldsymbol{\textcolor{red}{\xmark}} older}             \\
                        %  \cdashline{3-3}
                        % \cdashline{5-6}
                         &                            & Object Comparison                             &                  & \multicolumn{2}{l}{The size of a airplane is usually much \textit{\textbf{{[}MASK{]}}} than the size of a house.  \hfill  \boldsymbol{\textcolor{red}{\xmark}} smaller \boldsymbol{\textcolor{green}{\cmark}} larger}              \\
                        %  \cdashline{3-3}
                        % \cdashline{5-6}
                         &                            & Always-Never                                  &                  & \multicolumn{2}{l}{A chicken \textit{\textbf{{[}MASK{]}}} has horns.  \hfill  \boldsymbol{\textcolor{green}{\cmark}} never \boldsymbol{\textcolor{red}{\xmark}} rarely \boldsymbol{\textcolor{red}{\xmark}} sometimes \boldsymbol{\textcolor{red}{\xmark}} often \boldsymbol{\textcolor{red}{\xmark}} always}                \\
                        %  \cdashline{3-3}
                        % \cdashline{5-6}
                         &                            & Multi-Hop Composition                         &                  & \multicolumn{2}{l}{When comparing a 23, a 38 and a 31 year old, the \textit{\textbf{{[}MASK{]}}} is oldest. \hfill  \boldsymbol{\textcolor{green}{\cmark}} second \boldsymbol{\textcolor{red}{\xmark}} first \boldsymbol{\textcolor{red}{\xmark}} third}
\\ 
\bottomrule
\end{tabular}

\caption{$\mathcal{C}$ is the context, $\mathbb{P}(\cdot \mid \mathcal{C})$ is the probability over the vocabulary given the context; specific to different probe packages, $\mathbb{S}(\cdot)$ is some scoring function based on probability of words in sentence. $V_{\text{PTLM}}$ is the vocabulary of the PTLM that are grammatical words or numbers}
\label{tab:examples-main}
\end{table*}

==> tables/tab_probe_examples_main_morelines+taskmodified.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[thb]
\tiny
\setlength\tabcolsep{1.4pt}   % Column separation
\def\arraystretch{1.3}      % row separation

\begin{tabular}{c|c|c|c|ll}
\toprule
\textbf{Probe Package}            & \textbf{Knowledge}         & \textbf{Task Format}                                          & \textbf{Task   }                        & \multicolumn{2}{c}{\textbf{Examples}}                                                                                          \\
\cline{1-6}
\multirow{10}{*}{\begin{tabular}{@{}c@{}} \textbf{\texttt{Classifier}} \\ \textbf{\texttt{probing}} \end{tabular}}                        & \multirow{10}{*}{Linguistic}                         & \multirow{2}{*}{Token Labeling}           & \multirow{2}{*}{POS Tagging}       & \multicolumn{2}{c}{\multirow{1}{*}{\begin{dependency}[style=above]
          \begin{deptext}[column sep=0.2em]
              PRON \& AUX \& VERB \& ADV \& ADP \& DET \& NOUN \& PUNCT \\
              I \& 'm \& staying \& away \& from \& the  \& stock  \& . \\
          \end{deptext}
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cdashline{3-6}
                                            %  \cline{3-6}
                                             &              & \multirow{4}{*}{\begin{tabular}{@{}c@{}} Segmentation \\ {[}Annotation has some \\ notion of segmentation{]} \\ \end{tabular}}                                   & \multirow{2}{*}{Syntactic Chunking}                & \multicolumn{2}{c}{\multirow{1}{*}{
        \begin{dependency}[style=above]
            \begin{deptext}[column sep=0.1em]
              \graytextbf{B-NP} \& \graytextbf{B-VP} \& \graytextbf{B-PP} \& \textcolor{cyan}{\textbf{B-NP}} \& \textcolor{cyan}{\textbf{I-NP}} \& \textcolor{cyan}{\textbf{I-NP}} \& \graytextbf{O} \\
              \graytext{Shearson} \& \graytext{works} \& \graytext{at} \& \textcolor{cyan}{\textbf{American}} \& \textcolor{cyan}{\textbf{Express}} \& \textcolor{cyan}{\textbf{Co}} \& \graytext{.} \\
          \end{deptext}
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cdashline{4-6}
                                             &                &                                      & \multirow{2}{*}{Name Entity Recognition}      & \multicolumn{2}{c}{\multirow{1}{*}{\begin{dependency}[style=above]
            \begin{deptext}[column sep=0.2em]
              \graytextbf{O} \& \graytextbf{O} \& \textcolor{magenta}{\textbf{I-ORG}} \& \textcolor{magenta}{\textbf{I-ORG}} \& \textcolor{magenta}{\textbf{I-ORG}} \& \graytextbf{O} \& \graytextbf{O} \& \graytextbf{O} \& \graytextbf{O} \\
              \graytextbf{By} \& \graytextbf{stumps} \& \textcolor{magenta}{\textbf{Kent}} \& \textcolor{magenta}{\textbf{County}} \& \textcolor{magenta}{\textbf{Club}} \& \graytextbf{had} \& \graytextbf{reached} \& \graytextbf{108} \& \graytextbf{.} \\
          \end{deptext}
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cdashline{3-6}
                                             &                                                & \multirow{4}{*}{Pair Relations} & \multirow{2}{*}{Syntactic Arc Predication} & \multicolumn{2}{c}{\multirow{1}{*}{\begin{dependency}[edge vertical padding=-0.4ex]
          \begin{deptext} % [column sep=2em,]
              Peter \&[2em] and \& May \&[2em] bought \&[2em]  a \&[2em]  car \&[.0em] . \\
          \end{deptext}
          \deproot[edge unit distance=1.05ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted,>=}, hide label]{4}{ROOT}
          \depedge[edge unit distance=1.1ex, label style={text=lightgray,draw=lightgray},  edge style={lightgray,densely dotted,>=}, hide label]{4}{2}{\tiny Subj}
          \depedge[edge unit distance=0.8ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted,>=}, hide label]{2}{1}{\tiny Conj}
          \depedge[edge unit distance=0.8ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted,>=}, hide label]{2}{3}{\tiny Conj}
          \depedge[edge unit distance=0.3ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted,>=}, hide label]{6}{5}{\tiny Det}
        %   \depedge[edge unit distance=0.95ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted},]{4}{7}{\tiny Punct}
          \depedge[edge unit distance=0.8ex, label style={text=red}, edge style={red!60!black,thick,>=}]{3}{4}{\tiny \xmark}
          \depedge[edge unit distance=1ex, label style={text=red}, edge style={red!60!black,thick,>=}]{1}{3}{\tiny \xmark}
          \depedge[edge unit distance=0.8ex, label style={text=green,}, edge style={green!60!black,thick,>=},]{4}{6}{\tiny \boldsymbol{\cmark}} 
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cdashline{4-6}
                                             &                                                &  & \multirow{2}{*}{Syntactic Arc Classification}     & 
                                             \multicolumn{2}{c}{
                                             \multirow{1}{*}{\begin{dependency}[edge vertical padding=-0.4ex]
          \begin{deptext} % [column sep=2em]
            %   Peter \& and \& May \& bought \&  a \&[1em]  car \&[.1em] . \\
            Peter \&[2em] and \& May \&[2em] bought \&[2em]  a \&[2em]  car \&[.0em] . \\
          \end{deptext}
          \deproot[edge unit distance=1.05ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}, hide label]{4}{ROOT}
          \depedge[edge unit distance=1.1ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}]{4}{2}{\tiny Subj}
          \depedge[edge unit distance=0.8ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}]{2}{1}{\tiny Conj}
          \depedge[edge unit distance=0.8ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}]{2}{3}{\tiny Conj}
          \depedge[edge unit distance=0.8ex,]{4}{6}{\tiny Obj}
          \depedge[edge unit distance=0.3ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}]{6}{5}{\tiny Det}
        %   \depedge[edge unit distance=0.95ex]{4}{7}{\tiny Punct}
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cline{1-6}
\multirow{5}{*}{\blimp}                       & \multirow{5}{*}{Linguistic}                          & \multirow{5}{*}{\begin{tabular}{@{}c@{}} Comparing \\ sentence scores \\ \textbf{Expected:} \\
$\mathbb{S}(\text{\boldsymbol{\textcolor{green}{\cmark}}}) >  \mathbb{S}(\text{\boldsymbol{\textcolor{red}{\xmark}}})$ \end{tabular}} & Island Effect                                               
& \boldsymbol{\textcolor{green}{\cmark}} Which \textit{\textbf{bikes}} is John fixing?                   & \boldsymbol{\textcolor{red}{\xmark}} Which is John fixing \textit{\textbf{bikes}}?                             \\
                                             \cdashline{4-6}
                                             &                                 &                                   & Filler Gap                                      & \boldsymbol{\textcolor{green}{\cmark}} Brett knew \textit{\textbf{what}} many waiters find.                          & \boldsymbol{\textcolor{red}{\xmark}} Brett knew \textit{\textbf{that}} many waiters find.                      \\
                                             \cdashline{4-6}
                                             &                        &                              & Irregular Forms                                          &  \boldsymbol{\textcolor{green}{\cmark}} Aaron \textit{\textbf{broke}} the unicycle.                                   & \boldsymbol{\textcolor{red}{\xmark}} Aaron \textit{\textbf{broken}} the unicycle.                              \\
                                             \cdashline{4-6}
                                             &                      &                                     & Determiner                                              & \boldsymbol{\textcolor{green}{\cmark}} Rachelle had bought that \textit{\textbf{chair}}                             & \boldsymbol{\textcolor{red}{\xmark}} Rachelle had bought that \textit{\textbf{chairs}}.                        \\
                                             \cdashline{4-6}
                                             &                          &                                      & NPI Licensing                                       & \boldsymbol{\textcolor{green}{\cmark}} The truck has \textit{\textbf{clearly}}  tipped over                          & \boldsymbol{\textcolor{red}{\xmark}} The truck has \textit{\textbf{ever}} tipped over                          \\
                                             \cline{1-6}
\multirow{4}{*}{\lama}                        & \multirow{3}{*}{Factual}        & \multirow{4}{*}{\begin{tabular}{@{}c@{}}Fill-in [MASK] \\ \textbf{Expected:} \\ $\forall w \in V_{\text{PTLM}} / \{\text{\boldsymbol{\textcolor{green}{\cmark}}}\},$ \\ $\mathbb{P}(\text{\boldsymbol{\textcolor{green}{\cmark}}}\mid \mathcal{C}) >  \mathbb{P}(w\mid \mathcal{C})$ \\ \end{tabular}}                  & Google RE                                    & \multicolumn{2}{l}{Albert Einstein was born in \textit{\textbf{{[}MASK{]}}}       \hfill \boldsymbol{\textcolor{green}{\cmark}}: \textit{\textbf{{[}MASK{]}}} $= 1879$ }                            \\
                        \cdashline{4-6}
                                             &                                                &                   & T-REx                                         & \multicolumn{2}{l}{Humphrey Cobb was a \textit{\textbf{{[}MASK{]}}} and novelist     \hfill \boldsymbol{\textcolor{green}{\cmark}}: \textit{\textbf{{[}MASK{]}}} $= \text{screenwriter}$ }                            \\
                        \cdashline{4-6}
                                             &                                                &                   & SQuAD                                         & \multicolumn{2}{l}{A significant minority of in Warsaw were \textit{\textbf{{[}MASK{]}}}  \hfill \boldsymbol{\textcolor{green}{\cmark}}: \textit{\textbf{{[}MASK{]}}} $ = \text{Jewish}$ }                       \\
                        \cdashline{2-2}
                        \cdashline{4-6}
                                             &   \multirow{1}{*}{Commonsense}       &                   & ConceptNet                                    & \multicolumn{2}{l}{You can use \textit{\textbf{{[}MASK{]}}} to bathe your dog.    \hfill \boldsymbol{\textcolor{green}{\cmark}}: \textit{\textbf{{\textbf{[}MASK{]}}}} $= \text{shampoo}$ }                                \\
                                             \cline{1-6}
\multirow{11}{*}{\cat}                         & 
\multirow{11}{*}{Commonsense}                   & \multirow{11}{*}{
\begin{tabular}{@{}c@{}} Comparing \\ sentence scores \\ \textbf{Expected:} \\
$\forall \text{\boldsymbol{\textcolor{red}{\xmark}}s}, \mathbb{S}(\text{\boldsymbol{\textcolor{green}{\cmark}}}) >  \mathbb{S}(\text{\boldsymbol{\textcolor{red}{\xmark}}})$ \end{tabular}}                      & Conjunction Acceptability                     & \boldsymbol{\textcolor{green}{\cmark}} Jim yelled at Kevin  \textit{\textbf{because}} Jim was so upset. & \boldsymbol{\textcolor{red}{\xmark}} Jim yelled at Kevin \textit{\textbf{and}}  Jim was so upset.                                                                                                  \\
                        \cdashline{4-6}
                                             &                                                &                     & Winograd                     & \boldsymbol{\textcolor{green}{\cmark}} The fish ate the worm. The \textit{\textbf{fish}} was hungry.  & \boldsymbol{\textcolor{red}{\xmark}} The fish ate the worm. The \textit{\textbf{worm}} was hungry.                                                                                                  \\
                        \cdashline{4-6}
                                             &                                                &                      & Sense Making                                  & \boldsymbol{\textcolor{green}{\cmark}} Money can be used for buying \textit{\textbf{cars}}. & \boldsymbol{\textcolor{red}{\xmark}} Money can be used for buying \textit{\textbf{stars}}.                                                                                      \\
                        \cdashline{4-6}
                                             &                                                &                      & \multirow{4}{*}{SWAG}      & \multicolumn{2}{l}{\boldsymbol{\textcolor{green}{\cmark}} Someone unlocks the door and they go in. \textit{\textbf{Someone leads the way in}}.}\\
                                             &                                                &                &                       &    \multicolumn{2}{l}{\boldsymbol{\textcolor{red}{\xmark}} Someone unlocks the door and they go in. \textit{\textbf{Someone opens the door and walks out}}.}\\
                                             &                                                &                &                       &    \multicolumn{2}{l}{\boldsymbol{\textcolor{red}{\xmark}} Someone unlocks the door and they go in. \textit{\textbf{Someone walks out of the driveway}}. }\\
                                             &                                                &                &                       &    \multicolumn{2}{l}{\boldsymbol{\textcolor{red}{\xmark}} Someone unlocks the door and they go in. \textit{\textbf{Someone walks next to someone and sits on a pew.}}}\\
                        \cdashline{4-6}
                                             &                                                &                     &  \multirow{4}{*}{Argument Reasoning}              &   \multicolumn{2}{l}{
                                             \boldsymbol{\textcolor{green}{\cmark}} People can choose not to use Google, \textit{\textbf{and since all other search engines re-direct to Google}}, }    \\
                                             &                                                &                 &                     &  \multicolumn{2}{l}{\;\;\;  Google is not a harmful monopoly.}      \\
                                             &                                                &                 &                     &   \multicolumn{2}{l}{
                                             \boldsymbol{\textcolor{red}{\xmark}} People can choose not to use Google, \textit{\textbf{but since other search engines do not re-direct to Google}}, }    \\
                                             &                                                &                 &                     &  \multicolumn{2}{l}{\;\; Google is not a harmful monopoly.}      \\
                                             \cline{1-6}
\multirow{5}{*}{\olmpics} & \multirow{5}{*}{Reasoning}            & \multirow{5}{*}{\begin{tabular}{@{}c@{}}Fill-in [MASK] \\ \textbf{Expected:} $\forall \text{\boldsymbol{\textcolor{red}{\xmark}}s},$ \\ $\mathbb{P}(\text{\boldsymbol{\textcolor{green}{\cmark}}}\mid \mathcal{C}) >  \mathbb{P}(\text{\boldsymbol{\textcolor{red}{\xmark}}}\mid \mathcal{C})$ \end{tabular}}      & Taxonomy Conjunction                          & \multicolumn{2}{l}{A ferry and a floatplane are both a type of \textit{\textbf{{[}MASK{]}}}.  \hfill \boldsymbol{\textcolor{green}{\cmark}} vehicle \boldsymbol{\textcolor{red}{\xmark}} airplane \boldsymbol{\textcolor{red}{\xmark}} boat}            \\
                        \cdashline{4-6}
                         &              &                        & Age Comparison                                        & \multicolumn{2}{l}{A 21 year old person age is \textit{\textbf{{[}MASK{]}}} than a 35 year old person.  \hfill  \boldsymbol{\textcolor{green}{\cmark}} younger \boldsymbol{\textcolor{red}{\xmark}} older}             \\
                        \cdashline{4-6}
                         &                     &                  & Object Comparison                      & \multicolumn{2}{l}{The size of a airplane is usually much \textit{\textbf{{[}MASK{]}}} than the size of a house.  \hfill  \boldsymbol{\textcolor{red}{\xmark}} smaller \boldsymbol{\textcolor{green}{\cmark}} larger}              \\
                        \cdashline{4-6}
                         &                             &                          & Always-Never                         & \multicolumn{2}{l}{A chicken \textit{\textbf{{[}MASK{]}}} has horns.  \hfill  \boldsymbol{\textcolor{green}{\cmark}} never \boldsymbol{\textcolor{red}{\xmark}} rarely \boldsymbol{\textcolor{red}{\xmark}} sometimes \boldsymbol{\textcolor{red}{\xmark}} often \boldsymbol{\textcolor{red}{\xmark}} always}                \\
                        \cdashline{4-6}
                         &                             &                  & Multi-Hop Composition                        & \multicolumn{2}{l}{When comparing a 23, a 38 and a 31 year old, the \textit{\textbf{{[}MASK{]}}} is oldest. \hfill  \boldsymbol{\textcolor{green}{\cmark}} second \boldsymbol{\textcolor{red}{\xmark}} first \boldsymbol{\textcolor{red}{\xmark}} third}
\\ 
\bottomrule
\end{tabular}

\caption{$\mathcal{C}$ is the context, $\mathbb{P}(\cdot \mid \mathcal{C})$ is the probability over the vocabulary given the context; specific to different probe packages, $\mathbb{S}(\cdot)$ is some scoring function based on probability of words in sentence. $V_{\text{PTLM}}$ is the vocabulary of the PTLM that are grammatical words or numbers}
\label{tab:examples-main}
\end{table*}

==> tables/tab_probe_examples_main_taskmodified.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[thb]
\tiny
\setlength\tabcolsep{1.4pt}   % Column separation
\def\arraystretch{1.2}      % row separation

\begin{tabular}{c|c|c|c|ll}
\toprule
\textbf{Probe Package}              & \textbf{Knowledge}                  & \textbf{Task Format}                               & \textbf{Task}                        & \multicolumn{2}{c}{\textbf{Examples}}                                                                                          \\
\cline{1-6}
\multirow{10}{*}{\begin{tabular}{@{}c@{}} \cwr  \end{tabular}}                        & \multirow{10}{*}{Linguistic}                         & \multirow{2}{*}{Token Labeling}           & \multirow{2}{*}{POS Tagging}       & \multicolumn{2}{c}{\multirow{1}{*}{\begin{dependency}[style=above]
          \begin{deptext}[column sep=0.2em]
              PRON \& AUX \& VERB \& ADV \& ADP \& DET \& NOUN \& PUNCT \\
              I \& 'm \& staying \& away \& from \& the  \& stock  \& . \\
          \end{deptext}
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                            %  \cdashline{3-6}
                                             \cline{3-6}
                                             &              & \multirow{4}{*}{\begin{tabular}{@{}c@{}} Segmentation \\ {[}Annotation has some \\ notion of segmentation{]} \\ \end{tabular}}                                   & \multirow{2}{*}{Syntactic Chunking}                & \multicolumn{2}{c}{\multirow{1}{*}{
        \begin{dependency}[style=above]
            \begin{deptext}[column sep=0.1em]
              \graytextbf{B-NP} \& \graytextbf{B-VP} \& \graytextbf{B-PP} \& \textcolor{cyan}{\textbf{B-NP}} \& \textcolor{cyan}{\textbf{I-NP}} \& \textcolor{cyan}{\textbf{I-NP}} \& \graytextbf{O} \\
              \graytext{Shearson} \& \graytext{works} \& \graytext{at} \& \textcolor{cyan}{\textbf{American}} \& \textcolor{cyan}{\textbf{Express}} \& \textcolor{cyan}{\textbf{Co}} \& \graytext{.} \\
          \end{deptext}
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cdashline{4-6}[1pt/1pt]
                                             &                &                                      & \multirow{2}{*}{Name Entity Recognition}      & \multicolumn{2}{c}{\multirow{1}{*}{\begin{dependency}[style=above]
            \begin{deptext}[column sep=0.2em]
              \graytextbf{O} \& \graytextbf{O} \& \textcolor{magenta}{\textbf{I-ORG}} \& \textcolor{magenta}{\textbf{I-ORG}} \& \textcolor{magenta}{\textbf{I-ORG}} \& \graytextbf{O} \& \graytextbf{O} \& \graytextbf{O} \& \graytextbf{O} \\
              \graytextbf{By} \& \graytextbf{stumps} \& \textcolor{magenta}{\textbf{Kent}} \& \textcolor{magenta}{\textbf{County}} \& \textcolor{magenta}{\textbf{Club}} \& \graytextbf{had} \& \graytextbf{reached} \& \graytextbf{108} \& \graytextbf{.} \\
          \end{deptext}
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cline{3-6}
                                             &                                                & \multirow{4}{*}{Pairwise Relations} & \multirow{2}{*}{Syntactic Arc Predication} & \multicolumn{2}{c}{\multirow{1}{*}{\begin{dependency}[edge vertical padding=-0.4ex]
          \begin{deptext} % [column sep=2em,]
              Peter \&[2em] and \& May \&[2em] bought \&[2em]  a \&[2em]  car \&[.0em] . \\
          \end{deptext}
          \deproot[edge unit distance=0.90ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted,>=}, hide label]{4}{ROOT}
          \depedge[edge unit distance=1.1ex, label style={text=lightgray,draw=lightgray},  edge style={lightgray,densely dotted,>=}, hide label]{4}{2}{\tiny Subj}
          \depedge[edge unit distance=0.8ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted,>=}, hide label]{2}{1}{\tiny Conj}
          \depedge[edge unit distance=0.8ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted,>=}, hide label]{2}{3}{\tiny Conj}
          \depedge[edge unit distance=0.3ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted,>=}, hide label]{6}{5}{\tiny Det}
        %   \depedge[edge unit distance=0.95ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted},]{4}{7}{\tiny Punct}
          \depedge[edge unit distance=0.8ex, label style={text=red}, edge style={red!60!black,thick,>=}]{3}{4}{\tiny \xmark}
          \depedge[edge unit distance=1ex, label style={text=red}, edge style={red!60!black,thick,>=}]{1}{3}{\tiny \xmark}
          \depedge[edge unit distance=0.8ex, label style={text=green,}, edge style={green!60!black,thick,>=},]{4}{6}{\tiny \boldsymbol{\cmark}} 
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cdashline{4-6}
                                             &                                                &  & \multirow{2}{*}{Syntactic Arc Classification}     & 
                                             \multicolumn{2}{c}{
                                             \multirow{1}{*}{\begin{dependency}[edge vertical padding=-0.4ex]
          \begin{deptext} % [column sep=2em]
            %   Peter \& and \& May \& bought \&  a \&[1em]  car \&[.1em] . \\
            Peter \&[2em] and \& May \&[2em] bought \&[2em]  a \&[2em]  car \&[.0em] . \\
          \end{deptext}
          \deproot[edge unit distance=0.90ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}, hide label]{4}{ROOT}
          \depedge[edge unit distance=1.1ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}]{4}{2}{\tiny Subj}
          \depedge[edge unit distance=0.8ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}]{2}{1}{\tiny Conj}
          \depedge[edge unit distance=0.8ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}]{2}{3}{\tiny Conj}
          \depedge[edge unit distance=0.8ex,]{4}{6}{\tiny Obj}
          \depedge[edge unit distance=0.3ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted}]{6}{5}{\tiny Det}
        %   \depedge[edge unit distance=0.95ex]{4}{7}{\tiny Punct}
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cline{1-6}
\multirow{5}{*}{\begin{tabular}{@{}c@{}} \blimp  \end{tabular}}                       & \multirow{5}{*}{Linguistic}                          & \multirow{5}{*}{\begin{tabular}{@{}c@{}} Comparing \\ sentence scores \\ \textbf{Expected:} \\
$\mathcal{S}(\text{\boldsymbol{\textcolor{green}{\cmark}}}) >  \mathcal{S}(\text{\boldsymbol{\textcolor{red}{\xmark}}})$ \end{tabular}} & Island Effect                                               
& \boldsymbol{\textcolor{green}{\cmark}} Which \textit{\textbf{bikes}} is John fixing?                   & \boldsymbol{\textcolor{red}{\xmark}} Which is John fixing \textit{\textbf{bikes}}?                             \\
                                            %  \cdashline{4-6}
                                             &                                 &                                   & Filler-Gap                                      & \boldsymbol{\textcolor{green}{\cmark}} Brett knew \textit{\textbf{what}} many waiters find.                          & \boldsymbol{\textcolor{red}{\xmark}} Brett knew \textit{\textbf{that}} many waiters find.                      \\
                                            %  \cdashline{4-6}
                                             &                        &                              & Irregular Forms                                          &  \boldsymbol{\textcolor{green}{\cmark}} Aaron \textit{\textbf{broke}} the unicycle.                                   & \boldsymbol{\textcolor{red}{\xmark}} Aaron \textit{\textbf{broken}} the unicycle.                              \\
                                            %  \cdashline{4-6}
                                             &                      &                                     & Determiner-Noun Agree.                                              & \boldsymbol{\textcolor{green}{\cmark}} Rachelle had bought that \textit{\textbf{chair}}                             & \boldsymbol{\textcolor{red}{\xmark}} Rachelle had bought that \textit{\textbf{chairs}}.                        \\
                                            %  \cdashline{4-6}
                                             &                          &                                      & NPI Licensing                                       & \boldsymbol{\textcolor{green}{\cmark}} The truck has \textit{\textbf{clearly}}  tipped over                          & \boldsymbol{\textcolor{red}{\xmark}} The truck has \textit{\textbf{ever}} tipped over                          \\
                                             \cline{1-6}
\multirow{4}{*}{\begin{tabular}{@{}c@{}} \lama  \end{tabular}}                        & \multirow{3}{*}{Factual}        & \multirow{4}{*}{\begin{tabular}{@{}c@{}}Fill-in [MASK] \\ \textbf{Expected:} \\ $\forall w \in V_{\text{PTLM}} / \{\text{\boldsymbol{\textcolor{green}{\cmark}}}\},$ \\ $p(\text{\boldsymbol{\textcolor{green}{\cmark}}}\mid \mathcal{C}) >  p(w\mid \mathcal{C})$ \\ \end{tabular}}                  & Google RE                                    & \multicolumn{2}{l}{Albert Einstein was born in \textit{\textbf{{[}MASK{]}}}       \hfill \boldsymbol{\textcolor{green}{\cmark}}: \textit{\textbf{{[}MASK{]}}} $= 1879$ }                            \\
                        % \cdashline{4-6}
                                             &                                                &                   & T-REx                                         & \multicolumn{2}{l}{Humphrey Cobb was a \textit{\textbf{{[}MASK{]}}} and novelist     \hfill \boldsymbol{\textcolor{green}{\cmark}}: \textit{\textbf{{[}MASK{]}}} $= \text{screenwriter}$ }                            \\
                        % \cdashline{4-6}
                                             &                                                &                   & SQuAD                                         & \multicolumn{2}{l}{A significant minority of in Warsaw were \textit{\textbf{{[}MASK{]}}}  \hfill \boldsymbol{\textcolor{green}{\cmark}}: \textit{\textbf{{[}MASK{]}}} $ = \text{Jewish}$ }                       \\
                        \cdashline{2-2}
                        \cdashline{4-6}
                                             &   \multirow{1}{*}{Commonsense}       &                   & ConceptNet                                    & \multicolumn{2}{l}{You can use \textit{\textbf{{[}MASK{]}}} to bathe your dog.    \hfill \boldsymbol{\textcolor{green}{\cmark}}: \textit{\textbf{{\textbf{[}MASK{]}}}} $= \text{shampoo}$ }                                \\
                                             \cline{1-6}
\multirow{11}{*}{\begin{tabular}{@{}c@{}} \cat  \end{tabular}}                         & 
\multirow{11}{*}{Commonsense}                   & \multirow{11}{*}{
\begin{tabular}{@{}c@{}} Comparing \\ sentence scores \\ \textbf{Expected:} \\
$\forall \text{\boldsymbol{\textcolor{red}{\xmark}}}$ \\ $\frac{\mathcal{S}(\cmark )}{|\cmark|} > \frac{\mathcal{S}(\text{\boldsymbol{\textcolor{red}{\xmark}}})}{|\text{\boldsymbol{\textcolor{red}{\xmark}}}|}$ \end{tabular}}                      & Conjunction Acceptability                     & \boldsymbol{\textcolor{green}{\cmark}} Jim yelled at Kevin  \textit{\textbf{because}} Jim was so upset. & \boldsymbol{\textcolor{red}{\xmark}} Jim yelled at Kevin \textit{\textbf{and}}  Jim was so upset.                                                                                                  \\
                        \cdashline{4-6}
                                             &                                                &                     & Winograd                     & \cmark The fish ate the worm. The \textit{\textbf{fish}} was hungry.  & \boldsymbol{\textcolor{red}{\xmark}} The fish ate the worm. The \textit{\textbf{worm}} was hungry.                                                                                                  \\
                        \cdashline{4-6}
                                             &                                                &                      & Sense Making                                  & \boldsymbol{\textcolor{green}{\cmark}} Money can be used for buying \textit{\textbf{cars}}. & \boldsymbol{\textcolor{red}{\xmark}} Money can be used for buying \textit{\textbf{stars}}.                                                                                      \\
                        \cdashline{4-6}
                                             &                                                &                      & \multirow{4}{*}{SWAG}      & \multicolumn{2}{l}{\boldsymbol{\textcolor{green}{\cmark}} Someone unlocks the door and they go in. \textit{\textbf{Someone leads the way in}}.}\\
                                             &                                                &                &                       &    \multicolumn{2}{l}{\boldsymbol{\textcolor{red}{\xmark}} Someone unlocks the door and they go in. \textit{\textbf{Someone opens the door and walks out}}.}\\
                                             &                                                &                &                       &    \multicolumn{2}{l}{\boldsymbol{\textcolor{red}{\xmark}} Someone unlocks the door and they go in. \textit{\textbf{Someone walks out of the driveway}}. }\\
                                             &                                                &                &                       &    \multicolumn{2}{l}{\boldsymbol{\textcolor{red}{\xmark}} Someone unlocks the door and they go in. \textit{\textbf{Someone walks next to someone and sits on a pew.}}}\\
                        \cdashline{4-6}
                                             &                                                &                     &  \multirow{4}{*}{Argument Reasoning}              &   \multicolumn{2}{l}{
                                             \boldsymbol{\textcolor{green}{\cmark}} People can choose not to use Google, \textit{\textbf{and since all other search engines re-direct to Google}}, }    \\
                                             &                                                &                 &                     &  \multicolumn{2}{l}{\;\;\;  Google is not a harmful monopoly.}      \\
                                             &                                                &                 &                     &   \multicolumn{2}{l}{
                                             \boldsymbol{\textcolor{red}{\xmark}} People can choose not to use Google, \textit{\textbf{but since other search engines do not re-direct to Google}}, }    \\
                                             &                                                &                 &                     &  \multicolumn{2}{l}{\;\; Google is not a harmful monopoly.}      \\
                                             \cline{1-6}
\multirow{5}{*}{\begin{tabular}{@{}c@{}} \olmpics   \end{tabular}} & \multirow{5}{*}{Reasoning}            & \multirow{5}{*}{\begin{tabular}{@{}c@{}}Fill-in [MASK] \\ \textbf{Expected:} $\forall \text{\boldsymbol{\textcolor{red}{\xmark}}},$ \\ $p(\text{\boldsymbol{\textcolor{green}{\cmark}}}\mid \mathcal{C}) >  p(\text{\boldsymbol{\textcolor{red}{\xmark}}}\mid \mathcal{C})$ \end{tabular}}      & Always-Never                         & \multicolumn{2}{l}{A chicken \textit{\textbf{{[}MASK{]}}} has horns.  \hfill  \boldsymbol{\textcolor{green}{\cmark}} never \boldsymbol{\textcolor{red}{\xmark}} rarely \boldsymbol{\textcolor{red}{\xmark}} sometimes \boldsymbol{\textcolor{red}{\xmark}} often \boldsymbol{\textcolor{red}{\xmark}} always}                \\
                        % \cdashline{4-6}
                         &              &                        & Age Comparison                                        & \multicolumn{2}{l}{A 21 year old person age is \textit{\textbf{{[}MASK{]}}} than a 35 year old person.  \hfill  \boldsymbol{\textcolor{green}{\cmark}} younger \boldsymbol{\textcolor{red}{\xmark}} older}             \\
                        % \cdashline{4-6}
                         &                     &                  & Object Comparison                      & \multicolumn{2}{l}{The size of a airplane is usually much \textit{\textbf{{[}MASK{]}}} than the size of a house.  \hfill  \boldsymbol{\textcolor{red}{\xmark}} smaller \boldsymbol{\textcolor{green}{\cmark}} larger}              \\
                        % \cdashline{4-6}
                         &                             &                          & Taxonomy Conjunction                          & \multicolumn{2}{l}{A ferry and a floatplane are both a type of \textit{\textbf{{[}MASK{]}}}.  \hfill \boldsymbol{\textcolor{green}{\cmark}} vehicle \boldsymbol{\textcolor{red}{\xmark}} airplane \boldsymbol{\textcolor{red}{\xmark}} boat}            \\
                        % \cdashline{4-6}
                         &                             &                  & Multi-Hop Composition                        & \multicolumn{2}{l}{When comparing a 23, a 38 and a 31 year old, the \textit{\textbf{{[}MASK{]}}} is oldest. \hfill  \boldsymbol{\textcolor{green}{\cmark}} second \boldsymbol{\textcolor{red}{\xmark}} first \boldsymbol{\textcolor{red}{\xmark}} third}
\\ 
\bottomrule
\end{tabular}

\caption{$\mathcal{C}$ is the context, $p(\cdot \mid \mathcal{C})$ is the probability over the vocabulary given the context; specific to different probe packages, $\mathcal{S}(\cdot)$ is some scoring function based on probability of words in sentence. $V_{\text{PTLM}}$ is the vocabulary of the PTLM that are grammatical words or numbers}
\label{tab:examples-main}
\end{table*}

==> tables/tab_probing_carbon_cost.tex <==
% \begin{table}[]
% \begin{tabular}{lrrrrrrrllll}
% Probe Name                   & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Carbon Footprint (g CO2e) From \\ GPU\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Energy Needed (kWh) From \\ GPU\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Carbon Footprint (g CO2e) From \\ CPU\end{tabular}} & \multicolumn{1}{l}{Energy Needed (kWh) From CPU} & \multicolumn{1}{l}{No. of Experiement} & \multicolumn{1}{l}{Total Carbon Footprint (g CO2e)} & \multicolumn{1}{l}{Total Energy Needed (kWh)} & CPU usage & Duration (min) & CPU Memory (GB) & GPU Memory (Utility)  {[}GB (\%){]} \\
% Chunking                     & 9.67                                                                                              & 0.02                                                                                        & 16.67                                                                                             & 0.04                                             & 358                                    & 9429.72                                             & 21.48                                         & 5 cores   & 15             & 15              & 3 (20 \%)                           \\
% PoS                          & 13.08                                                                                             & 0.03                                                                                        & 9.64                                                                                              & 0.02                                             & 358                                    & 8133.76                                             & 17.9                                          & 2 cores   & 20             & 14              & 5 (20 \%)                           \\
% NER                          & 12.9                                                                                              & 0.03                                                                                        & 22.22                                                                                             & 0.05                                             & 358                                    & 12572.96                                            & 28.64                                         & 5 cores   & 20             & 15              & 3 (20\%)                            \\
% Syntactic Arc Prediction     & 8.12                                                                                              & 0.02                                                                                        & 4.77                                                                                              & 0.01                                             & 358                                    & 4614.62                                             & 10.74                                         & 2 cores   & 10             & 13              & 5 (25 \%)                           \\
% Syntactic Arc Classification & 6.5                                                                                               & 0.01                                                                                        & 4.77                                                                                              & 0.01                                             & 358                                    & 4034.66                                             & 7.16                                          & 2 cores   & 10             & 13              & 4 (20 \%)                           \\
% BLiMP                        & 64.01                                                                                             & 0.14                                                                                        & 25.73                                                                                             & 0.06                                             & 358                                    & 32126.92                                            & 71.6                                          & 6 cores   & 30             & 8               & 10 (100\%)                          \\
% LAMA ConceptNet              & 5.06                                                                                              & 0.01                                                                                        & 14.27                                                                                             & 0.03                                             & 358                                    & 6920.14                                             & 14.32                                         & 6 cores   & 10             & 38              & 7 (15\%)                            \\
% LAMA Google                  & 1.32                                                                                              & 0.003                                                                                       & 1.83                                                                                              & 0.004                                            & 358                                    & 1127.7                                              & 2.506                                         & 2 cores   & 4              & 9               & 3 (10\%)                            \\
% LAMA Trex                    & 6.68                                                                                              & 0.01                                                                                        & 25.82                                                                                             & 0.06                                             & 358                                    & 11635                                               & 25.06                                         & 6 cores   & 20             & 9               & 4 (10\%)                            \\
% LAMA SQuAD                   & 0.65                                                                                              & 0.0014                                                                                      & 0.09                                                                                              & 0.002                                            & 358                                    & 264.92                                              & 1.2172                                        & 2 cores   & 2              & 7               & 2 (10\%)                            \\
% CAT                          & 171.14                                                                                            & 0.38                                                                                        & 20.42                                                                                             & 0.05                                             & 358                                    & 68578.48                                            & 153.94                                        & 1 cores   & 90             & 4               & 2 (60\%)                            \\
% oLMpics                      & 15.21                                                                                             & 0.03                                                                                        & 1.82                                                                                              & 0.004                                            & 358                                    & 6096.74                                             & 12.172                                        & 1 cores   & 8              & 4               & 2 (60\%)                           
% \end{tabular}
% \caption{}
% \label{tab:probing-carbon-cost}
% \end{table}
\begin{table*}[thb]
\small
\setlength\tabcolsep{8pt}   % Column separation
\def\arraystretch{1.8}      % row separation

\begin{tabular}{c|c|c}
\toprule
\textbf{Probe Name} & \textbf{Total Carbon Footprint (g CO2e)} & \textbf{Total Energy Needed (kWh)} \\
\cline{1-3}
\nelson Chunking                     & 26.34  & 0.06   \\
\nelson PoS                          & 22.72  & 0.05   \\
\nelson NER                          & 35.12  & 0.08   \\
\nelson Syntactic Arc Prediction     & 12.89  & 0.03   \\
\nelson  Syntactic Arc Classification & 11.27  & 0.02   \\
\blimp                        & 89.74  & 0.2    \\
\lama ConceptNet              & 19.33  & 0.04   \\
\lama Google                  & 3.15   & 0.007  \\
\lama Trex                    & 32.5   & 0.07   \\
\lama SQuAD                   & 0.74   & 0.0034 \\
\cat                          & 191.56 & 0.43   \\
\olmpics                     & 17.03  & 0.034 \\
\bottomrule
Total                      & 165535.62  & 345.2552 \\
\bottomrule
\end{tabular}

\caption{For every probing tasks, we report their Carbon Footprint (g CO2e) and Energy Needed (kWh) for one single run. For some tasks, it is more convenient for us to run all probing tests (e.g. 75 tests in \blimp has the same cost).  We ran those probing tasks with checkpoints reported in Table \ref{tab:num-checkpoints} and include the estimated total cost in the bottom line.}
\label{tab:probing-carbon-cost}
\end{table*}

==> tables/tab_small.tex <==
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}
\newcolumntype{R}[1]{>{\PreserveBackslash\raggedleft}p{#1}}
\newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[thb]
%\tiny
\small
\setlength\tabcolsep{2pt}   % Column separation
\def\arraystretch{1.4}      % row separation

\begin{tabular}{c|c|c|c|L{4.5cm}L{4.5cm}}
\toprule
\textbf{Package}            & \textbf{Knowledge}         & \textbf{Task}                                          & \textbf{Format}                        & \multicolumn{2}{c}{\textbf{Examples}}                                                                                          \\
\cline{1-6}
\multirow{6}{*}{\begin{tabular}{@{}c@{}} \nelson  \end{tabular}}                        & \multirow{11}{*}{Ling.}                   & \multirow{2}{*}{POS Tagging}                  & \multirow{4}{*}{\shortstack[c]{Token\\ Labeling}}      & \multicolumn{2}{c}{\multirow{1}{*}{\begin{dependency}[style=above]
          \begin{deptext}[column sep=0.2em]
              \graytextbf{PRON} \& \graytextbf{AUX} \& \textbf{VERB} \& \graytextbf{ADV} \& \graytextbf{ADP} \& \graytextbf{DET} \& \graytextbf{NOUN} \& \graytextbf{PUNCT} \\
              \graytextbf{I} \& \graytextbf{'m} \& \textbf{staying} \& \graytextbf{away} \& \graytextbf{from} \& \graytextbf{the}  \& \graytextbf{stock}  \& \graytextbf{.} \\
          \end{deptext}
        \end{dependency}}}                                                                                                  \\
 %                                            &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
 %                                            \cdashline{3-3}[1pt/1pt]
                                             %\cdashline{5-6}[1pt/1pt]
                                            %  \cline{3-6}
 %                                            &                                                & \multirow{2}{*}{Chunking}           &      & \multicolumn{2}{c}{\multirow{1}{*}{
 %       \begin{dependency}[style=above]
 %           \begin{deptext}[column sep=0.1em]
 %             \graytextbf{B-NP} \& \graytextbf{B-VP} \& \graytextbf{B-PP} \& \textcolor{black}{\textbf{B-NP}} \& \textcolor{lightgray}{\textbf{I-NP}} \& \textcolor{lightgray}{\textbf{I-NP}} \& \graytextbf{O} \\
 %             \graytext{\textbf{Shearson}} \& \graytext{\textbf{works}} \& \graytext{\textbf{at}} \& \textcolor{black}{\textbf{American}} \& \textcolor{lightgray}{\textbf{Express}} \& \textcolor{lightgray}{\textbf{Co}} \& \graytext{.} \\
 %         \end{deptext}
 %       \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cdashline{3-3}[1pt/1pt]
                                             \cdashline{5-6}[1pt/1pt]
                                             &                                                & \multirow{2}{*}{NER}     &       & \multicolumn{2}{c}{\multirow{1}{*}{\begin{dependency}[style=above]
            \begin{deptext}[column sep=0.2em]
              \graytextbf{O} \& \graytextbf{O} \& \textcolor{lightgray}{\textbf{I-ORG}} \& \textcolor{black}{\textbf{I-ORG}} \& \textcolor{lightgray}{\textbf{I-ORG}} \& \graytextbf{O} \& \graytextbf{O} \& \graytextbf{O} \& \graytextbf{O} \\
              \graytextbf{By} \& \graytextbf{stumps} \& \textcolor{lightgray}{\textbf{Kent}} \& \textcolor{black}{\textbf{County}} \& \textcolor{lightgray}{\textbf{Club}} \& \graytextbf{had} \& \graytextbf{reached} \& \graytextbf{108} \& \graytextbf{.} \\
          \end{deptext}
        \end{dependency}}}                                                                                                  \\
                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
                                             \cline{3-6}
                                             &                                                & \multirow{2}{*}{Arc Predict.} & \multirow{2}{*}{\shortstack[c]{Pair \\ Labeling}} & \multicolumn{2}{c}{\multirow{1}{*}{\begin{dependency}[edge vertical padding=-0.4ex]
          \begin{deptext} % [column sep=2em,]
              Peter \&[2em] and \& May \&[2em] bought \&[2em]  a \&[2em]  car \&[.0em] . \\
          \end{deptext}
          \deproot[edge unit distance=1.05ex, label style={text=gray,draw=gray}, edge style={gray,densely dotted,>=}, hide label]{4}{ROOT}
          \depedge[edge unit distance=1.1ex, label style={text=gray,draw=gray},  edge style={gray,densely dotted,>=}, hide label]{4}{2}{\tiny Subj}
          \depedge[edge unit distance=0.8ex, label style={text=gray,draw=gray}, edge style={gray,densely dotted,>=}, hide label]{2}{1}{\tiny Conj}
          \depedge[edge unit distance=0.8ex, label style={text=gray,draw=gray}, edge style={gray,densely dotted,>=}, hide label]{2}{3}{\tiny Conj}
          \depedge[edge unit distance=0.3ex, label style={text=gray,draw=gray}, edge style={gray,densely dotted,>=}, hide label]{6}{5}{\tiny Det}
        %   \depedge[edge unit distance=0.95ex, label style={text=lightgray,draw=lightgray}, edge style={lightgray,densely dotted},]{4}{7}{\tiny Punct}
          \depedge[edge unit distance=0.8ex, label style={text=red}, edge style={red!60!,thick,>=}]{3}{4}{\xmark}
          \depedge[edge unit distance=1ex, label style={text=red}, edge style={red!60!,thick,>=}]{1}{3}{\xmark}
          \depedge[edge unit distance=0.8ex, label style={text=darkgreen,}, edge style={darkgreen!60!black,thick,>=},]{4}{6}{\cmark} 
        \end{dependency}}}                                                                                                  \\
&                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
%                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
%                                             \cdashline{3-3}[1pt/1pt]
%                                             \cdashline{5-6}[1pt/1pt]
%                                             &                                                & \multirow{2}{*}{Arc Class.}     &  & 
%                                             \multicolumn{2}{c}{
%                                             \multirow{1}{*}{\begin{dependency}[edge vertical padding=-0.4ex]
%          \begin{deptext} % [column sep=2em]
%            %   Peter \& and \& May \& bought \&  a \&[1em]  car \&[.1em] . \\
%            Peter \&[2em] and \& May \&[2em] bought \&[2em]  a \&[2em]  car \&[.0em] . \\
%          \end{deptext}
%          \deproot[edge unit distance=1.05ex, label style={text=gray,draw=gray}, edge style={gray,densely dotted}, hide label]{4}{ROOT}
%          \depedge[edge unit distance=1.1ex, label style={text=gray,draw=gray}, edge style={gray,densely dotted}]{4}{2}{\tiny Subj}
%          \depedge[edge unit distance=0.8ex, label style={text=gray,draw=gray}, edge style={gray,densely dotted}]{2}{1}{\tiny Conj}
%          \depedge[edge unit distance=0.8ex, label style={text=gray,draw=gray}, edge style={gray,densely dotted}]{2}{3}{\tiny Conj}
%          \depedge[edge unit distance=0.8ex,]{4}{6}{\tiny Obj}
%          \depedge[edge unit distance=0.3ex, label style={text=gray,draw=gray}, edge style={gray,densely dotted}]{6}{5}{\tiny Det}
%        %   \depedge[edge unit distance=0.95ex]{4}{7}{\tiny Punct}
%        \end{dependency}}}                                                                                                  \\
%                                             &                                                &                                               &                                      & \multicolumn{2}{c}{}                                                                                                  \\
%                                             \cline{1-6}
%                       & \multirow{5}{*}{Ling.}                  & Irregular Forms                      & \multirow{5}{*}{\begin{tabular}{@{}c@{}} %Comparing \\ sentence scores \\
%$\mathbb{P}( \cmark)$\\
%$>  \mathbb{P}(\xmark)$? \end{tabular}}                     &  \cmark Aaron \textit{\textbf{broke}} the unicycle.                                   & \xmark Aaron \textit{\textbf{broken}} the unicycle.                              \\
%                                            \cdashline{3-3}[1pt/1pt]
%                                             \cdashline{5-6}[1pt/1pt]
 \cline{1-1} \cline{3-6}
\multirow{4}{*}{\blimp} &                                                & Det-Noun                                    &  \multirow{5}{*}{
\begin{tabular}{@{}c@{}} 
$\mathbb{S}(\cmark)$\\
$>  \mathbb{S}( \xmark)$? \end{tabular}}                    &  \cmark Rachelle had bought that \textit{\textbf{chair}}                             & \xmark Rachelle had bought that \textit{\textbf{chairs}}.                        \\
                                             \cdashline{3-3}[1pt/1pt]
                                             \cdashline{5-6}[1pt/1pt]
                                             &                                                & NPI Licensing                                 &                      & \cmark The truck has \textit{\textbf{clearly}}  tipped over                          & \xmark The truck has \textit{\textbf{ever}} tipped over                          \\
                                             
                                             \cdashline{3-3}[1pt/1pt]
                                             \cdashline{5-6}[1pt/1pt]
                                             &                                                & Island Effect                                            &                 & \cmark Which \textit{\textbf{bikes}} is John fixing?                   & \xmark Which is John fixing \textit{\textbf{bikes}}?                             \\
                                             \cdashline{3-3}[1pt/1pt]
                                             \cdashline{5-6}[1pt/1pt]
                                             &                                                & \multirow{2}{*}{Filler Gap}                                   &                      & \cmark Brett knew \textit{\textbf{what}} many waiters find.                          & \xmark Brett knew \textit{\textbf{that}} many waiters find.                      \\
                                             
                                             \cline{1-6}
\multirow{6}{*}{\lama}                        & \multirow{4}{*}{Factual}        & Google RE                                     & \multirow{6}{*}{\begin{tabular}{@{}c@{}}
Masked \\ LM \end{tabular}}                 & Einstein was born in \textit{\textbf{{[}MASK{]}}.}  & \cmark: \textit{\textbf{{[}MASK{]}}} $=$ 1879                             \\
                                             \cdashline{3-3}[1pt/1pt]
                                             \cdashline{5-6}[1pt/1pt]
                                             &                                                &  \multirow{2}{*}{T-REx}                                       &                   & Humphrey Cobb was a \textit{\textbf{{[}MASK{]}}} and novelist.     & \cmark: \textit{\textbf{{[}MASK{]}}} $= \text{screenwriter}$                             \\
                                             \cdashline{3-3}[1pt/1pt]
                                             \cdashline{5-6}[1pt/1pt]
                                             &                                                & SQuAD                                         &                   & A Turing machine handles \textit{\textbf{{[}MASK{]}}} on a strip of tape.  & \cmark: \textit{\textbf{{[}MASK{]}}} $ = \text{symbols}$                        \\
                                             \cline{2-2}
                                             \cdashline{3-3}[1pt/1pt]
                                             \cdashline{5-6}[1pt/1pt]
                                             &   \multirow{9}{*}{CSense}       & \multirow{2}{*}{ConceptNet}                                     &                   & You can use \textit{\textbf{{[}MASK{]}}} to bathe your dog.   &  \cmark: \textit{\textbf{{\textbf{[}MASK{]}}}} $= \text{shampoo}$                                 \\
                                             \cline{1-1}  \cline{3-6}
\multirow{7}{*}{\cat}                         & 
                   & \multirow{2}{*}{Conjunction}                      & \multirow{7}{*}{
\begin{tabular}{@{}c@{}} 
$\mathbb{S}(\cmark)$\\
$>  \mathbb{S}( \xmark)$?
%$\frac{\mathbb{S}(\cmark)}{|\cmark|}$\\
%$>  \frac{\mathbb{S}(\xmark)}{|\xmark|}$? 
\end{tabular}}                      
&  \cmark Jim yelled at Kevin  \textit{\textbf{because}} Jim was so upset. & \xmark Jim yelled at Kevin \textit{\textbf{and}}  Jim was so upset.                                                                                                  \\
                                            \cdashline{3-3}[1pt/1pt]
                                            \cdashline{5-6}[1pt/1pt]
                                             &                                                & \multirow{2}{*}{Winograd}                      &                     &  \cmark The fish ate the worm. The \textit{\textbf{fish}} was hungry.  & \xmark The fish ate the worm. The \textit{\textbf{worm}} was hungry.                                                                                                  \\
                                             \cdashline{3-3}[1pt/1pt]
                                             \cdashline{5-6}[1pt/1pt]
%  &                                                & Sense Making                                  &              &        \cmark Money can be used for buying \textit{\textbf{cars}}. & \xmark Money can be used for buying \textit{\textbf{stars}}.                                                                                      \\
                                             \cdashline{3-3}[1pt/1pt]
                                             \cdashline{5-6}[1pt/1pt]
                                             &                                                & \multirow{3}{*}{SWAG}      &                      & \multicolumn{2}{l}{Prompt: Someone unlocks the door and they go in.}\\
                                             &                                                &                &                       &    \multicolumn{2}{l}{\cmark \textit{\textbf{Someone leads the way in}}. \xmark \textit{\textbf{Someone walks out of the driveway}}}\\
                                             &                                                &                &                       &    \multicolumn{2}{l}{\xmark \textit{\textbf{Someone opens the door and walks out}}.}\\
                                            % &                                                &                &                       &    %\multicolumn{2}{l}{\xmark \textit{\textbf{Someone walks out of the driveway}}. }\\
                                            % &                                                &                &                       &    %\multicolumn{2}{l}{\xmark \textit{\textbf{Someone walks next to someone and sits on a pew.}}}\\
                                             \cdashline{3-3}[1pt/1pt]
%                                             \cdashline{5-6}[1pt/1pt]
%&                                          %      &  \multirow{3}{*}{Argument}              &                     &   \multicolumn{2}{l}{People can choose not to use Google, <insert>} \\
%&                                                &  &  & \multicolumn{2}{l}{Google is not a harmful monopoly.} \\
%                                             People can choose not to use Google,} <insert> Google is not a harmful monopoly.} \\
%                                             &                                                &                 &                     &  \multicolumn{2}{l}{\cmark \textit{\textbf{and since all other search engines re-direct to Google}},}      \\
%                                             &                                                &                 &                     &   \multicolumn{2}{l}{
%                                             \xmark \textit{\textbf{but since other search engines do not re-direct to Google}}, }    \\
                                    \cline{1-6}
\multirow{4}{*}{\olmpics} & \multirow{4}{*}{Reason} & \multirow{2}{*}{Taxonomy}                        & \multirow{4}{*}{\shortstack[c]{Masked\\ LM}}                 & A ferry and a floatplane are both a type of \textit{\textbf{{\textbf{[}MASK{]}}}}.  & \cmark vehicle  \xmark airplane \xmark boat            \\
                        \cdashline{3-3}[1pt/1pt]
                        \cdashline{5-6}[1pt/1pt]
                         &                            & \multirow{2}{*}{Age}                                  &                  & A 21 year old person age is \textit{\textbf{{[}MASK{]}}} than a 35 year old person. & \cmark younger \xmark older             \\
 %                        \cdashline{3-3}[1pt/1pt]
 %                       \cdashline{5-6}[1pt/1pt]
 %                        &                            & Object                              &                  & 
 %                        The size of a airplane is usually much \textit{\textbf{{[}MASK{]}}} than the size of a house. & \xmark smaller \cmark larger              \\
 %                        \cdashline{3-3}[1pt/1pt]
 %                       \cdashline{5-6}[1pt/1pt]
 %                        &                            & Always-Never                                  &                  & A chicken \textit{\textbf{{[}MASK{]}}} has horns.  & \cmark  never \xmark rarely  \xmark sometimes  \xmark often \xmark always                \\
 %                        \cdashline{3-3}[1pt/1pt]
 %                       \cdashline{5-6}[1pt/1pt]
 %                        &                            & Multi-Hop                         &                  & When comparing a 23, a 38 and a 31 year old, the \textit{\textbf{{[}MASK{]}}} is oldest. & \cmark second \xmark first  \xmark third
\bottomrule
\end{tabular}
\caption{Overview of example probing tasks. $\mathbb{S}$ denotes a scoring function that uses a pretrained language model. \yizhong{It seems that this new version removes some tasks due to the bigger font? Then we don't have a comprehensive list of the all the probe tasks. And some task names don't align with those in Figure 1. Which one do you prefer?} \jungo{Yeah I couldn
t include all of them. I personally prefer readability over comprehensiveness, but we'll see what Hanna/Noah says.} }
%\caption{Detailed illustration of representative tasks from selected probe packages. $\mathbb{S}(\cdot)$ scores a sentence by sequentially masking words in sentence and accumulating log probability of masked words.  $\mathcal{C}$ denotes the rest of sentence without the masked word and $\mathbb{P}(\cdot \mid \mathcal{C})$ is the conditional distribution over the vocabulary given $\mathcal{C}$; $V_{\text{PTLM}}$ is the vocabulary of the PTLM that are grammatical words or numbers. }
\label{tab:examples-small}
\end{table*}
